Prediction-Correction Algorithms for Time-Varying Constrained Optimization

This paper develops online algorithms to track solutions of time-varying constrained optimization problems. Particularly, resembling workhorse Kalman filtering-based approaches for dynamical systems, the proposed methods involve prediction-correction steps to provably track the trajectory of the optimal solutions of time-varying convex problems. The merits of existing prediction-correction methods have been shown for unconstrained problems and for setups where computing the inverse of the Hessian of the cost function is computationally affordable. This paper addresses the limitations of existing methods by tackling constrained problems and by designing first-order prediction steps that rely on the Hessian of the cost function (and do not require the computation of its inverse). In addition, the proposed methods are shown to improve the convergence speed of existing prediction-correction methods when applied to unconstrained problems. Numerical simulations corroborate the analytical results and showcase performance and benefits of the proposed algorithms. A realistic application of the proposed method to real-time control of energy resources is presented.

==> Algorithm.tex <==
% !TEX root = TimeVarying_part1.tex
\section{Centralized algorithm}\label{sec:centr}

We first focus on centralized algorithms, i.e., algorithms that assume that the computations are performed by a unique computing entity. In order to converge to the solution trajectory $\x^*(t)$, we will generate a sequence of near optimal decision variables $\{\x_k\}$ by taking into account both how the solution changes in time and how different our current update is from the optimizer at each time step. To do this, we set up a prediction-correction scheme, much like a Kalman filter strategy in estimation theory. In the first step, we will predict how the solution changes, and in the correction step we will do one step of gradient or Newton method towards the optimizer at that time instance. As mentioned in the Introduction, we call this strategy \emph{solution tracking}, to contrast it with standard \emph{running} algorithms that do not predict how the solution changes, but only adapt to it. 

\subsection{Prediction step}

To generate the prediction step, we reformulate the time-varying problem~\eqref{eq.problem} in terms of optimality conditions. Solving~\eqref{eq.problem} means to compute the solution of the following nonlinear system of equations
\begin{equation}
\nabla_{\x} f(\x^*(t); t) = \mathbf{0}, 
\end{equation}
for each $t$. For any other vector $\x$ (for example the approximate solution $\x_k$), we can write 
\begin{equation}\label{eq.isoerror}
\nabla_{\x} f(\x; t) = \r(t)
\end{equation}
where $\r(t)$ is some residual error. The aim of the prediction step is to keep this residual error as much fixed as possible while the optimization problem is changing. To say it in another way, we want to predict how to update $\x_k$ such that we stay close to the iso-residual manifold.  We can see how such trajectory evolves by perturbing it as
\begin{equation}
\nabla_{\x} f(\x; t) + \nabla_{\x\x} f(\x; t) \delta\x + \nabla_{t\x} f(\x; t) \delta t = \r(t),  
\end{equation}
and by using~\eqref{eq.isoerror} and by dividing it by $\delta t \neq 0$, we obtain the continuous dynamical system
\begin{equation}\label{eq.dyn}
\dot{\x} = - [\nabla_{\x\x} f(\x; t)]^{-1} \nabla_{t\x} f(\x; t). 
\end{equation}
By passing now in the discrete domain (where our algorithm will live), we sample the problem at sampling times $t_k$, for $k = 0,1,2,\dots$, and for the sake of simplicity we let this sampling be uniform, with sampling interval equal to $h$. We can integrate~\eqref{eq.dyn} by using a first-order forward Euler scheme as   
\begin{multline}\label{eq.up}
{\x}(t_{k+1}) = \x(t_{k}) - [\nabla_{\x\x} f(\x(t_k); t_k)]^{-1} \nabla_{t\x} f(\x(t_k); t_k) \, h \\ + \Delta,
\end{multline}
where $\Delta$ represents the discretization error. The discretization error can be upper bounded as follows. 

\begin{proposition}\label{prop.err}
Under Assumptions~\ref{as.0}, \ref{as.str}, and \ref{as.smooth}, the discretization error $\Delta$ of the Euler method~\eqref{eq.up} w.r.t. the real dynamics~\eqref{eq.dyn} is upper bounded by
$$
\Delta \leq \frac{h^2}{2}\left[\frac{C_0 C_2}{m^2} + \frac{C_3}{m}\right] = O(h^2).
$$
\end{proposition}
\vskip2mm

\begin{proof}
See Appendix~\ref{ap.prop}.
\end{proof}
\vskip2mm

Proposition~\ref{prop.err} says that under our assumptions we can use the Euler method. We will forget for the moment of the constant in the discretization error and live with its order in $h$ only. We can use the update rule~\eqref{eq.up} as the basics of our prediction step. Let ${\x}_{k+1|k}$ be the predicted decision variable vector; this will be computed as
\begin{equation}\label{eq:update}
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h.
\end{equation}


\subsection{Correction step}

The correction step can be devised by using, for example, a constant stepsize  projected gradient method based on the updated objective function at time $t_{k+1}$
\begin{equation}\label{eq.corr}
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \gamma \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})],
\end{equation}
for a choice of stepsize $\gamma > 0$, and where $P_{X}$ is the projection operator. Another way to design the correction step would be to use projected Newton's method; we will see how to perform that in Section~\ref{sec:newton}.  


{\color{green} [Here some words on the algorithm!]}


\subsection{Convergence analysis}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Centralized solution tracking (gradient-based)}
\label{alg.centr}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h
$$
\textbf{2:} Correction step:
$$
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \gamma \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})]
$$ 
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%

In Algorithm~\ref{alg.centr}, we summarize the devised centralized algorithm, whose convergence is encoded in the following theorem. 

\begin{theorem}\label{th.centr}
Let Assumption~\ref{as.0}, \ref{as.str}, and \ref{as.smooth} hold and let $\{\x_k\}$ be the sequence generated by Algorithm~\ref{alg.centr}. Define the rates $\rho$ and $\sigma$ as
%
\begin{equation}\label{thm:rho_sigma}
\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}, \quad \sigma = 1 + h(C_0 C_1/m^2 + C_2/m).
\end{equation}
%
\begin{enumerate}
\item If the sampling interval $h$ is chosen sufficiently small, then there exists a $\gamma>0$ for which 
\begin{equation*}
\rho \sigma < 1
\end{equation*}
and, in this case, convergence of $\{\x_k\}$ to $\x^*(t_k)$ is Q-linear up to a bounded error as,
\begin{equation}\label{result1}
\|{\x}_{k} - \x^*(t_{k})\| \leq (\rho \sigma)^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h^2).
\end{equation}
\item Irrespectively of the selection of $h$, if we pick $\gamma < m/L^2$, then convergence goes as   
\begin{equation}\label{result2}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h).
\end{equation}
\end{enumerate} 
\end{theorem}
%
\vskip2mm
\begin{myproof}

In order to prove Theorem~\ref{th.centr}, we start by bounding the error in the prediction step by terms that depend on the functional smoothness and the discretization error using Taylor expansions. Then we bound the tracking error of the gradient step using standard convergence properties of gradient descent on strongly convex functions. By substituting the error improvement achieved in the correction step into the prediction step, we establish the main result.

First, we establish that the criteria in which the bound stated in \eqref{result1} may be satisfied, i.e. that $\rho \sigma$ can be made strictly less than one, for a sufficiently small $h$. Note that, since $m>0$, there is always a $\gamma$ that makes $\rho < 1$ since $\gamma < m/L^2$. In particular, if we take $\gamma = m/ 2 L^2$, then $\rho$ is minimized and it is equal to 
%
\begin{equation}\label{rho}
\rho^* = \sqrt{ 1 - \frac{m^2}{4 L^2}}. 
\end{equation}
%
The coefficient $\sigma$ is a monotonically increasing function in $h$, and it is equal to $1$ when $h = 0$; by continuity of $\sigma$ in $h$, we can always find a small enough stepsize $h$, such that $\sigma < 1/\rho^*$, which means that we can find a stepsize $\gamma$ that yields $\rho \sigma <1$.

Now we turn to establishing the discrete-time sampling error bound stated in \eqref{result1} is achieved by the updates \eqref{eq:update}-\eqref{eq.corr}. For simplicity, we modify the notation to omit the arguments $\x_k$ and $t_k$ of the function $f$. In particular, define $\nabla_{\x\x}f = \nabla_{\x\x}f(\x_k; t_k)$, $\nabla_{t\x} f = \nabla_{t\x} f(\x_k; t_k)$, $\nabla_{\x\x}f^* = \nabla_{\x\x}f({\x}^*(t_{k}); t_k)$, and $\nabla_{t\x} f^* = \nabla_{t\x} f({\x}^*(t_{k}); t_{k})$. 

Begin by considering the update~\eqref{eq:update}, the prediction step, evaluated at a generic point $\x_k$ sampled at the current sample time $t_k$ and with associated optimizer $\x^*(t)$, which due to optimality will have null residual vector $\r(t) = \mathbf{0}$. Thus we may write
%
\begin{equation*}\left\{\begin{array}{rcl}
{\x}_{k+1|k} &=& \x_{k} - [\nabla_{\x\x}f]^{-1}\nabla_{t\x} f\,h\\
{\x}^*(t_{k+1}) &=& {\x}^*(t_{k}) - [\nabla_{\x\x}f^*]^{-1} \nabla_{t\x} f^*\,h + O(h^2).
\end{array}\right.
\end{equation*}
%
By subtracting one from the other and by considering the norm of the result, we obtain 
%
\begin{align}\label{eq.imp}
\|{\x}_{k+1|k}& -  \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\|  \\  & + \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h + O(h^2) .\nonumber 
\end{align}
%
Set the second term in the right-hand side of \eqref{eq.imp} as  $a= \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h$. We may rewrite $a$ by adding and subtracting the Newton step with the Hessian evaluated at the current optimal point,  $[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f$, to obtain
%
\begin{align}\label{eq.hessian_cross_term}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h,
\end{align}
%
We may bound the first and second-order derivative terms in the previous expression \eqref{eq.hessian_cross_term} by using Assumption~\ref{as.smooth} regarding the functional smoothness as well as the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} to write
%
\begin{equation}\label{eq.a}
a  \leq C_0 h \left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We now further bound the first term of the right-hand-side. To do that, we use the non-singularity of the Hessian to write 
%
\begin{multline}\label{eq.dummy10_midstep}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| = \\ \|[\nabla_{\x\x}f^*]^{-1}(\nabla_{\x\x}f - \nabla_{\x\x}f^*)[\nabla_{\x\x}f]^{-1} \|,
\end{multline} 
%
which by employing, once again, the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} we can bound as
\begin{equation}\label{eq.dummy10}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| \leq \frac{1}{m^2}\|\nabla_{\x\x}f - \nabla_{\x\x}f^* \|,
\end{equation} 
%
and therefore~\eqref{eq.a} can be written as
\begin{equation}\label{eq.amid}
a  \leq \frac{C_0}{m^2} h \left\|\nabla_{\x\x}f - \nabla_{\x\x}f^*\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We consider the Taylor expansion of the mixed second-order terms and the second-order terms in \eqref{eq.amid}, and apply the Mean Value Theorem with $\tilde{\x}$ as a point on the line between $\x_k$ and $\x^*(t_k)$ to obtain the following expressions,
%
\begin{subequations}\label{eq.dummy11}
\begin{multline}
\left\| \nabla_{\x\x} f- \nabla_{\x\x} f^*  \right\| \leq \left\|\nabla_{\x \x\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \\ \leq C_1 \|\x_k - \x^*(t_k)\|
\end{multline}
\begin{multline}
\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| \leq \left\|\nabla_{\x t\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \\ \leq C_2 \|\x_k - \x^*(t_k)\|
\end{multline}
\end{subequations}
%
The expressions in \eqref{eq.dummy11} may be substituted together into~\eqref{eq.amid} to yield
 %
\begin{align}
a  &\leq \frac{C_0 C_1 h}{m^2}\|\x_k - \x^*(t_k)\| + \frac{C_2 h}{m}\|\x_k - \x^*(t_k)\|.
\end{align}
%
Now we can use this bound for $a$ in~\eqref{eq.imp} to get
%
\begin{multline*}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \\ \Big[1 + h\left(\frac{C_0 C_1 h}{m^2} + \frac{C_2 h}{m}\right) \Big]\|{\x}_{k} - \x^*(t_{k})\| + O(h^2).
\end{multline*}
%
which, by the definition of $\sigma$ as stated in \eqref{thm:rho_sigma} in Theorem \ref{th.centr}, allows us to conclude
%
\begin{equation}\label{eq.fin1}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \sigma \|{\x}_{k} - \x^*(t_{k})\| + O(h^2).
\end{equation}
%
For the correction step [cf. \eqref{eq.corr}] , we may use the standard property of projected gradient descent for strongly convex functions. In particular, the gradient converges Q-linearly as
%
\begin{equation}\label{eq.fin2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \|{\x}_{k+1|k} - \x^*(t_{k+1})\|
\end{equation}
%
where $\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}$, see \cite{Nesterov2004} for further details.
%
%\subsection{Total algorithm}

We are ready to consider the combined error bound achieved by the prediction-correction scheme. By plugging the correction error \eqref{eq.fin2} into the prediction error \eqref{eq.fin1} we obtain
%
\begin{equation}\label{eq.fin_t_k}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \sigma \|{\x}_{k} - \x^*(t_{k})\| + \rho O(h^2).
\end{equation}
%
Now recursively apply the relationship \eqref{eq.fin_t_k} backwards in time to the initial time sample at $t_0$ to write
%
\begin{equation*}\label{eq.fin_t_0}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq (\rho \sigma)^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h^2),
\end{equation*}
%
which is the result \eqref{result1} in Theorem \ref{th.centr}.

To establish the result stated in \eqref{result2} of Theorem \ref{th.centr}, observe that in the worst case, we may upper bound the term $a$ in \eqref{eq.amid} by using the bounds in Assumption \ref{as.smooth} to obtain the right hand side of the following expression 
%
\begin{align}\label{eq.worst_case}
a  & \leq  \frac{C_0 h}{m^2}
 \|\nabla_{\x\x}f - \nabla_{\x\x}f^*\| 
 + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| \nonumber\\
 & \leq \frac{2 C_0 L h}{m^2} + \frac{2 C_0 h}{m} = O(h),
\end{align}
%
Remembering the definition of the nonnegative scalar term $a=\left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h $ and substituting the bound~\eqref{eq.worst_case} into \eqref{eq.imp}, we can write
%
\begin{equation}\label{eq.a_subst}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\| + O(h).
\end{equation}
%
This, together with the contraction property of the gradient step as stated in \eqref{eq.fin2} yields
%
\begin{equation}\label{eq.sampling_error2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \|{\x}_{k} - \x^*(t_{k})\| + \rho O(h).
\end{equation}
%
If we iterate the expression \eqref{eq.sampling_error2} backwards in time to the initial point ${\x}_{0}$, we obtain
%
\begin{equation}\label{eq.rho_error_dependence}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h),
\end{equation}
%
which is~\eqref{result2}. With $\rho= \sqrt{1 + \gamma^2 L^2 - \gamma m}$ as defined in \eqref{thm:rho_sigma}, we only need to find a $\gamma$ that makes $\rho < 1$. Selecting any $\gamma$  satisfying $\gamma < m/L^2 $ concludes the proof.

\end{myproof}


\vskip2mm
\begin{corollary}\label{co.centr}
Under the same conditions of Theorem~\ref{th.centr},
\begin{enumerate}
\item If we pick $\gamma = m/2 L^2$, then the convergence bounded error is between $O(h)$ and $O(h^2)$. 
\item If we do not perform the prediction step in Algorithm~\ref{alg.centr} but only the correction step (i.e., we use Algorithm~\ref{alg.centr} as a running algorithm), then, if we pick $\gamma < m/L^2$, convergence goes as 
\begin{equation*}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h).
\end{equation*}
\end{enumerate}
\end{corollary}
%
\vskip2mm
\begin{myproof}

Point 1) follows from the proof of Theorem~\ref{th.centr}. In fact, if we select $\gamma = m/2 L^2$ then we minimize $\rho$ (as stated in~\eqref{rho}). Therefore, with this selection of $\gamma$, two cases are possible. 

The first case is that $h$ is small enough, such that $\rho \sigma < 1$. Here, we can use the first part of Theorem~\ref{th.centr} and, in particular, Equation~\eqref{result1}, which brings a bounded error of size $O(h^2)$. 

The second case is that $h$ is not small enough, such that $\rho \sigma \geq 1$. Here, we can use the second part of Theorem~\ref{th.centr}, i.e., Equation~\eqref{result2}, to bound the asymptotical error to $O(h)$. 

By putting together the two cases, the claim of Point 1) follows. 

Point 2) also follows directly from the proof of Theorem~\ref{th.centr}. Suppose that we execute the correction step \eqref{eq.corr} without the prediction step \eqref{eq:update}. Such an update would be equivalent to performing the updates \eqref{eq:update}-\eqref{eq.corr} with the prediction step evaluated at $\nabla_{t\x} f = {\bf{0}}$. Substituting this case into \eqref{eq.imp} yields
\begin{align*}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| &\leq \|{\x}_{k} - \x^*(t_{k})\| \\
 & \qquad + \left\|[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h 
	+ O(h^2) \\ 
	&\leq \|{\x}_{k} - \x^*(t_{k})\| + \frac{C_0 h}{m} + O(h^2) \\
	 & \leq \|{\x}_{k} - \x^*(t_{k})\| + O(h),
\end{align*}
%
where we have bounded the magnitude of the Hessian and the derivative mixed first order derivative terms using Assumptions \ref{as.str}-\ref{as.smooth}, respectively. From here, the analysis proceeds exactly as from \eqref{eq.a_subst} to the conclusion of 2) in Theorem~\ref{th.centr}, yielding \eqref{eq.rho_error_dependence}, which concludes the proof. 

\end{myproof}

\vskip2mm
Theorem~\ref{th.centr} says that our tracking algorithm generates a converging sequence of approximate solutions and the error bound depends (at worst) linearly on the sampling interval. Convergence is quite fast (in fact Q-linear), as one would expect in strongly convex problems. Corollary~\ref{co.centr} confirms our intuition that performing the prediction step improves upon state-of-the-art running algorithms (passing from an error bound of $O(h)$ to $O(h^2)$ if $h$ is chosen small enough). 


\begin{remark}\label{rem.k}
We can readily extend the results on this section and the following one when the constant $C_0, C_1, C_2, m, L$ are constant in the decision variable $\x$ but not uniformly in time. In order to do that, we have to substitute these constants by other ones, depending on the sampled time instance $t_k$ as $C_{0,k}, C_{1,k}, C_{2,k}, m_k, L_k$. With this substitution, all the results hold true (with minor modifications) and in particular the stepsize $\gamma$ can be chosen to vary from $k$ to $k+1$. 
\end{remark}


\section{Newton correction}\label{sec:newton}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Centralized solution tracking (Newton-based)}
\label{alg.newton}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h.
$$
\textbf{2:} Correction step:
\begin{multline*}
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \\ [\nabla_{\x\x} f(\x_{k+1|k}; t_{k+1})]^{-1} \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})]
\end{multline*}
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%
In this section, we explore the possibility of using a Newton's step for the correction step in Algorithm~\ref{alg.centr}. We want to see if substituting~\eqref{eq.corr} with 
\begin{multline}
{\x}_{k+1} = \x_{k+1|k} - [\nabla_{\x\x} f(\x_{k+1|k}; t_{k+1})]^{-1}\times\\ \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})
\end{multline}
yields a further decrease in the asymptotic error from $O(h^2)$ to something smaller than that. Intuitionally that should be the case, since Newton's method has local quadratic convergence, so we expect to reduce $O(h^2)$ to a $O(h^4)$ error. In this section, we will prove that this is not in general the case, which undermines the usefulness of a Newton's correction step in time-varying problems. 


In particular, we analyze the local convergence of Algorithm~\ref{alg.newton}. 

\begin{theorem}\label{th.newton}
Let Assumptions~\ref{as.0}, \ref{as.str}, and \ref{as.smooth} hold true. Suppose the initial guess $\x_0$ is picked close enough to the initial optimizer, i.e., the norm $\|\x_0 - \x^*(t_0)\| \leq \alpha h^2 /2$, with $\alpha h^2 /2 \ll 1$. Define the parameter $\alpha' = [C_0 C_2/ m^2 + C_3/m]$, so that the Euler discretization error $\Delta$ in Proposition~\ref{prop.err} has the worst case value of $\Delta = \alpha' h^2/2$. In addition, suppose that this worst case value is small enough, i.e., $\alpha' h^2/2 \ll 1$. With this in place, for the sequence $\{\x_k\}$ generated by Algorithm~\ref{alg.newton} we have for all $k>1$
\begin{enumerate}
\item if $C_1/2 m \leq 2\alpha/[(\alpha + \alpha')^2\, h^2]$, then 
$$
\|\x_k - \x^*(t_k)\| \leq O(h^2),
$$
\item if, in addition, $C_1/2 m \leq 1$, then 
$$
\|\x_k - \x^*(t_k)\| \leq O(h^4).
$$
\end{enumerate}
\end{theorem}
\vskip2mm

\begin{proof}
See Appendix~\ref{ap.newton}. 
\end{proof}
\vskip2mm

Theorem~\ref{th.newton} says that, in general, if we select $h$ small enough, we can track the optimizer $\x^*(t_k)$ at worst with a $O(h^2)$ error bound. This is very similar to the result we had for the gradient-based tracking algorithm. In special cases, when $C_1/2m \leq 1$, then the quadratic convergence of the Newton's method appears and we track the optimizer at worst with a error bound of $O(h^4)$. A special case of the second situation are quadratic cost functions, for which $C_1 = 0$, and we have perfect convergence. 

%We will see in the simulation results in Section~\ref{sec:num} that, in practice, since both $C_1$ and $m$ vary in time, Algorithm~\ref{alg.newton} generates a sequence that oscillates between a $O(h^2)$ error level and a $O(h^4)$ one, thereby making a Newton's correction step less useful, beyond limited special cases.   


\section{Approximate time derivative}\label{sec:app}

In several situations, we are not provided with the knowledge of how the function changes in time. 

\textcolor{red}{In which situations would one expect to need to do such an approximation? Is there a connection to stochastic control in discrete time?}

In these situations, to still be able to use our algorithms, we need to estimate the term $\nabla_{t\x} f(\x; t)$ is some ways. Let $\tilde{\nabla}_{t\x}{f}_k$ be an approximate version of $\nabla_{t\x}f(\x_k; t_k)$. Examples of such approximate version are the following. 

%We notice that most of the analysis in Theorem~\ref{th.centr} and \ref{th.net} carries trough unchanged. The only addition in the proofs is that we need to consider the extra source of error
%\begin{equation}\label{extraerr}
%\frac{h}{m}\|\tilde{\nabla}_{t\x}{f}_k -  \nabla_{t\x}f(\x_k; t_k)\| 
%\end{equation}
%which can be easily bounded once $\tilde{\nabla}_{t\x}{f}_k$ is available. Examples are the following.

\vskip2mm
\noindent\textbf{First-order backward derivative.} We can approximate the derivative as 
\begin{equation}\label{fobd}
\tilde{\nabla}_{t\x}{f}_k = \frac{1}{h} (\nabla_{\x}f(\x_k; t_k) - \nabla_{\x}f(\x_{k-1}; t_{k-1})),
\end{equation}
which has an approximation error of $O(h)$. %This combined with the $h$ factor in~\eqref{extraerr} brings the additional error to an $O(h^2)$ level.

\vskip2mm
\noindent\textbf{Higher-order backward derivative.} We can approximate the derivative recursively as
\begin{multline*}
\tilde{\nabla}_{t\x}{f}_k = \frac{1}{h}\left(a \nabla_{\x}f(\x_k; t_k) + b \nabla_{\x}f(\x_{k-1}; t_{k-1})\right. \\ \left.+ c \nabla_{\x}f(\x_{k-2}; t_{k-2}) + d\nabla_{\x}f(\x_{k-3}; t_{k-3})\right) - \beta \tilde{\nabla}_{t\x}{f}_{k-1},
\end{multline*}
which, if we specify the coefficient $(a,b,c,d,\beta)$ properly, leads to an approximation error of $O(h^2)$, $O(h^3)$, or $O(h^4)$~\cite{Lee1992}. %and therefore yields an error of at least one order of magnitude lower than the existing error bound. 

\vskip2mm
In the next corollary, we quantify the additional error of approximating the time derivative in our prediction-correction Algorithm~\ref{alg.centr}. We further show that this error goes as $O(h^2)$ for a simple first-order backward derivative, thereby stating that estimating the time derivative is not detrimental for our scheme. 

\begin{corollary}\label{co.approx}
Under the same conditions of Theorem~\ref{th.centr}, if we approximate the time derivative $\nabla_{t\x}f(\x_k; t_k)$ by using a first-order backward derivative as in~\eqref{fobd}, the asymptotic error bound of Algorithm~\ref{alg.centr} is not worse than the one of Theorem~\ref{th.centr}.  
\end{corollary}
%
\vskip2mm
\begin{myproof}

By Taylor expansion, one can see that
\begin{equation}\label{appder_oh}
\|\tilde{\nabla}_{t\x}{f}_k  - {\nabla}_{t\x}{f}(\x_k; t_k)\| = O(h),  
\end{equation}
also proving the claimed $O(h)$ error bound of the first-order backward derivative. In fact, one Taylor expands
\begin{equation}
{\nabla}_{\x}{f}(\x_{k-1}; t_{k-1}) = {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h + O(h^2),
\end{equation} 
and by solving for ${\nabla}_{t\x}{f}(\x_k; t_k)$, 
\begin{equation}
{\nabla}_{t\x}{f}(\x_k; t_k) = \frac{1}{h} ( {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h + O(h^2)).
\end{equation}
By substituting this result and the definition~\eqref{fobd} into~\eqref{appder_oh}, the $O(h)$ error bound is proven. 

Consider now the approximate prediction step, 
\begin{equation}
\x_{k+1|k} = \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h,
\end{equation}
which by adding and subtracting the exact prediction direction becomes, 
\begin{align}
\x_{k+1|k} &= \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h + \nonumber \\ &\quad 
+[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h  \nonumber \\ &\quad - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h.
\end{align}
By following the same steps as in Theorem~\ref{th.centr}, the term $a$ in Equation~\eqref{eq.hessian_cross_term} can be written with an extra error term as, 
\begin{align}\label{eq.hessian_cross_term_2}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h \nonumber \\ &\quad + \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h.
\end{align}
%
The extra error term w.r.t. Equation~\eqref{eq.hessian_cross_term} can be further bounded by using~\eqref{appder_oh} and the smoothness Assumption~\ref{as.smooth} (with the strong convexity constrant $m$)
\begin{multline}
 \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h \leq \\
 \|[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1}\| \| {\nabla}_{t\x}{f}(\x_k; t_k)  - \tilde{\nabla}_{t\x}{f}_k \| \, h \leq \\
 \frac{1}{m} O(h) \, h = O(h^2).
\end{multline}
This means that the extra error is of size $O(h^2)$ so it will not increase the $O(h^2)$ error bound already proven in Theorem~\ref{th.centr}.

\end{myproof}

Corollary~\ref{co.approx} says that we can approximate the time derivative simply by a first-order scheme. Better approximation will not decrease the functional dependence of the error in $h$, but may decrease the its magnitude. In the simulation results we show that

{\color{green} [Finish.]}  

\section{Prediction-Correction$(s)$ algorithms}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Prediction-Correction$(s)$ (gradient-based)}
\label{alg.pcs}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h
$$
\textbf{2:} Correction step: \\
\hspace*{4mm} \textbf{Set} $\x_{k+1/s|k} = \x_{k+1|k}$\\
\hspace*{4mm} \textbf{For} $\tau=1$ to $s$ \textbf{do}
$$
{\x}_{k+\tau/s} = P_{X}[\x_{k+\tau/s|k} - \gamma \nabla_{t\x} f(\x_{k+\tau/s|k}; t_{k+1})]
$$ 
\hspace*{4mm} \textbf{End}
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%


If we have enough computational power, we could always think to perform several correction steps (either of a gradient method or of a Newton's scheme), to further reduce the tracking asymptotical error. We call these algorithms Prediction-Correction$(s)$ algorithms (and they are parametrized over the number $s$ of correction steps. An example of such algorithm for gradient descent is given in Algorithm~\ref{alg.pcs}.

Convergence of such schemes can be proven in a similar fashion as in Theorem~\ref{th.centr}. As a bonus, in these schemes, the bigger $s$ is the larger $h$ can be chosen. This result as well as the convergence is encoded as follows. 

\begin{corollary}\label{co.pcs}
Under the same conditions of Theorem~\ref{th.centr}, Algorithm~\ref{alg.pcs} generates a sequence $\{\x_k\}$ that converges to $\x^*(t_k)$ asymptotically, with an error bound of 
$$
\lim_{k\to\infty} \|\x(t_k) - \x^*(t_k)\| = \frac{\rho^s}{1-\rho^s} O(h^2), \textrm{ if } \rho^s \sigma < 1, 
$$
and
$$
\lim_{k\to\infty} \|\x(t_k) - \x^*(t_k)\| = \frac{\rho^s}{1-\rho^s} O(h), \textrm{ if } \rho^s \sigma \geq 1, \rho < 1.
$$
In addition, if $s$ is selected as 
$$
s \geq \left\lceil \frac{p \log h}{\log(\rho(1 + h^p))}\right\rceil,
$$
then the asymptotical error is multiplied by a term $O(h^p)$.
\end{corollary}
%
\vskip2mm
\begin{myproof}

The proof is rather immediate and follows from the proof of Theorem~\ref{th.centr}. In particular, the only difference is in the correction step, which is performed $s$ times. Therefore, we can modify Equation~\eqref{eq.fin_t_k} as
$$
\|\x_{k+1} - \x^*(t_{k+1})\| \leq \rho^s \sigma \|\x_{k} - \x^*(t_{k})\| + \rho^s O(h^2),
$$
or Equation~\eqref{eq.sampling_error2} as 
$$
\|\x_{k+1} - \x^*(t_{k+1})\| \leq \rho^s \|\x_{k} - \x^*(t_{k})\| + \rho^s O(h),
$$
and the rest follows almost verbatim. The last result on the numbers of correction steps $s$ to obtain a certain error level, can be obtained directly by solving the equation
$$
\frac{\rho^s}{1-\rho^s} = h^p,
$$ 
for $s$. 

\end{myproof} 
















%\section{Approximate Hessian inverse}\label{sec:hess}





==> Conclusion.tex <==
% !TEX root = TimeVarying_part1.tex
\section{Conclusion}\label{sec:conclusions}
%
We have designed algorithms to track the solution of time-varying unconstrained and strongly convex optimization problems. These algorithms leverage the knowledge of how the cost function changes in time and are based on a predictor-corrector scheme. We have also developed approximation schemes for when the rate at which the objective varies in time is not known. We established that these methods yield convergence to a neighborhood of the optimal trajectory, with a neighborhood of convergence dependent on the sampling period. Moreover, the size of this neighborhood is an order of magnitude smaller than state-of-the art running algorithms which only perform correction steps. In some cases when the problem parameters are appropriately chosen and second-order information is incorporated, the neighborhood of the optimal trajectory to which the algorithm converges is several orders of magnitude smaller than existing approaches. 

Moreover, we conducted a numerical analysis of the proposed methods in a simple setting which empirically supported the established error bounds. We also considered the task of developing a control strategy for an autonomous system to follow an object whose position varies continuously in time, showing that the developed tools yield an effective strategy. In some cases, the algorithms which achieve higher accuracy require\! too\! much\! computational latency to be used in a closed loop control setting; however, when this latency may be afforded, the second-order methods yield highly accurate tools.

Future research directions encompass the generalization of this work to constrained problems, general convex cost functions, as well as approximate second-order methods to weaken the computational requirements of computing the Hessian inverse in the prediction step.

==> Proofs_1.tex <==

% !TEX root = TimeVarying_part1.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\section{Proof of Proposition~\ref{prop.err}}\label{ap.prop}

For the forward Euler method applied to the nonlinear dynamical system
%%%
\begin{equation}\label{proof_100}
\dot{x} = {\mathcal{F}}(x,t),
\end{equation}
%%%
the local discretization error is bounded by~\cite[Chapter~11]{Quarteroni2000} $h^2/2\, \|\mathrm{d}\mathcal{F}(x,t)/\mathrm{d}t\|$. We can extend this result, by considering that the forward Euler method is based on a truncated Taylor series expansion. Let us analyze the forward Euler method applied to the vector-valued nonlinear dynamical system
%%%
\begin{equation}\label{proof_110}
\dot{\x} = {\mathbold{F}}(\x,t).
\end{equation}
%%%
If we apply the forward Euler method to the relation in \eqref{proof_110}, starting at a certain point $\x(t_k)$, we obtain 
%%%
\begin{equation}\label{proof_120}
\x_{k+1} = \x(t_k)+ {\mathbold{F}}(\x(t_k),t_k)\, h. 
\end{equation}
%%%
Subtracting $\x(t_{k+1})$ from the both sides of the equality in \eqref{proof_120} and computing the norm of the resulted relation implies that
%%%
\begin{equation}\label{proof_130} 
\|\x_{k+1} - \x(t_{k+1})\| =  \left\|{\mathbold{F}}(\x(t_k),t_k)\, h  -\int_{t_k}^{t_{k+1}} \!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau \right\|.
\end{equation}
%%%%%
Notice that \eqref{proof_130} is resulted by considering the relation $\x(t_{k+1}) = \x(t_{k}) +\int_{t_k}^{t_{k+1}} {\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau$. Observe that according to the Mean Value theorem there exits a $\hat{\tau} \in [t_k, t_{k+1}]$ that satisfies 
%%%
\begin{equation}\label{proof_140} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau = \int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(t_k),t_k) + \nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,h \, \textrm{d} \tau.
\end{equation}
%%%%%
Notice that the term ${\mathbold{F}}(\x(t_k),t_k)$ does not depend on the integral variable $\tau$. Considering this observation and observing the definition $h:=t_{k+1}-t_k$, we can simplify the first part of the integral in the right hand side of \eqref{proof_140} as 
%
\begin{equation}\label{proof_145} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(t_k),t_k)  \textrm{d} \tau= {\mathbold{F}}(\x(t_k),t_k) h \; .
\end{equation}
%
 Since $\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau})$ is also not a function of variable $\tau$,   by applying the same argument we can simplify the second part of the integral in the right hand side of \eqref{proof_140} as
 %
 \begin{equation}\label{proof_147} 
  \int_{t_k}^{t_{k+1}}\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,h \, \textrm{d} \tau=\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,(h^2)/2 \;.
  \end{equation}
   Therefore, we can rewrite \eqref{proof_140} as 
%%%
\begin{equation}\label{proof_150} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau = {\mathbold{F}}(\x(t_k),t_k)\ \!h + \nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,\frac{h^2}{2}.
\end{equation}
%%%%%
By substituting the integral $\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau$ in \eqref{proof_130} by the simplification in \eqref{proof_150} and considering the definition of the discretization error vector $\mathbold{\Delta}:=\x_{k+1} - \x(t_{k+1})$ we can rewrite \eqref{proof_130} as
%%%
\begin{equation}\label{proof_160} 
\|\mathbold{\Delta} \|=  \frac{h^2}{2} \|\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau})\|.
\end{equation}
%%%%%
Observing the continuous dynamical system in \eqref{eq.dyn} we know that ${\mathbold{F}}(\x,t)$ is given by
%%%
\begin{equation}\label{proof_170} 
{\mathbold{F}}(\x,t) = -[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t).
\end{equation}
%%%%%
We proceed to find an upper bound for the right hand side of \eqref{proof_160}. Note that based on the definition in \eqref{proof_170} we can write 
%%%
\begin{align}\label{proof_180} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|= \left\|\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]\right\|
\end{align}
%%%%%
Notice that by applying the chain rule we can simplify the derivative $\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]$ as
%%%
\begin{align}\label{proof_190} 
&\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]=\\
&\qquad\qquad\qquad[\nabla_{\x\x}f(\x; t)]^{-2} \nabla_{t \x\x}f(\x; t) \nabla_{t\x}f(\x; t)\nonumber\\
&
\qquad\qquad\qquad+ [\nabla_{\x\x}f(\x; t)]^{-1}\nabla_{tt\x}f(\x; t)\nonumber.
\end{align}
%%%%%
Compute the norm of both sides of \eqref{proof_190}. Substitute the norm $\|\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]\|$ by $\|\nabla_{t}{\mathbold{F}}(\x,t) \|$ as shown in \eqref{proof_180}. Further apply the triangle inequality to the right hand side of the resulted expression to obtain 
%%%
\begin{align}\label{proof_200} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|&\leq\left\|[\nabla_{\x\x}f(\x; t)]^{-2} \nabla_{t \x\x}f(\x; t) \nabla_{t\x}f(\x; t)\right\|\nonumber\\
&
\quad+ \left\|[\nabla_{\x\x}f(\x; t)]^{-1}\nabla_{tt\x}f(\x; t)\right\|.
\end{align}
%%%%%
Observe the fact that $\nabla_{t \x\x}f(\x; t) = \nabla_{\x t\x}f(\x; t)$. We use the Cauchy-Schwartz inequality and the bounds in Assumptions \ref{as.str} and  \ref{as.smooth} to update the upper bound in \eqref{proof_200} as
%%%
\begin{align}\label{proof_210} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|  \leq \frac{C_0 C_2}{m^2} + \frac{C_3}{m}
\end{align}
%%%%%
Combining the relation in \eqref{proof_160} and the upper bound in \eqref{proof_210} follows the claim in \eqref{prop_claim_err_bound}.
%%
\qed 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem \ref{th.GTT_convg}}\label{app.GTT_convg}


In order to prove Theorem \ref{th.GTT_convg}, we start by bounding the error in the prediction step by the terms that depend on the functional smoothness and the discretization error using Taylor expansions. Then we bound the tracking error of the gradient step using standard convergence properties of gradient descent on strongly convex functions. By substituting the error improvement achieved in the correction step into the prediction step, we establish the main result.

First, we establish that the criteria in which the bound stated in \eqref{result1} may be satisfied, i.e. that $\rho \sigma$ can be made strictly less than 1, for a sufficiently small $h$. Note that, since $m>0$, there is always a $\gamma$ that makes $\rho < 1$ since $\gamma < m/L^2$. In particular, if we take $\gamma = m/ 2 L^2$, then $\rho$ is minimized and it is equal to 
%
\begin{equation}\label{rho}
\rho^* = \sqrt{ 1 - \frac{m^2}{4 L^2}}. 
\end{equation}
%
The coefficient $\sigma$ is a monotonically increasing function in $h$, and it is equal to $1$ when $h = 0$; by continuity of $\sigma$ in $h$, we can always find a small enough stepsize $h$, such that $\sigma < 1/\rho^*$, which means that we can find a stepsize $\gamma$ that yields $\rho \sigma <1$.

Now we turn to establishing the discrete-time sampling error bound stated in \eqref{result1} is achieved by the updates \eqref{GTT_prediction}-\eqref{GTT_correction}. For simplicity, we modify the notation to omit the arguments $\x_k$ and $t_k$ of the function $f$. In particular, define 
%
\begin{align}\label{eq:thm1_defs}
&\nabla_{\x\x}f = \nabla_{\x\x}f(\x_k; t_k)\; , &&\nabla_{t\x} f = \nabla_{t\x} f(\x_k; t_k)\;,\nonumber \\ 
&\nabla_{\x\x}f^* = \nabla_{\x\x}f({\x}^*(t_{k}); t_k)\;,  && \nabla_{t\x} f^* = \nabla_{t\x} f({\x}^*(t_{k}); t_{k}) \; . \nonumber
\end{align}
%
Begin by considering the update~\eqref{GTT_prediction}, the prediction step, evaluated at a generic point $\x_k$ sampled at the current sample time $t_k$ and with associated optimizer $\x^*(t)$, which due to optimality will have null residual vector $\r(t) = \mathbf{0}$. Thus we may write
%
\begin{equation}\label{eq:null_residual}
\left\{\begin{array}{rcl}
{\x}_{k+1|k} &=& \x_{k} - [\nabla_{\x\x}f]^{-1}\nabla_{t\x} f\,h\\
{\x}^*(t_{k+1}) &=& {\x}^*(t_{k}) - [\nabla_{\x\x}f^*]^{-1} \nabla_{t\x} f^*\,h + \Delta.
\end{array}\right.
\end{equation}
%
By subtracting one from the other and by considering the norm of the result, we obtain 
%
\begin{align}\label{eq.imp}
\|{\x}_{k+1|k}& -  \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\|  \\  & + \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h + \|\mathbold{\Delta}\| .\nonumber 
\end{align}
%
Define $a$ as the second term in the right-hand side of \eqref{eq.imp}, as  $a= \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h$. We may rewrite $a$ by adding and subtracting the Newton step with the Hessian evaluated at the current optimal point,  $[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f$, to obtain
%
\begin{align}\label{eq.hessian_cross_term}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h,
\end{align}
%
We may bound the first and second-order derivative terms in the previous expression \eqref{eq.hessian_cross_term} by using Assumption~\ref{as.smooth} regarding the functional smoothness as well as the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} to write
%
\begin{equation}\label{eq.a}
a  \leq C_0 h \left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We now further bound the first term of the right-hand-side. To do that, we use the non-singularity of the Hessian to write 
%
\begin{multline}\label{eq.dummy10_midstep}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| = \\ \|[\nabla_{\x\x}f^*]^{-1}(\nabla_{\x\x}f - \nabla_{\x\x}f^*)[\nabla_{\x\x}f]^{-1} \|,
\end{multline} 
%
which by employing, once again, the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} we can bound as
\begin{equation}\label{eq.dummy10}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| \leq \frac{1}{m^2}\|\nabla_{\x\x}f - \nabla_{\x\x}f^* \|,
\end{equation} 
%
and therefore~\eqref{eq.a} can be written as
\begin{equation}\label{eq.amid}
a  \leq \frac{C_0}{m^2} h \left\|\nabla_{\x\x}f - \nabla_{\x\x}f^*\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We consider the Taylor expansion of the mixed second-order terms and the second-order terms in \eqref{eq.amid}, and apply the Mean Value Theorem with $\tilde{\x}$ as a point on the line between $\x_k$ and $\x^*(t_k)$ to obtain the following expressions,
%
%\begin{subequations}
\begin{align} \label{eq.dummy11}
\left\| \nabla_{\x\x} f- \nabla_{\x\x} f^*  \right\| &
\leq \left\|\nabla_{\x \x\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \nonumber\\ 
&\leq C_1 \|\x_k - \x^*(t_k)\| \\
%\end{multline}
%\begin{multline}
\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| &
\leq \left\|\nabla_{\x t\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \nonumber \\
& \leq C_2 \|\x_k - \x^*(t_k)\| \label{eq.dummy111}
\end{align}
%\end{subequations}
%
The expressions in \eqref{eq.dummy11} - \eqref{eq.dummy111} may be substituted together into~\eqref{eq.amid} to yield
 %
\begin{align}
a  &\leq \frac{C_0 C_1 h}{m^2}\|\x_k - \x^*(t_k)\| + \frac{C_2 h}{m}\|\x_k - \x^*(t_k)\|.
\end{align}
%
Now we can use this bound for $a$ in~\eqref{eq.imp} to get
%
\begin{align}\label{some_bound}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq&  \Big[1 + h\left(\frac{C_0 C_1 h}{m^2} + \frac{C_2 h}{m}\right) \Big] \times \nonumber \\
& \quad \|{\x}_{k} - \x^*(t_{k})\| + \|\mathbold{\Delta}\|.
\end{align}
%
By considering the definition of $\sigma$ in \eqref{thm:rho_sigma} and substituting the discretization error norm $\|\mathbold{\Delta}\|$ by its upper bound in \eqref{prop_claim_err_bound}, we obtain that
%
\begin{equation}\label{eq.fin1}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \sigma \|{\x}_{k} - \x^*(t_{k})\| + \frac{h^2}{2}\left[\frac{C_0 C_2}{m^2} + \frac{C_3}{m}\right] .
\end{equation}
%
For the correction step [cf. \eqref{GTT_correction}] , we may use the standard property of projected gradient descent for strongly convex functions. In particular, the gradient converges Q-linearly as
%
\begin{equation}\label{eq.fin2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\| \leq \rho \|{\hat{\x}}_{k+1}^{s} - \x^*(t_{k+1})\| .
\end{equation}
%
where $\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}$. To see this, it is sufficient to write the projected gradient step as 
\begin{multline}\label{eq.explanation1}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 = \\  \|P_X[{\hat{\x}}_{k+1}^{s} -\gamma \nabla_{\x} f(\hat{\x}_{k+1}^s; t_{k+1})] - \x^*(t_{k+1})\|^2 .
\end{multline}
Since $\x^*(t_{k+1}) = P_X[\x^*(t_{k+1})-\gamma\nabla_{\x} f(\x^*(t_{k+1}), t_{k+1})]$ for optimality, and since the projection is nonexpansive, we obtain 
\begin{multline}\label{eq.explanation2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 \leq  \|{\hat{\x}}_{k+1}^{s}  - \x^*(t_{k+1}) \\- \gamma (\nabla_{\x} f(\hat{\x}_{k+1}^s; t_{k+1}) - \nabla_{\x} f(\x^*(t_{k+1}), t_{k+1}) )\|^2 .
\end{multline}
By expanding the right-hand side and by the strong convexity and functional smoothness assumptions (Assumptions~\ref{as.str} and \ref{as.smooth}), we can write
\begin{equation}\label{eq.explanation2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 \! \leq \! (1+\gamma^2L^2-\gamma m)\|{\hat{\x}}_{k+1}^{s} - \x^*(t_{k+1})\|^2 .
\end{equation}
which is~\eqref{eq.fin2}. 
%see \cite{Nesterov2004} for further details. 
%
%
%
Observe that the sequence ${\hat{\x}}_{k+1}^{s}$ is initialized by the predicted variable $\x_{k+1|k}$ and the corrected variable $\x_{k+1}$ is equal to $ {\hat{\x}}_{k+1}^{\tau}$. Considering these observation and the relation in \eqref{eq.fin2} between two consecutive iterates of the sequence ${\hat{\x}}_{k+1}^{s}$ we can write 
%
\begin{equation}\label{eq.fin222}
\|{{\x}}_{k+1}- \x^*(t_{k+1})\| \leq \rho^\tau \|\x_{k+1|k} - \x^*(t_{k+1})\| .
\end{equation}
%
We are ready to consider the combined error bound achieved by the prediction-correction scheme. By plugging the correction error in \eqref{eq.fin222} into the prediction error in \eqref{eq.fin1} we obtain
%
\begin{equation}\label{eq.fin_t_k}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^\tau \sigma \|{\x}_{k} - \x^*(t_{k})\| +  \rho^\tau \Gamma,
\end{equation}
%
where $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$ is defined to simplify the notation. Notice that the relation between $\|{\x}_{k+1} - \x^*(t_{k+1})\|$ and $\|{\x}_{k} - \x^*(t_{k})\| $ in \eqref{eq.fin_t_k} is also holds true for $\|{\x}_{k} - \x^*(t_{k})\| $ and $\|{\x}_{k-1} - \x^*(t_{k-1})\| $. I.e., 
%
\begin{equation}\label{eq.fin_t_k_1}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^\tau \sigma \|{\x}_{k-1} - \x^*(t_{k-1})\| +  \rho^\tau \Gamma.
\end{equation}
%
Substituting the upper bound in \eqref{eq.fin_t_k_1} for $\|{\x}_{k} - \x^*(t_{k})\|$ into \eqref{eq.fin_t_k} implies an upper bound for $\|{\x}_{k+1} - \x^*(t_{k+1})\| $ in terms of the norm difference for time $k-1$ as
%
\begin{align}\label{eq.fin_t_k_new}
\|{\x}_{k+1} - \x^*(t_{k+1})\| &\leq (\rho^\tau \sigma)^2 \|{\x}_{k-1} - \x^*(t_{k-1})\|
\nonumber \\
& \qquad +\rho^\tau \Gamma(\rho^\tau \sigma+1) .
\end{align}
%
Now recursively apply the relationship \eqref{eq.fin_t_k} backwards in time to the initial time sample and use the same argument form \eqref{eq.fin_t_k} to \eqref{eq.fin_t_k_new} to write 
%
\begin{equation}\label{eq.fin_t_00}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq (\rho^\tau \sigma)^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \rho^\tau \Gamma \sum_{i=0}^k (\rho^\tau\sigma)^i.
\end{equation}
%
Substituting $k+1$ by $k$ and simplifying the sum in \eqref{eq.fin_t_00} leads to
%
\begin{equation}\label{eq.fin_t_0000}
\|{\x}_{k} - \x^*(t_{k})\| \leq (\rho^\tau \sigma)^{k} \|{\x}_{0} - \x^*(t_{0})\| + \rho^\tau \Gamma \left[ \frac{1-(\rho^\tau\sigma)^k}{1-\rho^\tau\sigma}\right].
\end{equation}
%
Considering the result in \eqref{eq.fin_t_0000} and the definition for the constant $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$, the result in \eqref{result1} follows.

To establish the result stated in \eqref{result2}, observe that in the worst case, we may upper bound the term $a$ in \eqref{eq.amid} by using the bounds in Assumption \ref{as.smooth} to obtain the right hand side of the following expression 
%
\begin{align}\label{eq.worst_case}
a  
 & \leq \frac{2 C_0 L h}{m^2} + \frac{2 C_0 h}{m}.
\end{align}
%
Remembering the definition of the nonnegative scalar term $a:=\left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h $ and substituting the bound~\eqref{eq.worst_case} into \eqref{eq.imp}, we can write
%
\begin{multline}\label{eq.a_subst}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\| \\ + h\left(\frac{2 C_0 L }{m^2} + \frac{2 C_0 }{m}\right) +  \|\mathbold{\Delta}\|.
\end{multline}
%
To simplify the notation we define a new constant $\Gamma_2:= h\left(({2 C_0 L }/{m^2} )+ ({2 C_0 }/{m})\right)$. Considering this definition and observing the  the relation in \eqref{eq.fin222} we can write 
%
\begin{equation}\label{eq.sampling_error2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^\tau \|{\x}_{k} - \x^*(t_{k})\| + \rho^\tau (\Gamma_2 + \Gamma).
\end{equation}
%
%
Now recursively apply the relationship \eqref{eq.sampling_error2} backwards in time to the initial time sample and use the same argument form \eqref{eq.fin_t_k} to \eqref{eq.fin_t_0000} to write 
%
\begin{multline}\label{eq.rho_error_dependence}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^{\tau(k+1)} \|{\x}_{0} - \x^*(t_{0})\| \\ +  \rho^\tau (\Gamma_2 + \Gamma) \left[ \frac{1-\rho^{\tau (k+1)}}{1-\rho^\tau}\right].
\end{multline}
%
Note that relation \eqref{eq.rho_error_dependence} shows an upper bound for $\|{\x}_{k+1} - \x^*(t_{k+1})\|$ in terms of the initial error $\|{\x}_{0} - \x^*(t_{0})\|$ and an extra error term for the bound of convergence. If we substitute $k+1$ by $k$ in \eqref{eq.rho_error_dependence} and recall the definition $\Gamma_2:= h\left(({2 C_0 L }/{m^2} )+ ({2 C_0 }/{m})\right)$ and $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$, then the result in \eqref{result2} follows.
%%
\qed

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem~\ref{th.NTT_convg} }\label{ap.newton}

We consider once again the proof of Theorem~\ref{th.GTT_convg}, in particular Equation~\eqref{some_bound} for $k = 0$, due to the prediction step. For the correction step, if we applied one time the Newton step, we would have that
\begin{equation}\label{eq.dummy300}
\|\x_{1} - \x^*(t_{1})\| \leq  (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \frac{\gamma C_1}{2 m} \|\x_{1|0} - \x^*(t_{1})\|^2.
\end{equation}
The reason for~\eqref{eq.dummy300} is explained as follows: Define
\begin{align}%\label{eq:thm1_defs2}
&\nabla_{\x\x}f_1 = \nabla_{\x\x}f(\x_{1|0}; t_1)\; , &&\nabla_{\x} f_1 = \nabla_{\x} f(\x_{1|0}; t_1)\;,\nonumber \\ 
&\nabla_{\x\x}f^*_1 = \nabla_{\x\x}f({\x}^*(t_{1}); t_1)\;,  && \nabla_{\x} f^*_1 = \nabla_{\x} f({\x}^*(t_{1}); t_{1}) \; . \nonumber
\end{align}
We can write, by applying one Newton step
\begin{align}
\|\x_{1} - \x^*(t_{1})\| &=  \|P_X[\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1]- \x^*(t_{1})\| \nonumber \\
& = \|P_X[\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1]- P_X[\x^*(t_{1})]\| \nonumber \\
& \leq \|\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1- \x^*(t_{1})\|, \label{eq.aryan1}
\end{align}
where we have used the fact that $\x^*(t_{1}) \in X$ and the nonexpansive property of the projection. We can now expand the right-hand side of~\eqref{eq.aryan1} as
\begin{equation}\label{eq.aryan2}
(1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma\|\x_{1|0} - \x^*(t_{1}) - \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1\|,
\end{equation}
which can be further upper bounded as 
\begin{align}
\eqref{eq.aryan2} & \leq (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma\|\nabla_{\x\x}f_1^{-1}\|\times \nonumber \\ &\qquad\qquad\qquad\|\nabla_{\x\x}f_1(\x_{1|0} - \x^*(t_{1})) - \nabla_{\x}f_1\| \nonumber \\ 
&\leq (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma \frac{C_1}{2 m}\| \x_{1|0} - \x^*(t_{1})\|^2,\label{eq.aryan3}
\end{align}

\textbf{Maybe expand this one!}

where the last inequality comes from the Assumption~\ref{as.smooth}, and in particular the Lipschitz continuity of the Hessian~[cfr.~\cite[Chapter~1]{Nesterov2004}]. By plugging the bound~\eqref{eq.aryan3} into~\eqref{eq.aryan1} the claim~\eqref{eq.dummy300} follows. 

Consider now $\gamma = 1$ and multiple Newton steps: we have,
\begin{equation}\label{eq.dummy30}
\|\x_{1} - \x^*(t_{1})\| \leq  \left(\frac{C_1}{2 m}\right)^{2\tau - 1}\hskip-2mm \left(\|\x_{1|0} - \x^*(t_{1})\|\right)^{2 \tau}.
\end{equation}
In order to ease the notation, we define $p_k$ as $\|\x_{k} - \x^*(t_{k})\|$ and $q = 2\tau -1$. By substituting~\eqref{eq.dummy30} into the bound on the predictions step~\eqref{some_bound}, we obtain, 
\begin{equation}\label{eq.dummy31}
p_1 \leq \left(\frac{C_1}{2 m}\right)^q  \left(\sigma p_0 + \|\mathbold{\Delta}\| \right)^{2\tau}.
\end{equation}
Due to strong convexity and Lipschitz continuity of the gradient (Assumptions~\ref{as.str} and \ref{as.smooth}), and the fact that at optimality the gradient vanishes, we can write
\begin{align}
\|\nabla_x f(\x_0, t_0)\| &= \|\nabla_x f(\x_0, t_0) - \nabla_x f^*_0\| \nonumber \\&\hspace*{-1.5cm}\geq (\nabla_x f(\x_0, t_0) - \nabla_x f^*_0)^\transp(\x_{0} - \x^*(t_0))/\|\x_{0} - \x^*(t_0)\| \nonumber \\  &\geq  m \|\x_{0} - \x^*(t_0)\|, 
\end{align}
\begin{equation}
\|\nabla_x f(\x_1, t_1)\| = \|\nabla_x f(\x_1, t_1) - \nabla_x f^*_1\| \leq L \|\x_{1} - \x^*(t_1)\|.
\end{equation}
Calling.. , due to , the inequality~\eqref{eq.dummy31} implies, 
\begin{equation}\label{eq.dummy31aryan}
g_1 \leq \frac{1}{L}\,\left(\frac{C_1}{2 m}\right)^q  \left(\sigma/m \,g_0 + \|\mathbold{\Delta}\| \right)^{2\tau}.
\end{equation}
and by recalling that by the local convergence hypothesis we have $g_0 \leq \beta\|\mathbold{\Delta}\|$, then
\begin{equation}\label{eq.dummy32}
g_1 \leq  \frac{1}{L} \left(\frac{C_1}{2 m}\right)^{q} \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau}.
\end{equation}

To enforce convergence of the sequence $\{g_k\}$, we need first to make sure that $g_1 \leq g_0$:
\begin{equation}\label{eq.dummy33}
\frac{1}{L}\left(\frac{C_1}{2 m}\right)^{q} \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau} \leq g_0 \leq \beta \|\mathbold{\Delta}\|,
\end{equation}
which yields
\begin{equation}\label{eq.dummy34}
\frac{C_1}{2 m}\|\mathbold{\Delta}\| \leq  \frac{(\beta\, L) ^{1/q}}{\left(\sigma/m\, \beta + 1 \right)^{2\tau/q}}.
\end{equation}
If condition~\eqref{eq.dummy34} is satisfied, then $g_1 \leq g_0$. By induction on $g_k$, one can show that under~\eqref{eq.dummy34}, it is also true that 
\begin{equation}\label{eq.dummy35}
g_k \leq \beta\,\|\mathbold{\Delta}\|, \quad \text{ for all } k\geq 1,
\end{equation}
or, by using again the strong convexity assumption
\begin{equation}\label{eq.dummy35}
p_k \leq g_k/m \leq \beta/m\,\|\mathbold{\Delta}\|, \quad \text{ for all } k\geq 1,
\end{equation}
which is the claim~\eqref{..}.

If we want to make sure to have a smaller asymptotical error (and quadratic convergence of the Newton method), then we need to change~\eqref{eq.dummy33} and enforce
\begin{equation}\label{eq.dummy36}
\frac{1}{L}\left(\frac{C_1}{2 m}\right)^{2\tau - 1}\hskip-2mm \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau} \leq \beta \|\mathbold{\Delta}\|^{2\tau}.
\end{equation}
Since $\|\mathbold{\Delta}\| \leq 1$ this condition is stronger than~\eqref{eq.dummy33} and implies $g_1 \leq g_0$. By solving~\eqref{eq.dummy36}, we obtain the condition:
\begin{equation}\label{eq.dummy37}
\left(\frac{C_1}{2 m}\right)^{q}  \leq \frac{\beta L}{\left(\sigma \beta + 1 \right)^{2\tau}},
\end{equation}
In particular, if this condition is satisfied then, 
\begin{equation}\label{eq.dummy38}
p_k \leq g_k/m \leq \beta/m \,\|\mathbold{\Delta}\|^{2\tau}, \quad \text{ for all } k\geq 1.
\end{equation}
%%%
which is . 
\qed


\section{Proof of Theorem~\ref{th.AGT_convg} }\label{ap.agt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     P  R   O  O   F    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We prove Theorem~\ref{th.AGT_convg} by evaluating the extra error term coming from the approximate time derivative in~\eqref{fobd}. In particular, by Taylor expansion, one can see that
\begin{equation}\label{appder_oh}
\|\tilde{\nabla}_{t\x}{f}_k  - {\nabla}_{t\x}{f}(\x_k; t_k)\| = O(h),  
\end{equation} 
In fact, one Taylor expands
\begin{align}
{\nabla}_{\x}{f}(\x_{k-1}; t_{k-1})  =& {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h \nonumber \\
& \quad + {\nabla}_{tt\x}{f}(\x(\tau); \tau) {h^2}/{2},
\end{align} 
for a particular choice of $\tau\in[t_{k-1}, t_k]$. By solving for ${\nabla}_{t\x}{f}(\x_k; t_k)$, 
\begin{align}
{\nabla}_{t\x}{f}(\x_k; t_k) = \frac{1}{h} ( {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h \nonumber \\
 + {\nabla}_{tt\x}{f}(\x(\tau); \tau) {h^2}/{2}).
\end{align}
By substituting this result and the definition~\eqref{fobd} into~\eqref{appder_oh}, the $O(h)$ error bound is proven. 

Consider now the approximate prediction step, 
\begin{equation}
\x_{k+1|k} = \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h,
\end{equation}
which by adding and subtracting the exact prediction direction becomes, 
\begin{align}
\x_{k+1|k} &= \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h + \nonumber \\ 
&\quad 
+[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h  \nonumber \\ 
&\quad - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h.
\end{align}
By following the same steps as in Theorem~\ref{th.GTT_convg}, the term $a$ in Equation~\eqref{eq.hessian_cross_term} can be written with an extra error term as, 
\begin{align}\label{eq.hessian_cross_term_2}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\
 &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h \nonumber \\ &\quad + \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h.
\end{align}
%
The extra error term w.r.t. Equation~\eqref{eq.hessian_cross_term} can be further bounded by using~\eqref{appder_oh} and the smoothness Assumption~\ref{as.smooth} (with the strong convexity constrant $m$)
\begin{align}\label{dummy_101}
& \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h  \nonumber\\
&\quad \leq \|[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1}\| \| {\nabla}_{t\x}{f}(\x_k; t_k)  - \tilde{\nabla}_{t\x}{f}_k \| \, h  \nonumber\\
&\quad \leq \frac{1}{m} \|{\nabla}_{tt\x}{f}(\x(\tau); \tau) {h}/{2}\| \, h = \frac{C_3}{m}\,\frac{h^2}{2}.
\end{align}
By adding this extra error term in the bounds~\eqref{some_bound} and \eqref{eq.a_subst} and proceeding in similar fashion as in the proof of Theorem~\ref{th.GTT_convg}, claims~\eqref{result2a} and \eqref{result1a} can be easily proven. 
%
\qed

\section{Proof of Theorem~\ref{th.ANT_convg} }\label{ap.ant}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     P  R   O  O   F    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The proof of Theorem~\ref{th.ANT_convg} is based on the proof of Theorems~\ref{th.NTT_convg} and \ref{th.AGT_convg}. In particular, the use of an approximate time derivative yields an additional error term equivalent to $({C_3}/{m})\,({h^2}/{2})$ as shown in~\eqref{dummy_101}. This means that~\eqref{eq.dummy31} will now read
\begin{align}
p_1 &\leq \left(\frac{C_1}{2 m}\right)^{q} \left(\sigma p_0 + \|\mathbold{\Delta}\| + \frac{C_3}{m}\,\frac{h^2}{2} \right)^{2\tau} \nonumber \\
 &= \left(\frac{C_1}{2 m}\right)^q (\sigma p_0 + D)^{2\tau} \; ,
\end{align}
where we have used the definition of the cumulative error $D$. The rest follows as in the proof of Theorem~\ref{th.NTT_convg}.
%
\qed


==> arXiv Version 2/Algorithm.tex <==
% !TEX root = TimeVarying_part1.tex
\section{Centralized algorithm}\label{sec:centr}

We first focus on centralized algorithms, i.e., algorithms that assume that the computations are performed by a unique computing entity. In order to converge to the solution trajectory $\x^*(t)$, we will generate a sequence of near optimal decision variables $\{\x_k\}$ by taking into account both how the solution changes in time and how different our current update is from the optimizer at each time step. To do this, we set up a prediction-correction scheme, much like a Kalman filter strategy in estimation theory. In the first step, we will predict how the solution changes, and in the correction step we will do one step of gradient or Newton method towards the optimizer at that time instance. As mentioned in the Introduction, we call this strategy \emph{solution tracking}, to contrast it with standard \emph{running} algorithms that do not predict how the solution changes, but only adapt to it. 

\subsection{Prediction step}

To generate the prediction step, we reformulate the time-varying problem~\eqref{eq.problem} in terms of optimality conditions. Solving~\eqref{eq.problem} means to compute the solution of the following nonlinear system of equations
\begin{equation}
\nabla_{\x} f(\x^*(t); t) = \mathbf{0}, 
\end{equation}
for each $t$. For any other vector $\x$ (for example the approximate solution $\x_k$), we can write 
\begin{equation}\label{eq.isoerror}
\nabla_{\x} f(\x; t) = \r(t)
\end{equation}
where $\r(t)$ is some residual error. The aim of the prediction step is to keep this residual error as much fixed as possible while the optimization problem is changing. To say it in another way, we want to predict how to update $\x_k$ such that we stay close to the iso-residual manifold.  We can see how such trajectory evolves by perturbing it as
\begin{equation}
\nabla_{\x} f(\x; t) + \nabla_{\x\x} f(\x; t) \delta\x + \nabla_{t\x} f(\x; t) \delta t = \r(t),  
\end{equation}
and by using~\eqref{eq.isoerror} and by dividing it by $\delta t \neq 0$, we obtain the continuous dynamical system
\begin{equation}\label{eq.dyn}
\dot{\x} = - [\nabla_{\x\x} f(\x; t)]^{-1} \nabla_{t\x} f(\x; t). 
\end{equation}
By passing now in the discrete domain (where our algorithm will live), we sample the problem at sampling times $t_k$, for $k = 0,1,2,\dots$, and for the sake of simplicity we let this sampling be uniform, with sampling interval equal to $h$. We can integrate~\eqref{eq.dyn} by using a first-order forward Euler scheme as   
\begin{multline}\label{eq.up}
{\x}(t_{k+1}) = \x(t_{k}) - [\nabla_{\x\x} f(\x(t_k); t_k)]^{-1} \nabla_{t\x} f(\x(t_k); t_k) \, h \\ + \Delta,
\end{multline}
where $\Delta$ represents the discretization error. The discretization error can be upper bounded as follows. 

\begin{proposition}\label{prop.err}
Under Assumptions~\ref{as.0}, \ref{as.str}, and \ref{as.smooth}, the discretization error $\Delta$ of the Euler method~\eqref{eq.up} w.r.t. the real dynamics~\eqref{eq.dyn} is upper bounded by
$$
\Delta \leq \frac{h^2}{2}\left[\frac{C_0 C_2}{m^2} + \frac{C_3}{m}\right] = O(h^2).
$$
\end{proposition}
\vskip2mm

\begin{proof}
See Appendix~\ref{ap.prop}.
\end{proof}
\vskip2mm

Proposition~\ref{prop.err} says that under our assumptions we can use the Euler method. We will forget for the moment of the constant in the discretization error and live with its order in $h$ only. We can use the update rule~\eqref{eq.up} as the basics of our prediction step. Let ${\x}_{k+1|k}$ be the predicted decision variable vector; this will be computed as
\begin{equation}\label{eq:update}
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h.
\end{equation}


\subsection{Correction step}

The correction step can be devised by using, for example, a constant stepsize  projected gradient method based on the updated objective function at time $t_{k+1}$
\begin{equation}\label{eq.corr}
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \gamma \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})],
\end{equation}
for a choice of stepsize $\gamma > 0$, and where $P_{X}$ is the projection operator. Another way to design the correction step would be to use projected Newton's method; we will see how to perform that in Section~\ref{sec:newton}.  


{\color{green} [Here some words on the algorithm!]}


\subsection{Convergence analysis}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Centralized solution tracking (gradient-based)}
\label{alg.centr}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h
$$
\textbf{2:} Correction step:
$$
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \gamma \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})]
$$ 
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%

In Algorithm~\ref{alg.centr}, we summarize the devised centralized algorithm, whose convergence is encoded in the following theorem. 

\begin{theorem}\label{th.centr}
Let Assumption~\ref{as.0}, \ref{as.str}, and \ref{as.smooth} hold and let $\{\x_k\}$ be the sequence generated by Algorithm~\ref{alg.centr}. Define the rates $\rho$ and $\sigma$ as
%
\begin{equation}\label{thm:rho_sigma}
\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}, \quad \sigma = 1 + h(C_0 C_1/m^2 + C_2/m).
\end{equation}
%
\begin{enumerate}
\item If the sampling interval $h$ is chosen sufficiently small, then there exists a $\gamma>0$ for which 
\begin{equation*}
\rho \sigma < 1
\end{equation*}
and, in this case, convergence of $\{\x_k\}$ to $\x^*(t_k)$ is Q-linear up to a bounded error as,
\begin{equation}\label{result1}
\|{\x}_{k} - \x^*(t_{k})\| \leq (\rho \sigma)^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h^2).
\end{equation}
\item Irrespectively of the selection of $h$, if we pick $\gamma < m/L^2$, then convergence goes as   
\begin{equation}\label{result2}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h).
\end{equation}
\end{enumerate} 
\end{theorem}
%
\vskip2mm
\begin{myproof}

In order to prove Theorem~\ref{th.centr}, we start by bounding the error in the prediction step by terms that depend on the functional smoothness and the discretization error using Taylor expansions. Then we bound the tracking error of the gradient step using standard convergence properties of gradient descent on strongly convex functions. By substituting the error improvement achieved in the correction step into the prediction step, we establish the main result.

First, we establish that the criteria in which the bound stated in \eqref{result1} may be satisfied, i.e. that $\rho \sigma$ can be made strictly less than one, for a sufficiently small $h$. Note that, since $m>0$, there is always a $\gamma$ that makes $\rho < 1$ since $\gamma < m/L^2$. In particular, if we take $\gamma = m/ 2 L^2$, then $\rho$ is minimized and it is equal to 
%
\begin{equation}\label{rho}
\rho^* = \sqrt{ 1 - \frac{m^2}{4 L^2}}. 
\end{equation}
%
The coefficient $\sigma$ is a monotonically increasing function in $h$, and it is equal to $1$ when $h = 0$; by continuity of $\sigma$ in $h$, we can always find a small enough stepsize $h$, such that $\sigma < 1/\rho^*$, which means that we can find a stepsize $\gamma$ that yields $\rho \sigma <1$.

Now we turn to establishing the discrete-time sampling error bound stated in \eqref{result1} is achieved by the updates \eqref{eq:update}-\eqref{eq.corr}. For simplicity, we modify the notation to omit the arguments $\x_k$ and $t_k$ of the function $f$. In particular, define $\nabla_{\x\x}f = \nabla_{\x\x}f(\x_k; t_k)$, $\nabla_{t\x} f = \nabla_{t\x} f(\x_k; t_k)$, $\nabla_{\x\x}f^* = \nabla_{\x\x}f({\x}^*(t_{k}); t_k)$, and $\nabla_{t\x} f^* = \nabla_{t\x} f({\x}^*(t_{k}); t_{k})$. 

Begin by considering the update~\eqref{eq:update}, the prediction step, evaluated at a generic point $\x_k$ sampled at the current sample time $t_k$ and with associated optimizer $\x^*(t)$, which due to optimality will have null residual vector $\r(t) = \mathbf{0}$. Thus we may write
%
\begin{equation*}\left\{\begin{array}{rcl}
{\x}_{k+1|k} &=& \x_{k} - [\nabla_{\x\x}f]^{-1}\nabla_{t\x} f\,h\\
{\x}^*(t_{k+1}) &=& {\x}^*(t_{k}) - [\nabla_{\x\x}f^*]^{-1} \nabla_{t\x} f^*\,h + O(h^2).
\end{array}\right.
\end{equation*}
%
By subtracting one from the other and by considering the norm of the result, we obtain 
%
\begin{align}\label{eq.imp}
\|{\x}_{k+1|k}& -  \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\|  \\  & + \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h + O(h^2) .\nonumber 
\end{align}
%
Set the second term in the right-hand side of \eqref{eq.imp} as  $a= \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h$. We may rewrite $a$ by adding and subtracting the Newton step with the Hessian evaluated at the current optimal point,  $[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f$, to obtain
%
\begin{align}\label{eq.hessian_cross_term}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h,
\end{align}
%
We may bound the first and second-order derivative terms in the previous expression \eqref{eq.hessian_cross_term} by using Assumption~\ref{as.smooth} regarding the functional smoothness as well as the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} to write
%
\begin{equation}\label{eq.a}
a  \leq C_0 h \left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We now further bound the first term of the right-hand-side. To do that, we use the non-singularity of the Hessian to write 
%
\begin{multline}\label{eq.dummy10_midstep}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| = \\ \|[\nabla_{\x\x}f^*]^{-1}(\nabla_{\x\x}f - \nabla_{\x\x}f^*)[\nabla_{\x\x}f]^{-1} \|,
\end{multline} 
%
which by employing, once again, the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} we can bound as
\begin{equation}\label{eq.dummy10}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| \leq \frac{1}{m^2}\|\nabla_{\x\x}f - \nabla_{\x\x}f^* \|,
\end{equation} 
%
and therefore~\eqref{eq.a} can be written as
\begin{equation}\label{eq.amid}
a  \leq \frac{C_0}{m^2} h \left\|\nabla_{\x\x}f - \nabla_{\x\x}f^*\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We consider the Taylor expansion of the mixed second-order terms and the second-order terms in \eqref{eq.amid}, and apply the Mean Value Theorem with $\tilde{\x}$ as a point on the line between $\x_k$ and $\x^*(t_k)$ to obtain the following expressions,
%
\begin{subequations}\label{eq.dummy11}
\begin{multline}
\left\| \nabla_{\x\x} f- \nabla_{\x\x} f^*  \right\| \leq \left\|\nabla_{\x \x\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \\ \leq C_1 \|\x_k - \x^*(t_k)\|
\end{multline}
\begin{multline}
\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| \leq \left\|\nabla_{\x t\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \\ \leq C_2 \|\x_k - \x^*(t_k)\|
\end{multline}
\end{subequations}
%
The expressions in \eqref{eq.dummy11} may be substituted together into~\eqref{eq.amid} to yield
 %
\begin{align}
a  &\leq \frac{C_0 C_1 h}{m^2}\|\x_k - \x^*(t_k)\| + \frac{C_2 h}{m}\|\x_k - \x^*(t_k)\|.
\end{align}
%
Now we can use this bound for $a$ in~\eqref{eq.imp} to get
%
\begin{multline*}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \\ \Big[1 + h\left(\frac{C_0 C_1 h}{m^2} + \frac{C_2 h}{m}\right) \Big]\|{\x}_{k} - \x^*(t_{k})\| + O(h^2).
\end{multline*}
%
which, by the definition of $\sigma$ as stated in \eqref{thm:rho_sigma} in Theorem \ref{th.centr}, allows us to conclude
%
\begin{equation}\label{eq.fin1}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \sigma \|{\x}_{k} - \x^*(t_{k})\| + O(h^2).
\end{equation}
%
For the correction step [cf. \eqref{eq.corr}] , we may use the standard property of projected gradient descent for strongly convex functions. In particular, the gradient converges Q-linearly as
%
\begin{equation}\label{eq.fin2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \|{\x}_{k+1|k} - \x^*(t_{k+1})\|
\end{equation}
%
where $\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}$, see \cite{Nesterov2004} for further details.
%
%\subsection{Total algorithm}

We are ready to consider the combined error bound achieved by the prediction-correction scheme. By plugging the correction error \eqref{eq.fin2} into the prediction error \eqref{eq.fin1} we obtain
%
\begin{equation}\label{eq.fin_t_k}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \sigma \|{\x}_{k} - \x^*(t_{k})\| + \rho O(h^2).
\end{equation}
%
Now recursively apply the relationship \eqref{eq.fin_t_k} backwards in time to the initial time sample at $t_0$ to write
%
\begin{equation*}\label{eq.fin_t_0}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq (\rho \sigma)^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h^2),
\end{equation*}
%
which is the result \eqref{result1} in Theorem \ref{th.centr}.

To establish the result stated in \eqref{result2} of Theorem \ref{th.centr}, observe that in the worst case, we may upper bound the term $a$ in \eqref{eq.amid} by using the bounds in Assumption \ref{as.smooth} to obtain the right hand side of the following expression 
%
\begin{align}\label{eq.worst_case}
a  & \leq  \frac{C_0 h}{m^2}
 \|\nabla_{\x\x}f - \nabla_{\x\x}f^*\| 
 + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| \nonumber\\
 & \leq \frac{2 C_0 L h}{m^2} + \frac{2 C_0 h}{m} = O(h),
\end{align}
%
Remembering the definition of the nonnegative scalar term $a=\left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h $ and substituting the bound~\eqref{eq.worst_case} into \eqref{eq.imp}, we can write
%
\begin{equation}\label{eq.a_subst}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\| + O(h).
\end{equation}
%
This, together with the contraction property of the gradient step as stated in \eqref{eq.fin2} yields
%
\begin{equation}\label{eq.sampling_error2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \|{\x}_{k} - \x^*(t_{k})\| + \rho O(h).
\end{equation}
%
If we iterate the expression \eqref{eq.sampling_error2} backwards in time to the initial point ${\x}_{0}$, we obtain
%
\begin{equation}\label{eq.rho_error_dependence}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h),
\end{equation}
%
which is~\eqref{result2}. With $\rho= \sqrt{1 + \gamma^2 L^2 - \gamma m}$ as defined in \eqref{thm:rho_sigma}, we only need to find a $\gamma$ that makes $\rho < 1$. Selecting any $\gamma$  satisfying $\gamma < m/L^2 $ concludes the proof.

\end{myproof}


\vskip2mm
\begin{corollary}\label{co.centr}
Under the same conditions of Theorem~\ref{th.centr},
\begin{enumerate}
\item If we pick $\gamma = m/2 L^2$, then the convergence bounded error is between $O(h)$ and $O(h^2)$. 
\item If we do not perform the prediction step in Algorithm~\ref{alg.centr} but only the correction step (i.e., we use Algorithm~\ref{alg.centr} as a running algorithm), then, if we pick $\gamma < m/L^2$, convergence goes as 
\begin{equation*}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h).
\end{equation*}
\end{enumerate}
\end{corollary}
%
\vskip2mm
\begin{myproof}

Point 1) follows from the proof of Theorem~\ref{th.centr}. In fact, if we select $\gamma = m/2 L^2$ then we minimize $\rho$ (as stated in~\eqref{rho}). Therefore, with this selection of $\gamma$, two cases are possible. 

The first case is that $h$ is small enough, such that $\rho \sigma < 1$. Here, we can use the first part of Theorem~\ref{th.centr} and, in particular, Equation~\eqref{result1}, which brings a bounded error of size $O(h^2)$. 

The second case is that $h$ is not small enough, such that $\rho \sigma \geq 1$. Here, we can use the second part of Theorem~\ref{th.centr}, i.e., Equation~\eqref{result2}, to bound the asymptotical error to $O(h)$. 

By putting together the two cases, the claim of Point 1) follows. 

Point 2) also follows directly from the proof of Theorem~\ref{th.centr}. Suppose that we execute the correction step \eqref{eq.corr} without the prediction step \eqref{eq:update}. Such an update would be equivalent to performing the updates \eqref{eq:update}-\eqref{eq.corr} with the prediction step evaluated at $\nabla_{t\x} f = {\bf{0}}$. Substituting this case into \eqref{eq.imp} yields
\begin{align*}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| &\leq \|{\x}_{k} - \x^*(t_{k})\| \\
 & \qquad + \left\|[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h 
	+ O(h^2) \\ 
	&\leq \|{\x}_{k} - \x^*(t_{k})\| + \frac{C_0 h}{m} + O(h^2) \\
	 & \leq \|{\x}_{k} - \x^*(t_{k})\| + O(h),
\end{align*}
%
where we have bounded the magnitude of the Hessian and the derivative mixed first order derivative terms using Assumptions \ref{as.str}-\ref{as.smooth}, respectively. From here, the analysis proceeds exactly as from \eqref{eq.a_subst} to the conclusion of 2) in Theorem~\ref{th.centr}, yielding \eqref{eq.rho_error_dependence}, which concludes the proof. 

\end{myproof}

\vskip2mm
Theorem~\ref{th.centr} says that our tracking algorithm generates a converging sequence of approximate solutions and the error bound depends (at worst) linearly on the sampling interval. Convergence is quite fast (in fact Q-linear), as one would expect in strongly convex problems. Corollary~\ref{co.centr} confirms our intuition that performing the prediction step improves upon state-of-the-art running algorithms (passing from an error bound of $O(h)$ to $O(h^2)$ if $h$ is chosen small enough). 


\begin{remark}\label{rem.k}
We can readily extend the results on this section and the following one when the constant $C_0, C_1, C_2, m, L$ are constant in the decision variable $\x$ but not uniformly in time. In order to do that, we have to substitute these constants by other ones, depending on the sampled time instance $t_k$ as $C_{0,k}, C_{1,k}, C_{2,k}, m_k, L_k$. With this substitution, all the results hold true (with minor modifications) and in particular the stepsize $\gamma$ can be chosen to vary from $k$ to $k+1$. 
\end{remark}


\section{Newton correction}\label{sec:newton}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Centralized solution tracking (Newton-based)}
\label{alg.newton}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h.
$$
\textbf{2:} Correction step:
\begin{multline*}
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \\ [\nabla_{\x\x} f(\x_{k+1|k}; t_{k+1})]^{-1} \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})]
\end{multline*}
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%
In this section, we explore the possibility of using a Newton's step for the correction step in Algorithm~\ref{alg.centr}. We want to see if substituting~\eqref{eq.corr} with 
\begin{multline}
{\x}_{k+1} = \x_{k+1|k} - [\nabla_{\x\x} f(\x_{k+1|k}; t_{k+1})]^{-1}\times\\ \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})
\end{multline}
yields a further decrease in the asymptotic error from $O(h^2)$ to something smaller than that. Intuitionally that should be the case, since Newton's method has local quadratic convergence, so we expect to reduce $O(h^2)$ to a $O(h^4)$ error. In this section, we will prove that this is not in general the case, which undermines the usefulness of a Newton's correction step in time-varying problems. 


In particular, we analyze the local convergence of Algorithm~\ref{alg.newton}. 

\begin{theorem}\label{th.newton}
Let Assumptions~\ref{as.0}, \ref{as.str}, and \ref{as.smooth} hold true. Suppose the initial guess $\x_0$ is picked close enough to the initial optimizer, i.e., the norm $\|\x_0 - \x^*(t_0)\| \leq \alpha h^2 /2$, with $\alpha h^2 /2 \ll 1$. Define the parameter $\alpha' = [C_0 C_2/ m^2 + C_3/m]$, so that the Euler discretization error $\Delta$ in Proposition~\ref{prop.err} has the worst case value of $\Delta = \alpha' h^2/2$. In addition, suppose that this worst case value is small enough, i.e., $\alpha' h^2/2 \ll 1$. With this in place, for the sequence $\{\x_k\}$ generated by Algorithm~\ref{alg.newton} we have for all $k>1$
\begin{enumerate}
\item if $C_1/2 m \leq 2\alpha/[(\alpha + \alpha')^2\, h^2]$, then 
$$
\|\x_k - \x^*(t_k)\| \leq O(h^2),
$$
\item if, in addition, $C_1/2 m \leq 1$, then 
$$
\|\x_k - \x^*(t_k)\| \leq O(h^4).
$$
\end{enumerate}
\end{theorem}
\vskip2mm

\begin{proof}
See Appendix~\ref{ap.newton}. 
\end{proof}
\vskip2mm

Theorem~\ref{th.newton} says that, in general, if we select $h$ small enough, we can track the optimizer $\x^*(t_k)$ at worst with a $O(h^2)$ error bound. This is very similar to the result we had for the gradient-based tracking algorithm. In special cases, when $C_1/2m \leq 1$, then the quadratic convergence of the Newton's method appears and we track the optimizer at worst with a error bound of $O(h^4)$. A special case of the second situation are quadratic cost functions, for which $C_1 = 0$, and we have perfect convergence. 

%We will see in the simulation results in Section~\ref{sec:num} that, in practice, since both $C_1$ and $m$ vary in time, Algorithm~\ref{alg.newton} generates a sequence that oscillates between a $O(h^2)$ error level and a $O(h^4)$ one, thereby making a Newton's correction step less useful, beyond limited special cases.   


\section{Approximate time derivative}\label{sec:app}

In several situations, we are not provided with the knowledge of how the function changes in time. 

\textcolor{red}{In which situations would one expect to need to do such an approximation? Is there a connection to stochastic control in discrete time?}

In these situations, to still be able to use our algorithms, we need to estimate the term $\nabla_{t\x} f(\x; t)$ is some ways. Let $\tilde{\nabla}_{t\x}{f}_k$ be an approximate version of $\nabla_{t\x}f(\x_k; t_k)$. Examples of such approximate version are the following. 

%We notice that most of the analysis in Theorem~\ref{th.centr} and \ref{th.net} carries trough unchanged. The only addition in the proofs is that we need to consider the extra source of error
%\begin{equation}\label{extraerr}
%\frac{h}{m}\|\tilde{\nabla}_{t\x}{f}_k -  \nabla_{t\x}f(\x_k; t_k)\| 
%\end{equation}
%which can be easily bounded once $\tilde{\nabla}_{t\x}{f}_k$ is available. Examples are the following.

\vskip2mm
\noindent\textbf{First-order backward derivative.} We can approximate the derivative as 
\begin{equation}\label{fobd}
\tilde{\nabla}_{t\x}{f}_k = \frac{1}{h} (\nabla_{\x}f(\x_k; t_k) - \nabla_{\x}f(\x_{k-1}; t_{k-1})),
\end{equation}
which has an approximation error of $O(h)$. %This combined with the $h$ factor in~\eqref{extraerr} brings the additional error to an $O(h^2)$ level.

\vskip2mm
\noindent\textbf{Higher-order backward derivative.} We can approximate the derivative recursively as
\begin{multline*}
\tilde{\nabla}_{t\x}{f}_k = \frac{1}{h}\left(a \nabla_{\x}f(\x_k; t_k) + b \nabla_{\x}f(\x_{k-1}; t_{k-1})\right. \\ \left.+ c \nabla_{\x}f(\x_{k-2}; t_{k-2}) + d\nabla_{\x}f(\x_{k-3}; t_{k-3})\right) - \beta \tilde{\nabla}_{t\x}{f}_{k-1},
\end{multline*}
which, if we specify the coefficient $(a,b,c,d,\beta)$ properly, leads to an approximation error of $O(h^2)$, $O(h^3)$, or $O(h^4)$~\cite{Lee1992}. %and therefore yields an error of at least one order of magnitude lower than the existing error bound. 

\vskip2mm
In the next corollary, we quantify the additional error of approximating the time derivative in our prediction-correction Algorithm~\ref{alg.centr}. We further show that this error goes as $O(h^2)$ for a simple first-order backward derivative, thereby stating that estimating the time derivative is not detrimental for our scheme. 

\begin{corollary}\label{co.approx}
Under the same conditions of Theorem~\ref{th.centr}, if we approximate the time derivative $\nabla_{t\x}f(\x_k; t_k)$ by using a first-order backward derivative as in~\eqref{fobd}, the asymptotic error bound of Algorithm~\ref{alg.centr} is not worse than the one of Theorem~\ref{th.centr}.  
\end{corollary}
%
\vskip2mm
\begin{myproof}

By Taylor expansion, one can see that
\begin{equation}\label{appder_oh}
\|\tilde{\nabla}_{t\x}{f}_k  - {\nabla}_{t\x}{f}(\x_k; t_k)\| = O(h),  
\end{equation}
also proving the claimed $O(h)$ error bound of the first-order backward derivative. In fact, one Taylor expands
\begin{equation}
{\nabla}_{\x}{f}(\x_{k-1}; t_{k-1}) = {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h + O(h^2),
\end{equation} 
and by solving for ${\nabla}_{t\x}{f}(\x_k; t_k)$, 
\begin{equation}
{\nabla}_{t\x}{f}(\x_k; t_k) = \frac{1}{h} ( {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h + O(h^2)).
\end{equation}
By substituting this result and the definition~\eqref{fobd} into~\eqref{appder_oh}, the $O(h)$ error bound is proven. 

Consider now the approximate prediction step, 
\begin{equation}
\x_{k+1|k} = \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h,
\end{equation}
which by adding and subtracting the exact prediction direction becomes, 
\begin{align}
\x_{k+1|k} &= \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h + \nonumber \\ &\quad 
+[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h  \nonumber \\ &\quad - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h.
\end{align}
By following the same steps as in Theorem~\ref{th.centr}, the term $a$ in Equation~\eqref{eq.hessian_cross_term} can be written with an extra error term as, 
\begin{align}\label{eq.hessian_cross_term_2}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h \nonumber \\ &\quad + \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h.
\end{align}
%
The extra error term w.r.t. Equation~\eqref{eq.hessian_cross_term} can be further bounded by using~\eqref{appder_oh} and the smoothness Assumption~\ref{as.smooth} (with the strong convexity constrant $m$)
\begin{multline}
 \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h \leq \\
 \|[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1}\| \| {\nabla}_{t\x}{f}(\x_k; t_k)  - \tilde{\nabla}_{t\x}{f}_k \| \, h \leq \\
 \frac{1}{m} O(h) \, h = O(h^2).
\end{multline}
This means that the extra error is of size $O(h^2)$ so it will not increase the $O(h^2)$ error bound already proven in Theorem~\ref{th.centr}.

\end{myproof}

Corollary~\ref{co.approx} says that we can approximate the time derivative simply by a first-order scheme. Better approximation will not decrease the functional dependence of the error in $h$, but may decrease the its magnitude. In the simulation results we show that

{\color{green} [Finish.]}  

\section{Prediction-Correction$(s)$ algorithms}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Prediction-Correction$(s)$ (gradient-based)}
\label{alg.pcs}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h
$$
\textbf{2:} Correction step: \\
\hspace*{4mm} \textbf{Set} $\x_{k+1/s|k} = \x_{k+1|k}$\\
\hspace*{4mm} \textbf{For} $\tau=1$ to $s$ \textbf{do}
$$
{\x}_{k+\tau/s} = P_{X}[\x_{k+\tau/s|k} - \gamma \nabla_{t\x} f(\x_{k+\tau/s|k}; t_{k+1})]
$$ 
\hspace*{4mm} \textbf{End}
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%


If we have enough computational power, we could always think to perform several correction steps (either of a gradient method or of a Newton's scheme), to further reduce the tracking asymptotical error. We call these algorithms Prediction-Correction$(s)$ algorithms (and they are parametrized over the number $s$ of correction steps. An example of such algorithm for gradient descent is given in Algorithm~\ref{alg.pcs}.

Convergence of such schemes can be proven in a similar fashion as in Theorem~\ref{th.centr}. As a bonus, in these schemes, the bigger $s$ is the larger $h$ can be chosen. This result as well as the convergence is encoded as follows. 

\begin{corollary}\label{co.pcs}
Under the same conditions of Theorem~\ref{th.centr}, Algorithm~\ref{alg.pcs} generates a sequence $\{\x_k\}$ that converges to $\x^*(t_k)$ asymptotically, with an error bound of 
$$
\lim_{k\to\infty} \|\x(t_k) - \x^*(t_k)\| = \frac{\rho^s}{1-\rho^s} O(h^2), \textrm{ if } \rho^s \sigma < 1, 
$$
and
$$
\lim_{k\to\infty} \|\x(t_k) - \x^*(t_k)\| = \frac{\rho^s}{1-\rho^s} O(h), \textrm{ if } \rho^s \sigma \geq 1, \rho < 1.
$$
In addition, if $s$ is selected as 
$$
s \geq \left\lceil \frac{p \log h}{\log(\rho(1 + h^p))}\right\rceil,
$$
then the asymptotical error is multiplied by a term $O(h^p)$.
\end{corollary}
%
\vskip2mm
\begin{myproof}

The proof is rather immediate and follows from the proof of Theorem~\ref{th.centr}. In particular, the only difference is in the correction step, which is performed $s$ times. Therefore, we can modify Equation~\eqref{eq.fin_t_k} as
$$
\|\x_{k+1} - \x^*(t_{k+1})\| \leq \rho^s \sigma \|\x_{k} - \x^*(t_{k})\| + \rho^s O(h^2),
$$
or Equation~\eqref{eq.sampling_error2} as 
$$
\|\x_{k+1} - \x^*(t_{k+1})\| \leq \rho^s \|\x_{k} - \x^*(t_{k})\| + \rho^s O(h),
$$
and the rest follows almost verbatim. The last result on the numbers of correction steps $s$ to obtain a certain error level, can be obtained directly by solving the equation
$$
\frac{\rho^s}{1-\rho^s} = h^p,
$$ 
for $s$. 

\end{myproof} 
















%\section{Approximate Hessian inverse}\label{sec:hess}





==> arXiv Version 2/Conclusion.tex <==
% !TEX root = TimeVarying_part1.tex
\section{Conclusion}\label{sec:conclusions}
%
We have designed algorithms to track the solution of time-varying unconstrained and strongly convex optimization problems. These algorithms leverage the knowledge of how the cost function changes in time and are based on a predictor-corrector scheme. We have also developed approximation schemes for when the rate at which the objective varies in time is not known. We established that these methods yield convergence to a neighborhood of the optimal trajectory, with a neighborhood of convergence dependent on the sampling period. Moreover, the size of this neighborhood is an order of magnitude smaller than state-of-the art running algorithms which only perform correction steps. In some cases when the problem parameters are appropriately chosen and second-order information is incorporated, the neighborhood of the optimal trajectory to which the algorithm converges is several orders of magnitude smaller than existing approaches. 

Moreover, we conducted a numerical analysis of the proposed methods in a simple setting which empirically supported the established error bounds. We also considered the task of developing a control strategy for an autonomous system to follow an object whose position varies continuously in time, showing that the developed tools yield an effective strategy. In some cases, the algorithms which achieve higher accuracy require\! too\! much\! computational latency to be used in a closed loop control setting; however, when this latency may be afforded, the second-order methods yield highly accurate tools.

Future research directions encompass the generalization of this work to constrained problems, general convex cost functions, as well as approximate second-order methods to weaken the computational requirements of computing the Hessian inverse in the prediction step.

==> arXiv Version 2/Convergence.tex <==
% !TEX root = Double.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%    S   E   C   T   I   O   N    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Convergence Analysis}\label{sec:conv}


In this section, we establish analytical results to bound the discrepancy between the optimal solution $\x^*(t)$ and the iterates $\x_k$ produced by the prediction-correction schemes developed in Section \ref{sec:probform}. Particularly, we will show that $\x_k$ tracks $\x^*(t)$ up to an error term that depends on the discrete-time sampling period. To this end, some technical conditions are required as stated next

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     A   S   S   U   M  P   T   I  O  N     %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{assumption} \label{as.str}
%The solution trajectory $\x^*(t)$ of~\eqref{eq.problem} is contained in the interior of a convex set $X\subseteq \mathbb{R}^n$ for each $t$.
%\end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     A   S   S   U   M  P   T   I  O  N     %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vskip2mm

\begin{assumption} \label{as.str} {\bf
The function $f(\x; t)$ is twice differentiable and $m$-strongly convex in $\x\in X$ and uniformly in $t$; that is, the Hessian of $f(\x; t)$ with respect to $\x$ is bounded below by $m$ for each $\x\in X$ and uniformly in $t$, 
$$
\nabla_{\x\x} f(\x; t) \succeq m \mathbf{I}, \quad \forall \x\in X, t.
$$  
In addition, the function $f(\x; t)$ has bounded second and third order derivatives with respect to $\x\in X$ and $t$:
$$
\|\nabla_{\x\x} f(\x; t)\|\leq L, \, \|\nabla_{t\x} f(\x; t)\|\leq C_0.
$$
}
\end{assumption}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     A   S   S   U   M  P   T   I  O  N     %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption} \label{as.smooth} 
{\bf
The function $f(\x; t)$ has bounded third order derivatives with respect to $\x\in X$ and $t$:
$$
\|\nabla_{\x\x\x} f(x; t)\|\!\leq \!C_1, \|\nabla_{\x t\x} f(\x; t)\|\!\leq\! C_2,  \|\nabla_{t t\x} f(\x; t)\|\!\leq \!C_3.
$$ 
}
\end{assumption}
\vskip2mm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   M  A   I    N        M   A   T   T  E   R    %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Assumption~\ref{as.str} is easily satisfied by taking $X$ to be $\mathbb{R}^n$, then we require the existence of a solution for~\eqref{eq.problem} at each time $t$. However, it is very useful in practice, when we know a priori that the solution trajectory has to be, for instance, positive. Then, we may use  algorithms and require the functional smoothness in Assumptions~\ref{as.str} and \ref{as.smooth} only in the set $X$. 
%

Assumption~\ref{as.str} guarantees that problem~\eqref{eq.problem} is strongly convex and has a \emph{unique} solution for each time instance. Uniqueness of the solution implies that the solution trajectory is also unique. Assumption\ref{as.str} also ensures that the Hessian is bounded from above; this property  is equivalent to the Lipschitz continuity of the gradient. This setting is common in the the time-varying optimization domain; see, for instance~\cite{Popkov2005, Dontchev2013, Jakubiec2013, Ling2013, Paper1, Paper2}. Assumption~\ref{as.smooth} ensures that the third derivative tensor $\nabla_{\x\x\x} f(x; t)$ is  bounded above (typically required for the analysis of Newton-type algorithms). Assumptions~\ref{as.str}-\ref{as.smooth} impose boundedness of the temporal variability of gradient and Hessian. These last properties ensure the possibility to build a prediction scheme based on the knowledge of (or an estimate of) how the function and its derivatives change over time. A similar assumption was required (albeit only locally) for the local convergence analysis in~\cite[Eq.~(3.2)]{Dontchev2013}. 

Assumption~\ref{as.str} is sufficient to show that the solution \emph{mapping} $t \mapsto \x^*(t)$ is single-valued and locally Lipschitz continuous in $t$; in particular, from \cite[Theorem 2F.10]{Dontchev2009} we have that
\begin{equation}\label{eq.lip}
\|\x^*(t_{k+1}) \!-\! \x^*(t_{k})\| \leq \! \frac{1}{m}\|\nabla_{t\x} f(\x; t)\| (t_{k+1}\!-\!t_{k}) \leq \frac{C_0 h }{m}, 
\end{equation} 
for sufficiently small sampling periods $h$. This result  established link between the sampling period $h$ and the temporal variability of the optimal solutions; further,~\eqref{eq.lip} will be utilized to substantiate convergence and tracking  capabilities of the proposed prediction-correction methods. 


\subsection{Constrained algorithm global $O(h)$ convergence}

We study the convergence properties of the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by the algorithm C-FOPC, for different choices of the stepsize. In the following theorem,  we show that the optimality gap $\|\x_k-\x^*(t_{k})\|$ converges exponentially to a given error bound, globally, i.e., from an arbitrary $\x_0$. 

\vskip2mm
\begin{theorem}\label{theo.constrained_0}

{\bf
Consider the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by the C-FOPC method, and let Assumption~\ref{as.str} hold true. Let $\x^*(t_k)$ be the optimizer of~\eqref{eq.problem} at time $t_k$. Define the following quantities 
\begin{equation}\label{stepsize_0}
\varrho_{\mathrm{P}} = \max\{|1-\alpha m|,|1- \alpha L|\}, \,\varrho_{\mathrm{C}} = \max\{|1-\beta m|,|1- \beta L|\},
\end{equation}
and choose the stepsizes $\alpha$ and $\beta$ as
\begin{equation}
\alpha < 2/L, \quad \beta < 2/L.
\end{equation}
Further, select the number of correction steps $C$ in a way that  
\begin{equation}\label{eq.cvrt}
\tau_0 := \varrho_{\mathrm{C}}^{C}\left[\varrho_{\mathrm{P}}^{P} + (\varrho_{\mathrm{P}}^{P}+1) \frac{2L}{m}\right]  <1.
\end{equation} 
%%
Then, the sequence $\{\|\x_k-\x^*(t_k)\|\}_{k \in \mathbb{N}}$ converges linearly with rate $\tau_0$ to an asymptotical error bound, and 
\begin{equation}\label{main.result1_0}
\limsup_{k\to\infty}\|\x_{k} - \x^*(t_k)\| = O(\varrho_{\mathrm{C}}^{C} h).
\end{equation}
}
\end{theorem}

\vskip2mm
\begin{IEEEproof}
See Appendix~\ref{ap.grad}, where we also derive all the constants in the right-hand side of~\eqref{main.result1_0}.
\end{IEEEproof}

\vskip2mm

Theorem~\ref{theo.constrained_0} says that the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by C-FOPC converges to a neighborhood of the optimal solution trajectory $\x^*(t)$. In particular, for a choice of prediction and correction steps $P$ and $C$, the sequence converge linearly to the asymptotic bound. The bound depends linearly on the sampling period and exponentially on the correction steps $C$. When one performs the correction step exactly, i.e., $C \to \infty$, then the asymptotic bound goes to zero (in fact, in that case each of the time-invariant problems is solved exactly). Finally, if one looks at the condition~\eqref{eq.cvrt}, one discovers that for global convergence one needs more that standard $\varrho_{\mathrm{C}}^{C} < 1$: in particular $C$ has to be chosen high enough to counteract any errors that come from the prediction step. We see next that this condition can be weakened in the case in which the cost function has higher order smoothness properties like the ones required by Assumption~\ref{as.smooth}. 




%% TALK ABOUT THE THEOREM. 
 



\subsection{Constrained algorithm local $O(h^2)$ convergence}

We study now the local convergence properties of the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by the algorithm C-FOPC under higher order smoothness (Assumption~\ref{as.smooth}), and we show that starting from a small enough optimality gap $\|\x_k-\x^*(t_{k})\|$, and for a small enough sampling period $h$, the error bound can be reduced from $O(h)$ to $O(h^2)$.

\vskip2mm

\begin{theorem}\label{theo.constrained}
{\bf
Consider the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by the C-FOPC method, and let Assumptions~\ref{as.str}-\ref{as.smooth} hold true. Let $\x^*(t_k)$ be the optimizer of~\eqref{eq.problem} at time $t_k$. Define the following quantities 
\begin{equation}\label{stepsize}
\varrho_{\mathrm{P}} = \max\{|1-\alpha m|,|1- \alpha L|\}, \, \varrho_{\mathrm{C}} = \max\{|1-\beta m|,|1- \beta L|\},
\end{equation}
and choose the stepsizes $\alpha$ and $\beta$ as
\begin{equation}
\alpha < 2/L, \quad \beta < 2/L.
\end{equation}
Further, select $\tau\in (0,1)$, the number of prediction steps $P$, and the number of correction steps $C$ in a way that  $\varrho_{\mathrm{P}}^{P}\varrho_{\mathrm{C}}^{C} < \tau$. 
%%

There exist an upper bound on the sampling period $\bar{h}$ and a convergence region $\bar{R}$, such that if the sampling period is chosen as $h \leq \bar{h}$ and the initial optimality gap satisfy $\|\x_{0} - \x^*(t_0)\| \leq \bar{R}$, then the sequence $\{\|\x_k-\x^*(t_k)\|\}_{k \in \mathbb{N}}$ converges linearly with rate $\tau$ to an asymptotical error bound, and 
\begin{equation}\label{main.result1}
\limsup_{k\to\infty}\|\x_{k} - \x^*(t_k)\| = O(h^2\,\varrho_{\mathrm{C}}^{C}) + O(h\,\varrho_{\mathrm{P}}^{P}\varrho_{\mathrm{C}}^{C}).
\end{equation}
In addition, the bounds $\bar{h}$ and $\bar{R}$ are given as
\begin{equation}
\bar{h} \!=\! \frac{\tau - \varrho_{\mathrm{C}}^{C}\varrho_{\mathrm{P}}^{P}}{\varrho_{\mathrm{C}}^{C}(\varrho_{\mathrm{P}}^{P} + 1)}\Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m} \Big)^{-1}\!\!\!, \bar{R} \!=\! \frac{2 \,m}{C_1}\! \Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m}\Big)\! (\bar{h}-h).
\end{equation}
}
\end{theorem}

\vskip2mm
\begin{IEEEproof}
See Appendix~\ref{ap.grad}, where we also derive all the constants in the right-hand side of~\eqref{main.result1}.
\end{IEEEproof}

\vskip2mm
%% TALK ABOUT THE THEOREM. AND DO THE LINK !
Theorem~\ref{theo.constrained} asserts that the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by C-FOPC locks to a neighborhood of the optimal solution trajectory $\x^*(t)$. In particular, for a choice of prediction and correction steps $P$ and $C$, there exist an upper bound on the sampling period and an attraction region, such that if the sampling period is smaller than the bound and the initial optimality gap is in the attraction region, then the sequence converge (at least) linearly to an asymptotic bound. The bound depends on the sampling period and on the selection of prediction and correction steps $P$ and $C$. When one performs an optimal prediction (that is $P \to \infty$), then the bound goes as $O(h^2)$, which is similar to the bounds derived in~\cite{Paper1}. When one performs the correction step exactly, i.e., $C \to \infty$, then the asymptotic bound goes to zero (in fact, in that case each time-invariant problem is solved exactly). % one is allowed to choose an arbitrarily big $h$, and convergence is global. 

%BLABLA on the putting together of the two theorems!

The presence of an attraction region is due to mimicking a Newton's step in the prediction stage (that is, the presence of the gradient $\nabla_{\x}f(\x_k; t_k)$ in the generalized equation~\eqref{ger0}). To further understand this point, consider the unconstrained case: as expressed in Section~\ref{sec:unc}, the prediction step optimization problem~\eqref{qp} has a closed-form solution as Eq.~\eqref{pred_up}. The presence of the gradient $\nabla_{\x}f(\x_k; t_k)$ translates into the presence of the Hessian inverse in~\eqref{pred_up}, which is a Newton's step. Our prediction strategy, even in the constrained case, mimics such step and inherits its pros and cons, e.g., the presence of a local convergence region. In addition, as in a Newton's method, when the function is quadratic, then $C_1 = 0$, and the convergence is global. 

By putting together the results of Theorems~\ref{theo.constrained_0}-\ref{theo.constrained}, one can arrive at simple strategies for parameter selection for the designer. In particular, for convergence, the designer needs only to know the strong convexity constant $m$ and the Lipschitz constant $L$, which is a standard requirement. Then, they can design the stepsizes $\alpha$ and $\beta$ as in~\eqref{stepsize_0} (or equivalently~\eqref{stepsize}) and the number of prediction and correction steps as in~\eqref{eq.cvrt}. With this in place, in the worst case they obtain a $O(\varrho_{\textrm{C}}^C h)$ error bound, and in the best case -- if the function satisfies Assumption~\ref{as.smooth}, the optimality gap enters in the attraction region, and $h$ is small enough -- they obtain a better $O(h^2\,\varrho_{\mathrm{C}}^{C}) + O(h\,\varrho_{\mathrm{P}}^{P}\varrho_{\mathrm{C}}^{C})$ error bound. This is the case, since the conditions on $C$ and $P$ are more stringent under Assumption~\ref{as.str} alone than with also the use of Assumption~\ref{as.smooth}. This eliminates de-facto the requirement of knowing (or estimating) the bounds $C_0, C_1, C_2, C_3$, which may be difficult to do in practice. 

%One could then utilize a warm start procedure to initialize the C-FOPC sequence and this obtains global convergence. Details are omitted in the interest of space. 

\subsection{Unconstrained algorithm convergence}

The results of Theorems~\ref{theo.constrained_0}-\ref{theo.constrained} can be tuned to the case of unconstrained problems as shown in the following. 

\vskip2mm

\begin{theorem}\label{theo.unconstrained_0}

{\bf
Consider the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by the U-FOPC method, and let Assumption~\ref{as.str} hold true. Let $\x^*(t_k)$ be the optimizer of~\eqref{eq.problem} at time $t_k$ for $X = \mathbb{R}^n$. Define the following quantities 
\begin{equation}
\varrho_{\mathrm{P}} = \max\{|1-\alpha m|,|1- \alpha L|\}, \, \varrho_{\mathrm{C}} = \max\{|1-\beta m|,|1- \beta L|\},
\end{equation}
and choose stepsizes $\alpha$ and $\beta$ as
\begin{equation}
\alpha < 2/L, \quad \beta < 2/L.
\end{equation}
Further, select the number of correction steps $C$ in a way that  
\begin{equation}\label{eq.cvrt_u}
\tau_0 := \varrho_{\mathrm{C}}^{C} \left[\varrho_{\mathrm{P}}^{P} +  (\varrho_{\mathrm{P}}^{P}+1)\Big(1-\gamma +\gamma \frac{2L}{m}\Big)\right]  <1.
\end{equation} 
%%
Then, the sequence $\{\|\x_k-\x^*(t_k)\|\}_{k \in \mathbb{N}}$ converges linearly with rate $\tau_0$ to an asymptotical error bound, and 
\begin{equation}\label{main.result2_0}
\limsup_{k\to\infty}\|\x_{k} - \x^*(t_k)\| = O(\varrho_{\mathrm{C}}^{C} h).
\end{equation}
}
\end{theorem}

\vskip2mm
\begin{IEEEproof}
See Appendix~\ref{ap.newton}, where we also derive all the constants in the right-hand side of~\eqref{main.result2_0}. The proofs leverage generalized equation theory and the special unconstrained nature of the problem.
\end{IEEEproof}

\vskip2mm

Similarly to Theorem~\ref{theo.constrained_0}, Theorem~\ref{theo.constrained_0} is a global $O(h)$ convergence result. From condition~\eqref{eq.cvrt_u}, it would seem that the best choice of $\gamma$ would be $\gamma = 0$; however this may not be the case when Assumption~\ref{as.smooth} holds. 

\vskip2mm

\begin{theorem}\label{theo.unconstrained}
%%
{\bf
Consider the sequence $\{\x_k\}_{k \in \mathbb{N}}$ generated by the U-FOPC method. Let Assumptions~\ref{as.str}-\ref{as.smooth} hold true. Let $\x^*(t_k)$ be the optimizer of~\eqref{eq.problem} at time $t_k$ for $X = \mathbb{R}^n$. Define, 
\begin{equation}
\varrho_{\mathrm{P}} = \max\{|1-\alpha m|,|1- \alpha L|\}, \, \varrho_{\mathrm{C}} = \max\{|1-\beta m|,|1- \beta L|\},
\end{equation}
and set the stepsizes $\alpha$ and $\beta$ as
\begin{equation}
\alpha < 2/L, \quad \beta < 2/L.
\end{equation}
Let $\tau\in (0,1)$, $P$, $C$ be such that 
\begin{equation}
(1-\gamma)\varrho_{\mathrm{C}}^{C}(1 + \varrho_{\mathrm{P}}^{P}) + \varrho_{\mathrm{P}}^{P}\varrho_{\mathrm{C}}^{C} < \tau.
\end{equation}
%%

There exist an upper bound on the sampling period $\bar{h}$ and a convergence region $\bar{R}$, such that if the sampling period is chosen as $h \leq \bar{h}$ and the initial optimality gap satisfy $\|\x_{0} - \x^*(t_0)\| \leq \bar{R}$, then the sequence $\{\|\x_k-\x^*(t_k)\|\}_{k \in \mathbb{N}}$ converges linearly with rate $\tau$ to an asymptotical error bound, and 
\begin{equation}\label{main.result2}
\limsup_{k\to\infty}\|\x_{k} - \x^*(t_k)\| = O(h^2\,\varrho_{\mathrm{C}}^{C}) + O(h\,\varrho_{\mathrm{P}}^{P}\varrho_{\mathrm{C}}^{C}).
\end{equation}
In addition, the bounds $\bar{h}$ and $\bar{R}$ are given as
\begin{align}\label{h.u}
\bar{h} &= \Big(\frac{\tau - \varrho_{\mathrm{C}}^{C}\varrho_{\mathrm{P}}^{P}}{\varrho_{\mathrm{C}}^{C}(\varrho_{\mathrm{P}}^{P} + 1)} - 1 + \gamma\Big)\Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m} \Big)^{-1}, \\ \bar{R} &= \frac{2 \,m}{\gamma C_1} \Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m}\Big)\, (\bar{h}-h).
\end{align}
}
\end{theorem}

\vskip2mm
\begin{IEEEproof}
See Appendix~\ref{ap.newton}, where we also derive all the constants in the right-hand side of~\eqref{main.result2}. The proofs leverage generalized equation theory and the special unconstrained nature of the problem. 
\end{IEEEproof}

\vskip2mm
Theorem~\ref{theo.unconstrained} is a local $O(h^2)$ convergence result. It can be seen as a generalization of Theorem~1 in~\cite{Paper1} and a special, yet more detailed, version of Theorem~\ref{theo.constrained}. In particular, by properly selecting the parameter $\gamma$, one obtains the results of both Theorem~\ref{theo.constrained} and~\cite{Paper1}; when  $\gamma = 1$, we obtain the  results of Theorem~\ref{theo.constrained} and this indicates that considering constrained problems does not add extra errors to the asymptotical bounds. On the other hand, if $\gamma = 0$, we are implicitly assuming that the prediction stage leads one to navigate into the iso-residual manifold;  since $\bar{R} \to \infty$, we also obtain global convergence. Furthermore, one can use $\gamma$ as a tuning mechanism to enlarge the convergence region. 

Finally, for $\gamma = 0$ and $P \to \infty$, then the results of theorem~\eqref{main.result2} boil down to those in~\cite{Paper1}. In particular, from~\eqref{h.u}, it can be seen  that the sampling period must satisfy the following relationship
\begin{equation}
\varrho_{\mathrm{C}}^{C}\Big[ 1 + h\, \Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m} \Big)\Big] < \tau < 1,
\end{equation}
which is the same requirement of~\cite[Theorem~1]{Paper1}. 




==> arXiv Version 2/Introduction.tex <==
% !TEX root = Double.tex

\section{Introduction}

%Current social and technological trends depict the rise of continental-size networks of interconnected, intelligent nodes. Ranging from the smart grid to transportation networks, these large-scale cyber-physical systems are supposed to change the way humans interact with the environment. At the core of these  

%Large-scale optimization problems

%Give a motivational introduction... 

%link it here to 
 

We consider constrained optimization problems that vary continuously in time. We outline the main ideas by first focusing on problems with a time-varying objective function. Consider then the following optimization problem:
\begin{equation}\label{eq.problem}
\x^*(t) :=\argmin_{\x\in X} f(\x; t), \quad \textrm{for } t \geq 0 \;, 
\end{equation}
where $X \subseteq \reals^n$ is a convex set; $t\in \reals_+$ is non-negative, continuous, and it is used to index time; and,  $f: \mathbb{R}^n\times \mathbb{R}_{+} \to \mathbb{R}$ is a \emph{smooth strongly convex function}.
%Our goal is to determine the solution $\x^*(t)$ of~\eqref{eq.problem} for each time $t$ which corresponds to the solution \emph{trajectory}. Time-varying optimization problems of the form \eqref{eq.problem} arise in  control \cite{Hours2014}, signal processing \cite{Jakubiec2013}, as well as in economics~\cite{Dontchev2013}. We are particularly interested in formulations of this setting which correspond to the tracking of objects whose position various continuously in time, or path-following problems. Target tracking problems of this type have a rich history in control, examples of which include waypoint generation in airborne vehicles \cite{castillo2007unmanned}, cruise control in automobiles \cite{vahidi2003research}, and intelligent behavior in robotics \cite{ardeshiri2010convex,verscheure2009time,cKoppelEtal15a,cKoppelEtal15b}.
The goal is to find (and track) the solution $\x^*(t)$ of~\eqref{eq.problem} for each time $t$ -- hereafter referred to as the  optimal solution \emph{trajectory}. 

Problem~\eqref{eq.problem} is a generalization of traditional time-invariant (i.e., static) problems, and can naturally model: a)  control problems where one seeks to generate a control action depending on a (parametric) varying optimization problem~\cite{Jerez2014,Hours2014,Gutjahr2016}; b) signal processing problems~\cite{Jakubiec2013}, where states of a dynamical process are  estimated online based on time-varying observations -- including time-varying compressive sensing settings~\cite{Asif2014,Yang2015,Vaswani2015,Balavoine2015,Simonetto2015a,Sopasakis2016}; and, c)  inferential problems on dynamic networks~\cite{Baingana2015}. Additional application domains include  robotics\cite{ardeshiri2010convex,verscheure2009time,Koppel2015a}, smart grids~\cite{Zhao2014,DallAnese2016,DallAnese2016a}, economics~\cite{Dontchev2013}, real-time magnetic resonance imaging (MRI)~\cite{Uecker2012}, and human migration studies~\cite{Nagurney2006}.

The problem \eqref{eq.problem} might be solved in a centralized setting based on a continuous time platform \cite{Ye2015,Rahili2015a,Rahili2015,Gong2016,Fazlyab2015,Fazlyab2016}; however, here we focus on a discrete time setting. The reason for this choice is motivated by the widespread use of digital computing units, such as control units (actuators) and digital sensors. In this context, we envision that our optimization problem will change in response to measurements taken at discrete time steps and its solution could provide control actions to be implemented on digital control units. 

Therefore, we use sampling arguments to reinterpret~\eqref{eq.problem}  as a sequence of time-invariant problems. In particular, upon sampling the objective functions $ f(\x; t)$ at time instants $t_{k}$,  $k=0,1,2,\dots$, where the sampling period $h := t_k - t_{k-1}$ can be chosen arbitrarily small, one can solve the sequence of time-invariant problems
%
\begin{equation}\label{eq.problemd}
\x^*(t_k) :=\argmin_{\x\in X} f(\x; t_k) ,  \hspace{.3cm}  k \in \mathbb{N}. 
\end{equation}
%
By decreasing $h$, an arbitrary accuracy may be achieved when approximating problem~\eqref{eq.problem} with \eqref{eq.problemd}. However, solving \eqref{eq.problemd} for each sampling time $t_k$ may not be computationally affordable in many application domains, even for moderate-size problems\footnote{Note that here we focus on constant sampling periods; variable ones induced by self-triggering have been considered in unconstrained problems~\cite{Fazlyab2016a} and could be considered in constrained problems in future works.}. %The requisite computation time for solving each instance of the problem often does not meet the requirements for real-time applicability, as in the control domain \cite{Bittanti2001}. 
%
%In addition, the idea of solving each instance of the problem up to an arbitrary accuracy does not lead to quantifiable real-time bounds. 
%
%It is also challenging to reasonably bound the time each problem instance will take to be solved~\cite{Boyd2004a}. In short, the majority of iterative methods for convex problems with static objectives may not be easily extended to handle time-varying objectives, with the exception of when the changes in the objective occur more slowly than the time necessary for computing the optimizer. 

%Similar arguments apply to the following minimax program: 
%\begin{equation}\label{eq.k0}
%\min_{\uu \in X}\, \max_{\vv \in V}\, K(\uu, \vv; t) , \quad \textrm{for } t \geq 0 \;,
%\end{equation}
%where $X \subseteq \reals^n$ and $V \subseteq \reals^q$ are convex sets, and function $K: \mathbb{R}^n\times \mathbb{R}^q \times \mathbb{R}_{+} \to \mathbb{R}$ is \emph{smooth strongly convex - strongly concave function}. Function $K(\uu, \vv; t)$ coincides with the regularized Lagrangian associated with a time-varying constrained optimization program (with time-varying inequality and equality constrains), with a double-smoothing regulatization~\cite{Nedic2011, Devolder2011}. However, it is worth pointing out that problem~\eqref{eq.k0}  is relevant also in robust optimization tasks~\cite{Boyd2004a}. 

Focusing on unconstrained optimization problems, the works in~\cite{Paper1, Paper2} developed a prediction-correction method to find and track the solution trajectory $\x^*(t)$ up to a bounded asymptotical error, starting from an arbitrary guess $\x_0$. This methodology arises from non-stationary optimization~\cite{Polyak1987,Popkov2005}, parametric programming~\cite{Robinson1980,Dontchev2009,Zavala2010,Dontchev2013}, and continuation methods in numerical mathematics~\cite{Allgower1990}. It also resembles evolutionary variational inequalities~\cite{Cojocaru2005,Nagurney2006} and path-following methods in interior point solvers~\cite{Nesterov2012}. This paper significantly broadens the method of~\cite{Paper1} by offering the following contributions. 
\begin{enumerate}
\item[\emph{(i)}] We develop prediction-correction methods to track the solutions of the time-varying \emph{constrained} problems~\eqref{eq.problem}; %particularly, a unique contribution consists in developing prediction-correction algorithms for the problem~\eqref{eq.k0}, and providing analytical bounds to characterize their tracking performance. 
\item[\emph{(ii)}] We develop first-order algorithms that do not involve the computation of the inverse of the Hessian of the cost function, as required in~\cite{Paper1}; the proposed prediction-correction method is computationally lighter, as it requires only matrix-vector multiplications. Further,  we offer a trade-off between tracking capabilities  and computational effort; and
\item[\emph{(iii)}] We show that the proposed prediction-correction algorithm improves on the method in~\cite{Paper1} when applied to unconstrained optimization problems; particularly, it exhibits enhanced local convergence properties by relying on Newton-like prediction steps. 
\end{enumerate}
The design and analysis of proposed prediction-correction methods are grounded on the theory of generalized equations and implicit function theorems~\cite{Dontchev2009}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% ORGANIZATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


{\bf Organization.} In Section~\ref{sec:probform}, we describe the prediction-correction methodology for constrained time-varying optimization problems. The special case of unconstrained case is developed in Section~\ref{sec:unc}. Convergence analysis is discussed in Section~\ref{sec:conv}, both for global $O(h)$ convergence and local $O(h^2)$ convergence. Numerical examples are displayed in Section~\ref{sec:num} -- including a realistic application in real-time control of energy resources --, and in Section~\ref{sec:concl}, we draw our conclusions. The proofs of all the propositions and theorems are given in the appendices. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% NOTATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


{\bf Notation.} Vectors are written as $\x\in\reals^n$ and matrices as $\A\in\reals^{n\times n}$. We use $\|\cdot\|$ to denote the Euclidean norm in the vector space, and the respective induced norms for matrices and tensors. The gradient of the function $f(\x; t)$ with respect to $\x$ at the point $(\x,t)$ is denoted as $\nabla_{\x} f(\x; t) \in \reals^n$, while the partial derivative of the same function with respect to (w.r.t.) $t$ at $(\x,t)$ is written as $\nabla_t f(\x; t)\in \reals$. Similarly, the notation $\nabla_{\x\x} f(\x; t) \in \reals^{n\times n}$ denotes the Hessian of $f(\x;t)$ w.r.t. $\x$ at $(\x,t)$, whereas $\nabla_{t\x} f(\x; t) \in \reals^{n}$ denotes the partial derivative of the gradient of $f(\x;t)$ w.r.t. the time $t$ at $(\x,t)$, i.e. the mixed first-order partial derivative vector of the objective. The tensor $\nabla_{\x\x\x} f(\x; t) \in \reals^{n\times n\times n}$ indicates the third derivative of $f(\x;t)$ w.r.t. $\x$ at $(\x,t)$, the matrix $\nabla_{\x t\x} f(\x; t) = \nabla_{t\x\x} f(\x; t)   \in \reals^{n\times n}$ indicates the time derivative of the Hessian of $f(\x;t)$ w.r.t. the time $t$ at $(\x,t)$, and the vector $\nabla_{t t\x} f(\x; t) \in \reals^{n}$ indicates the second derivative in time of the gradient of $f(\x;t)$ w.r.t. the time $t$ at $(\x,t)$. The indicator function is indicated as $\iota_{X}(\x)$ for the convex set $X \subseteq \mathbb{R}^n$; by definition $\iota_{X}(\x) = 0$ when $\x \in X$ and $+\infty$ otherwise. The subdifferential of $\iota_{\X}$ is the set-valued map known as normal cone $N_{X}: \mathbb{R}^n \rightrightarrows \mathbb{R}^n$ (Cf.~\cite{Dontchev2009}).
 
 


==> arXiv Version 2/Problem.tex <==
% !TEX root = Double.tex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Prediction-Correction Strategy}\label{sec:probform}


In this section, we first focus on problem~\eqref{eq.problem} and design a prediction-correction algorithm to track the (unique) trajectory of the optimal solution. As explained in the introduction, consider sampling~\eqref{eq.problem} at times $t_k$, $k \in \mathbb{N}$, and constructing a sequence of time-invariant problems~\eqref{eq.problemd}. In lieu of solving ~\eqref{eq.problemd} at each time step, the goal of the prediction-correction strategy is to determine an approximate optimizer for~\eqref{eq.problem} at $t_{k+1}$ in a computationally affordable way, given the current approximate optimizer at $t_k$. %To design the prediction-correction algorithm, we leverage tools from generalized equations and implicit function theory~\cite{Dontchev2009}.

\subsection{Prediction}

Suppose that $\x_k$ is an approximate solution of~\eqref{eq.problemd} at time $t_k$. Given $\x_k$,  the prediction step seeks an approximate optimizer for~\eqref{eq.problem} at $t_{k+1}$, given  the only information available at time $t_{k}$. Let $\x_{k+1|k}$ denote the output of the prediction step, which is computed as explained next. 

Notice first that solving the time-invariant problem~\eqref{eq.problemd} associated with time $t_k$ is equivalent to solving the generalized equation
\begin{equation}\label{ge}
\nabla_{\x} f(\x^*(t_k); t_k) + N_{X}(\x^*(t_k)) \ni \mathbf{0}
\end{equation}
where $N_X$ is the normal cone operator, while $\x^*(t_k)$ is the optimizer of~\eqref{eq.problemd} at $t_k$. Although many equivalent ways to formulate the solution of~\eqref{eq.problemd} exist, e.g., as the fixed-point of a properly defined operator, here we focus on generalized equations to build on the implicit function theorems of~\cite{Dontchev2013,Dontchev2009}.  

With~\eqref{ge} in place, the prediction step seeks the solution of the following perturbed generalized equation
\begin{multline}\label{ger0}
\nabla_{\x} f(\x_{k+1|k}; t_{k+1}) + N_{X}(\x_{k+1|k}) \approx \\
\nabla_{\x} f(\x_{k}; t_{k}) + \nabla_{\x\x} f(\x_{k}; t_{k}) (\x_{k+1|k} - \x_k)  \\ +  h\, \nabla_{t\x} f(\x_{k}; t_{k}) + N_{X}(\x_{k+1|k}) \ni \mathbf{0}.
\end{multline}
That is, the prediction step produces a solution that is optimal w.r.t. a perturbed (first-order) version of the original generalized equation~\eqref{ge}. The idea of this perturbed approximate version is motivated by the fact that one would like to solve $\nabla_{\x} f(\x_{k+1|k}; t_{k+1}) + N_{X}(\x_{k+1|k})\ni \mathbf{0}$, but that is not possible at time $t_{k}$. Therefore, we perturb said generalized equation by a backward Taylor expansion, in a way that is possible to solve it at time $t_k$.

We can now replace~\eqref{ger0} with the following equivalent formulation
\begin{multline}\label{qp}
\x_{k+1|k} \!= \!\argmin_{\x \in X} \Big\{\frac{1}{2} \x^\transp \nabla_{\x\x} f(\x_k; t_k) \x \\ + (\nabla_{\x} f(\x_k; t_k) + h\, \nabla_{t\x} f(\x_k; t_k) -\nabla_{\x\x} f(\x_k; t_k)\x_k )^\transp\x\Big\},
\end{multline}
where we can notice that the normal cone operator yields the feasible set over which the optimization is computed. 

In lieu of seeking an exact solution of~\eqref{qp} (which is a constrained optimization problem with quadratic cost), consider the less computational demanding task of finding an approximate solution of~\eqref{qp} by computing a number of  projected gradient descent steps -- the first key step towards a \emph{first-order} prediction-correction method (Note that we consciously avoid Newton's method here for the high computational complexity burden of computing the Hessian inverse). Particularly, let ${\widehat{\x}^0}$ be a dummy variable initialized as ${\widehat{\x}^0} = \x_k$; then, the following steps are performed:
\begin{multline}\label{gpred}
{\widehat{\x}^{p+1}} = \mathbb{P}_{X}[\widehat{\x}^{p} -  \alpha (\nabla_{\x\x} f(\x_k; t_k)(\widehat{\x}^{p}-\x_k) \\+ h\, \nabla_{t\x} f(\x_k; t_k) + \nabla_{\x} f(\x_k; t_k))],
\end{multline}
for $p = 0, 1, \dots, P-1$, where $P$ is a pre-determined number of gradient steps, $\alpha > 0$ is the stepsize, and $\mathbb{P}_X$ is the projection operator over the convex set $X$. Once $P$ steps are performed, $\tilde{\x}_{k+1|k}$ is set to:
\begin{equation}
\tilde{\x}_{k+1|k} = \widehat{\x}^{P}.
\end{equation}

%\subsubsection{Zero-residual prediction}

%Given a certain $\r$ at time $t_k$, the zero-residual prediction step attempts at finding a vector $\x_{k+1|k} for time $t_{k+1}$, for which the residual is zero. By using the same perturbation of~\eqref{ger1}, we will formulate the problem of finding $\x_{k+1|k}$ as the one of finding the solution of the generalized equation
%\begin{multline}\label{ger1.0}
%\nabla_{\x} f(\x_{k+1|k}; t_{k+1}) + N_{X}(\x_{k+1|k}) \approx \\
%\nabla_{\x} f(\x_{k}; t_{k}) + \nabla_{\x\x} f(\x_{k}; t_{k}) (\x_{k+1|k} - \x_k)  \\ +  h\, \nabla_{t\x} f(\x_{k}; t_{k}) + N_{X}(\x_{k+1|k}) \ni \mathbf{0},
%\end{multline}
%where we put $\r = \mathbf{0}$. The generalized equation~\eqref{ger1.0} yields the convex quadratic problem:
%\begin{equation}\label{qp.0}
%{\x}_{k+1|k} \!= \!\argmin_{\x} !!
%\end{equation}
%which, once solved, provides the predicted variable $\x_{k+1|k}$. 

%As in the tangential case, we look at first-order gradient methods to determine an approximate ${\x}_{k+1|k}$. Let ${\widehat{\x}^0}$ be a dummy variable initialized as ${\widehat{\x}^0} = \mathbf{0}$. The gradient zero-residual prediction is the following recursion, 
%\begin{multline}\label{gpred.0}
%{\widehat{\x}^{p+1}} \!\!= \mathbb{P}_{X}[\x_{k} + {\widehat{\x}^{p}} - \\ \alpha (\nabla_{\x\x} f(\x_k; t_k){\delta\widehat{\x}^{p}} + h\, \nabla_{t\x} f(\x_k; t_k))] - \x_k,
%\end{multline}
%for $p = 0, 1, \dots, P$, where $P+1$ is the total number of gradient steps and $\alpha > 0$ the stepsize. At the end, the approximate prediction variable $\tilde{\x}_{k+1|k}$ is computed as 
%\begin{equation}
%\tilde{\x}_{k+1|k} = \x_k + {\delta\widehat{\x}^{P+1}}.
%\end{equation}

%As one can notice the major difference between .. and .. is the presence of a Newton-like term (..) in the zero-residual gradient. This term will make the difference between convergence analysis for .. and .. 

%\subsubsection{Special case: unconstrained optimization.}

%It is instructive to look back at unconstrained optimization, for which $X = \reals^n$ and specialize the optimization problems ..-.. . The tangential strategy yields
%..
%
%while the zero-residual 
%.. 

%One can decide to solve these two problems analytically (if one can afford to compute the Hessian inverse), which leads to the predictions
%..
%..

%We see immediately the Newton-like term in .. 

%One can also decide instead to look for first-order gradient methods as, 

%.. 

%.. 

%Where we have used the same notation as of .. 

%As we see, we find as a special case the same methodology of .. (cf. .. and the equation ..). 


\subsection{Correction}

Once the cost function $f(\cdot; t_{k+1})$ becomes available, the correction step is performed to refine the estimate of the optimal solution $\x^*(t_{k+1})$. To this end, a first-order projected gradient method is considered next. Particularly, let $\widehat{\x}^{0} = \tilde{\x}_{k+1|k}$ be  a dummy variable; then, consider the following projected gradient steps
\begin{equation}\label{gcorr}
{\widehat{\x}^{c+1}} \!\!= \mathbb{P}_{X}[{\widehat{\x}^{c}} - \\ \beta (\nabla_{\x} f(\widehat{\x}^{c}; t_{k+1})],
\end{equation}
for $c = 0, 1, \dots, C-1$, where $C$ is a predetermined number of gradient steps and $\beta >0 $ the stepsize. The estimate of the optimal solution $\x^*_{k+1}$ is then computed as 
%\begin{equation}
${\x}_{k+1} = \widehat{\x}^{C}$.
%\end{equation}

%Notice that a Newton step could be implemented; however, to develop computationally light online schemes that naturally afford a distributed implementation, this paper considers first-order methods.  


\subsection{Complete Algorithm}

The complete algorithm Constrained - First Order Prediction Correction (C-FOPC) is tabulated as Algorithm~\ref{algo_fo}. Steps 4-7 are utilized to compute $ \tilde{\x}_{k+1|k}$ based on the information available at $t_{k}$. Provided that the projection operator is easy to carry out (set $X$ is simple, e.g., it is an $\ell_2$ or $\ell_{\infty}$ norm), and the Hessian is easy to evaluate, the computational complexity of these steps is $O(Pn^2)$, which is quadratic (due to matrix-vector multiplications) in the number of scalar decision variables. This is in contrast with  the algorithms presented in \cite{Paper1}, which involve the computation of the Hessian inverse and whose computational complexity is therefore $O(n^3)$. Steps 10-14 are utilized to compute ${\x}_{k+1}$, based on the information available at $t_{k+1}$. Provided that the projection operator is easy to perform (set $X$ is simple) and the gradient is easy to evaluate, the computational complexity of these steps is $O(Cn)$, which is linear in the number of scalar decision variables. 

%% Computation account
%\vskip2mm
%\begin{remark}
%\emph{[Distributed implementation]} C-FOPC naturally affords a distributed implementation for networked time-varying problems, i.e., for problems for which the gradient and Hessian can be computed via one-hop communication with neighboring nodes/agents and the constraint set $X$ is the cartesian product of local constraints (in fact, in these cases, C-FOPC involves only one round of communication among neighboring nodes to perform one step of prediction and one step of correction). This is in contrast with exact prediction schemes that necessitate the computation of an approximate inverse of the Hessian in a distributed fashion~\cite{Paper2}. The exact characterization of how this aspect affects the asymptotical error and convergence speed is left as future research. 
%\end{remark}

\begin{remark}
\emph{[Time derivative approximation]} The time derivative of the gradient $\nabla_{t\x} f(\x; t)$ can be substituted with an approximate version, as explained in~\cite{Paper1}.
\end{remark}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\begin{algorithm}[tb]
\caption{Constrained First-Order Prediction-Correction (C-FOPC)}\label{algo_fo} 
\begin{algorithmic}[1] 
\small{\REQUIRE  Initial variable $\x_0$. Initial objective function $f(\x;t_0)$, no. of prediction steps $P$ and correction steps $C$
\FOR {$k=0,1,2,\ldots$}
\STATE \color{blue}// time $t_k$ \color{black}
   \STATE Prediction: initialize ${\widehat{\x}^0} = \x_k$
%%%
   \FOR {$p=0:P-1$}
          \STATE  Predict the variable by the  gradient step  [cf \eqref{gpred}]   
         \begin{multline*}
{\widehat{\x}^{p+1}} \!\!= \mathbb{P}_{X}[ {\widehat{\x}^{p}} -  \alpha (\nabla_{\x\x} f(\x_k; t_k){(\widehat{\x}^{p} - \x_k)} +\\ h\, \nabla_{t\x} f(\x_k; t_k) + \nabla_{\x}f(\x_k; t_k))] \end{multline*}
\ENDFOR
\STATE Set the predicted variable $\tilde{\x}_{k+1|k}=\widehat{\x}^{P}$
%%%%%%%%%%%%%%%%
\STATE \color{blue}// time $t_{k+1}$ \color{black}
\STATE Acquire the updated function $f(\x;t_{k+1})$
%%%%%%%%%%%%%%%
   \STATE Initialize the sequence of corrected variables $\widehat{\x}^{0} = \tilde{\x}_{k+1|k}$ 
     \FOR {$c=0:C-1$}
          \STATE  Correct the variable by the  gradient step  [cf \eqref{gcorr}]   
         $${\widehat{\x}^{c+1}} \!\!= \mathbb{P}_{X}[{\widehat{\x}^{c}} - \beta (\nabla_{\x} f(\widehat{\x}^{c}; t_{k+1})]$$
          \ENDFOR
 %%%%%%%%%%%%%%%         
   \STATE Set the corrected variable ${\x}_{k+1}=\widehat{\x}^{C}$
          %
\ENDFOR}
\end{algorithmic}\end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Special Case: Unconstrained Problems}\label{sec:unc}

In this section, we focus on the special case of unconstrained problems (i.e., $X = \reals^n$). Although~\cite{Paper1} has given an extensive characterization of methods for unconstrained problems, we will see in this section that further important improvements can be achieved based on the prediction generalized equation~\eqref{ger0}. 

For unconstrained problems, the prediction equation~\eqref{ger0} can be rewritten as
\begin{multline}\label{ger0.0}
\nabla_{\x} f(\x_{k+1|k}; t_{k+1}) \approx 
\nabla_{\x} f(\x_{k}; t_{k}) + \\ \nabla_{\x\x} f(\x_{k}; t_{k}) (\x_{k+1|k} - \x_k)  +  h\, \nabla_{t\x} f(\x_{k}; t_{k}) = \mathbf{0}.
\end{multline}
Since the suboptimality at time $t_k$ can be easily characterized by the gradient, i.e., $\nabla_{\x} f(\x_{k}; t_{k})$, we can also modify~\eqref{ger0.0} to tune the prediction step. A way to do that is to require $\x_{k+1|k}$ to reduce the suboptimality by a factor of $1-\gamma \in [0,1]$, and pose the problem as 
\begin{multline}\label{ger0.1}
\nabla_{\x} f(\x_{k+1|k}; t_{k+1}) \approx 
\nabla_{\x} f(\x_{k}; t_{k}) + \nabla_{\x\x} f(\x_{k}; t_{k})\times\\ (\x_{k+1|k} - \x_k)  +  h\, \nabla_{t\x} f(\x_{k}; t_{k}) = (1-\gamma)\nabla_{\x} f(\x_k; t_{k}).
\end{multline}
When $\gamma = 1$,~\eqref{ger0.1} boils down to~\eqref{ger0.0} (when one seeks an ``optimal prediction''); on the other hand, when $\gamma = 0$, ~\eqref{ger0.1} coincide with~\cite{Paper1}, where a prediction vector that maintains the same suboptimality (i.e., the same gradient) between successive time steps is sought. Notice that the possibility of tuning the algorithm via $\gamma$ is possible only for unconstrained optimization problems, since we have access to a ``suboptimality measure''. 

From~\eqref{ger0.1} we obtain the prediction vector via the following update
\begin{multline}
\label{pred_up}
\x_{k+1|k} = \x_{k} - \nabla_{\x\x} f(\x_{k}; t_{k})^{-1}\times\\(h\, \nabla_{t\x} f(\x_{k}; t_{k}) + \gamma \, \nabla_{\x} f(\x_{k}; t_{k})),
\end{multline}
which combines a Newton-like step in the direction on the changing cost function, and a (damped) Newton's step towards the optimizer at time $t_k$. When $\gamma = 0$,~\eqref{pred_up} coincides with the prediction step in~\cite{Paper1}. To obtain a first-order update, it is then easy to modify~\eqref{gpred} as
\begin{multline}\label{gpred.0}
{\widehat{\x}^{p+1}} \!\!= \widehat{\x}^{p} - \alpha (\nabla_{\x\x} f(\x_k; t_k)(\widehat{\x}^{p}-\x_k) \\ + h\, \nabla_{t\x} f(\x_k; t_k)+\gamma\,\nabla_{\x} f(\x_k; t_k)),
\end{multline}
where the notation is the same as in~\eqref{gpred}. On the other hand, the correction update becomes in this case
\begin{equation}\label{gcorr.0}
{\widehat{\x}^{c+1}} \!\!= {\widehat{\x}^{c}} - \\ \beta (\nabla_{\x} f(\widehat{\x}^{c}; t_{k+1}).
\end{equation}
The resultant Unconstrained - First Order Prediction Correction (U-FOPC) method  is tabulated as Algorithm~\ref{algo_fou}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\begin{algorithm}[tb]
\caption{Unconstrained First-Order Prediction-Correction (U-FOPC)}\label{algo_fou} 
\begin{algorithmic}[1] 
\small{\REQUIRE  Initial variable $\x_0$. Initial objective function $f(\x;t_0)$, no. of prediction steps $P+1$ and correction steps $C+1$, sub-optimality requirement $\gamma\in[0,1]$
\FOR {$k=0,1,2,\ldots$}
\STATE \color{blue}// time $t_k$ \color{black}
   \STATE Prediction: initialize ${\widehat{\x}^0} = \x_k$
%%%
   \FOR {$p=0:P-1$}
          \STATE  Predict the variable by the  gradient step  [cf \eqref{gpred}]   
         \begin{multline*}
{\widehat{\x}^{p+1}}  = {\widehat{\x}^{p}} -\alpha (\nabla_{\x\x} f(\x_k; t_k){(\widehat{\x}^{p} - \x_k)} \\+ h\, \nabla_{t\x} f(\x_k; t_k)+\gamma\,\nabla_{\x} f(\x_k; t_k)) \end{multline*}
\ENDFOR
\STATE Set the predicted variable $\tilde{\x}_{k+1|k}=\widehat{\x}^{P}$
%%%%%%%%%%%%%%%%
\STATE \color{blue}// time $t_{k+1}$ \color{black}
\STATE Acquire the updated function $f(\x;t_{k+1})$
%%%%%%%%%%%%%%%
   \STATE Initialize the sequence of corrected variables $\widehat{\x}^{0} = \tilde{\x}_{k+1|k}$ 
     \FOR {$c=0:C-1$}
          \STATE  Correct the variable by the  gradient step  [cf \eqref{gcorr}]   
         $${\widehat{\x}^{c+1}} \!\!= \mathbb{P}_{X}[{\widehat{\x}^{c}} - \beta (\nabla_{\x} f(\widehat{\x}^{c}; t_{k+1})]$$
          \ENDFOR
 %%%%%%%%%%%%%%%         
   \STATE Set the corrected variable ${\x}_{k+1}=\widehat{\x}^{C}$
          %
\ENDFOR}
\end{algorithmic}\end{algorithm} 






==> arXiv Version 2/Proofs.tex <==

% !TEX root = TimeVarying_part1.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage

\section{Preliminaries}

We begin the convergence analysis by deriving an upper bound on the norm of the approximation error $\mathbold{\Delta}_k\in \reals^n$ incurred by the Taylor expansion in~\eqref{ger0}. In particular, given  the optimal solution $\x^*(t_k)$ at $t_k$, compute the optimal prediction step via the Taylor approximation~\eqref{ger0} and indicate the optimal prediction as $\x^*_{k+1|k}$. The objective is to bound the error:
%%%
\begin{align}\label{eq.def.delta}
\mathbold{\Delta}_k : = \x^*_{k+1|k} - \x^*(t_{k+1}),
\end{align}
which is committed when $\x^*(t_{k+1})$ is replaced by $\x^*_{k+1|k}$ (here we use the superscript $*$ to indicate that we compute the prediction from $\x^*(t_k)$ and not any $\x_k$).

%Deriving an  upper bound on $\|\mathbold{\Delta}_k \|$ is key towards to establishing convergence and tracking results, since it substantiates the error introduced by the prediction step. An upper bound on $\|\mathbold{\Delta}_k \|$  is derived next.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     P  R   O   P  O  S  I  T   I  O  N     %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{1mm}
\begin{proposition}\label{prop.err}
{\bf
The error norm $\|\mathbold{\Delta}_k\|$ is upper bounded as follows. 

\emph{Case a)} Under the sole Assumption~\ref{as.str}
\begin{equation}\label{prop_claim_err_bound_0}
\|\mathbold{\Delta}_k\| \leq 2 h \frac{C_0}{m} (1+L/m) =: \Delta_1 = O(h).
\end{equation}

\emph{Case b)} Under both Assumption~\ref{as.str} and~\ref{as.smooth}
%
\begin{equation}\label{prop_claim_err_bound}
\|\mathbold{\Delta}_k\| \leq \frac{h^2}{2} \left[\frac{C_0^2 C_1}{m^3} + \frac{2 C_0 C_2}{m^2} + \frac{C_3}{m}\right] =: \Delta_2 = O(h^2).
\end{equation}
}
%
\end{proposition}

\begin{IEEEproof}
Let us start by simplifying the notation. Define
\begin{align}\label{simplif}
\nabla_{\x} f_i = \nabla_{\x} f (\x^*(t_{k+i}); t_{k+i}), \quad & \Q_i = \nabla_{\x\x} f (\x^*(t_{k+i}); t_{k+i}) \\ \label{simplif22}
\c_i = \nabla_{t\x} f (\x^*(t_{k+i}); t_{k+i}),\quad & \x_i = \x^*(t_{k+i}), \, \x = \x^*_{k+1|k}.
\end{align}
With this notation in place, $\mathbold{\Delta}_k = \x - \x_{1}$ [Cf.~\eqref{eq.def.delta}]. In addition, $\x$ is computed by the generalized equation~\eqref{ger0}, 
\begin{equation}\label{proofA.dummy1}
\nabla_{\x} f_0 + \Q_0 (\x - \x_0) + h\, \c_0 + N_X(\x) \ni \mathbf{0},
\end{equation}
while $\x_1$ is the solution of 
\begin{equation}\label{proofA.dummy2}
\nabla_{\x} f_1 + N_X(\x_1) \ni \mathbf{0}.
\end{equation}

Define the supporting functions, 
\begin{align}\label{proofA.dummy3}
G(\y) &= \nabla_{\x} f_1 + \Q_1(\y - \x_1) + N_X(\y)\\
g(\y) &= \nabla_{\x} f_0 + \Q_0 (\y- \x_0) + h\, \c_0 + \nonumber \\ & \hskip3cm - [\nabla_{\x}f_1 + \Q_1 (\y - \x_1)].  
\end{align}
These two functions allows one to rewrite~\eqref{proofA.dummy1} as 
\begin{equation}\label{proofA.dummy4}
(g + G)(\x) \ni \mathbf{0}.
\end{equation}
It is also true that $(g + G)(\x_1) \ni g(\x_1)$, since for optimality $G(\x_1) \ni \mathbf{0}$. Define $F(\y) = (g + G)(\y)$, and consider the parametric generalized equation $F(\y) + \p \ni \mathbf{0}$. Under the Assumptions~\ref{as.str}-\ref{as.smooth}, as for \cite[Theorem~2F.9]{Dontchev2009}, we have that the solution mapping $\p \mapsto \y(\p)$ for the generalized equation $F(\y) + \p \ni \mathbf{0}$ is every-where single valued and Lipschitz continuous with constant $m^{-1}$, that is 
\begin{equation}\label{proofA.dummy5}
\|\y(\p) - \y(\p')\| \leq \frac{1}{m} \|\p - \p'\|.
\end{equation}

We can set $\p = \mathbf{0}$ and $\p' = -g(\x_1)$, which leads to 
\begin{equation}\label{proofA.dummy6}
\|\x - \x_1\| = \|\mathbold{\Delta}_k\| \leq \frac{1}{m} \|g(\x_1)\|.
\end{equation}

We proceed now to bound $\|g(\x_1)\|$. We can write $g(\x_1)$ as
\begin{equation}\label{eq-dummy}
g(\x_1) = \nabla_{\x} f_0 + \Q_0 (\x_1- \x_0) + h\, \c_0 - \nabla_{\x} f_1.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CASE A
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Case a)}

Given the expression of $g(\x_1)$, we can bound its norm via Assumption~\ref{as.str}
\begin{align}\label{eq.bound1}
\|g(\x_1)\| &\leq \|\nabla_{\x} f_0 - \nabla_{\x} f_1\| + \|\Q_0\|\|\x_1- \x_0\| + h\, \|\c_0\| \nonumber \\
&\leq \|\nabla_{\x} f_0 - \nabla_{\x} f_1\| + L \|\x_1- \x_0\| + h C_0,
\end{align}
where we have used the upper bound on the Hessian of the cost function. Furthermore, 
\begin{multline}\label{eq.bound2}
\!\!\!\|\nabla_{\x} f_0 - \nabla_{\x} f_1\|  = \|\nabla_{\x} f(\x^*(t_k);t_k) - \nabla_{\x} f(\x^*(t_{k+1});t_{k+1})\| \\
\leq \|\nabla_{\x} f(\x^*(t_k);t_{k+1}) - \nabla_{\x} f(\x^*(t_{k+1});t_{k+1})\| +\\ \|\nabla_{\x} f(\x^*(t_k);t_{k}) - \nabla_{\x} f(\x^*(t_{k});t_{k+1}) \|
\end{multline}
We can bound the first term in the right hand side with the Lipschitz property of the gradient of the cost function as
\begin{equation}\label{eq.bound3}
\|\nabla_{\x} f(\x^*(t_k);t_{k+1}) - \nabla_{\x} f(\x^*(t_{k+1});t_{k+1})\| \leq L \|\x_1 - \x_0\|,
\end{equation}
while the second part can be bounded by the upper bound on $\nabla_{t\x}f$, as
\begin{multline}\label{eq.bound4}
\!\!\|\nabla_{\x} f(\x^*(t_k);t_{k}) - \nabla_{\x} f(\x^*(t_{k});t_{k+1}) \| \!= \! \|\nabla_{\x} f(\x^*(t_k);t_{k})  \\-\nabla_{\x} f(\x^*(t_{k});t_{k}) - h\, \nabla_{t\x}f(\x^*(t_{k});\tau)\| \leq h C_0,
\end{multline}
where we have used the mean value theorem and $\tau \in [t_k, t_{k+1}]$. By putting Eq.s~\eqref{eq.bound1}, \eqref{eq.bound2}, \eqref{eq.bound3}, and~\eqref{eq.bound4} together, one arrives at
\begin{equation}\label{eq-dummy_1}
\|g(\x_1)\| \leq 2 L \|\x_1- \x_0\| + 2 h\, C_0,
\end{equation}
and by using~\eqref{proofA.dummy6} as well as the bound on $\|\x_1 - \x_0\|$ in~\eqref{eq.lip}, the claim~\eqref{prop_claim_err_bound_0} follows. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CASE B
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Case b)}
By allowing higher order smoothness, the bound on $g(\x_1)$ can be improved as follows. Consider~\eqref{eq-dummy}: it is nothing else but the error of the truncated Taylor expansion of $\nabla_{\x} f_1$:
\begin{equation}
\nabla_{\x} f_1 - \nabla_{\x} f_0 =  \Q_0 (\x_1-\x_0) + h \c_0 +\mathbold{\epsilon},
\end{equation} 
where the error $\mathbold{\epsilon}$ can be bounded as
\begin{multline}
\|\mathbold{\epsilon}\| \leq \frac{1}{2}\Big(\|\nabla_{\x\x\x} f\| \|\x_1- \x_0\|^2 + h\, \|\nabla_{t\x\x} f\| \|\x_1- \x_0\| +\\  h\, \|\nabla_{\x t\x} f\| \|\x_1- \x_0\|  + {h^2} \|\nabla_{t t\x} f\|\Big),
\end{multline}
and by using the upper bounds in Assumption~\ref{as.smooth}, 
\begin{equation}
\|g(\x_1)\| \leq \frac{1}{2}\, C_1 \|\x_1 - \x_0\|^2 + h\, C_2 \|\x_1 - \x_0\| + \frac{1}{2} h^2\, C_3. 
\end{equation}
By using the bound~\eqref{eq.lip} on the variability of the optimizers $\x_1$ and $\x_0$, then 
\begin{equation}
\|g(\x_1)\| \leq h^2\,C_1 \frac{C_0^2}{2 m^2} + h^2\, C_2 \frac{C_0}{m} + \frac{1}{2} h^2\, C_3, 
\end{equation}
and by combining this bound with~\eqref{proofA.dummy6}, the claim~\eqref{prop_claim_err_bound} follows. 
%%
\end{IEEEproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorems \ref{theo.constrained_0} and \ref{theo.constrained}}\label{ap.grad}

We divide the proof in different steps. Step 1: we bound the prediction error in Propositions~\ref{prop.intheo.1} and~\ref{prop.intheo.2}; Step 2: we bound the correction error; Step 3: we put the previous steps together and derive the convergence requirements and results. As done for Proposition~\ref{prop.err}, Case a) will refer to Theorem~\ref{theo.constrained_0}, while Case b) to Theorem~\ref{theo.constrained}.

 
\vskip2mm 

\noindent \textbf{Prediction error.} The optimal prediction error, i.e., the distance between the optimal predicted variable $\x_{k+1|k}$ and the optimizer at time step $t_{k+1}$, $\x^*(t_{k+1})$ can be bounded as the following proposition. 
\vskip2mm

\begin{proposition}\label{prop.intheo.1}
{\bf
The following facts hold true. 
\begin{enumerate}
\item[{Case a)}] Under the same assumptions and notation of Theorem~\ref{theo.constrained_0}, we have that
%%
\begin{equation}\label{prop_inside_0}
\|\x_{k+1|k} - \x^*(t_{k+1})\| \leq \frac{2 L}{m}\|\x_k- \x^*(t_k)\|+ \Delta_1.
\end{equation}
%%
\item[{Case b)}] Under the same assumptions and notation of Theorem~\ref{theo.constrained}, we have that
\begin{multline}\label{prop_inside}
\|\x_{k+1|k} - \x^*(t_{k+1})\| \leq \frac{C_1}{2\,m}\|\x_k- \x^*(t_k)\|^2 +\\ h\,\Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m}  \Big)\|\x_k- \x^*(t_k)\|+ \Delta_2.
\end{multline}
\end{enumerate}
}
\end{proposition}
\vskip2mm
\begin{IEEEproof}
We proceed as in the proof of Proposition~\ref{prop.err}. We use similar simplifications of~\eqref{simplif}, as
\begin{subequations}\label{simplif2}
\begin{align}
\nabla_{\x} f_k = \nabla_{\x} f (\x_k; t_{k}), \quad & \Q_k = \nabla_{\x\x} f \x_k; t_{k}) \\
\c_k = \nabla_{t\x} f (\x_k; t_{k}),\quad & \x = \x_{k+1|k}.
\end{align}
\end{subequations}
while $\nabla_{\x} f_1$ and $\x_1$ are defined just as in~\eqref{simplif}. The error $\|\x_{k+1|k} - \x^*(t_{k+1})\|$ is now $\x - \x_1$. 

The vector $\x$ is computed by the generalized equation~\eqref{ger0}, 
\begin{equation}\label{proofB.dummy1}
\nabla_{\x} f_k + \Q_k (\x - \x_k) + h\, \c_k + N_X(\x) \ni \mathbf{0},
\end{equation}
while $\x_1$ is the solution of~\eqref{proofA.dummy2}.

Define the supporting functions, 
\begin{align}\label{proofB.dummy3}
G(\y) &= \nabla_{\x} f_1 + \Q_1(\y - \x_1) + N_X(\y)\\
g(\y) &= \nabla_{\x} f_k + \Q_k (\y- \x_k) + h\, \c_k + \nonumber \\ & \hskip3cm - [\nabla_{\x}f_1 + \Q_1 (\y - \x_1)].  
\end{align}
These two functions allows one to rewrite~\eqref{proofB.dummy1} as 
\begin{equation}\label{proofB.dummy4}
(g + G)(\x) \ni \mathbf{0}.
\end{equation}
It is also true that $(g + G)(\x_1) \ni g(\x_1)$, since for optimality $G(\x_1) \ni \mathbf{0}$. Define $F(\y) = (g + G)(\y)$, and consider the parametric generalized equation $F(\y) + \p \ni \mathbf{0}$. Due to Assumptions~\ref{as.str}-\ref{as.smooth}, and due to \cite[Theorem~2F.9]{Dontchev2009}, we have that the solution mapping $\p \mapsto \y(\p)$ of the generalized equation $F(\y) + \p \ni \mathbf{0}$ is every-where single valued and Lipschitz continuous as
\begin{equation}\label{proofB.dummy5}
\|\y(\p) - \y(\p')\| \leq \frac{1}{m} \|\p - \p'\|.
\end{equation}

Set $\p = \mathbf{0}$ and $\p' = -g(\x_1)$, then, 
\begin{equation}\label{proofB.dummy6}
\|\x - \x_1\| \leq \frac{1}{m} \|g(\x_1)\|.
\end{equation}

We proceed now to bound $\|g(\x_1)\|$. We can write $g(\x_1)$ as
\begin{equation}\label{g1_ex}
g(\x_1) = \nabla_{\x} f_k + \Q_k (\x_1- \x_k) + h\, \c_k - \nabla_{\x} f_1,
\end{equation}
As in Proposition~\ref{prop.err}, we have two cases: 
\begin{align}
\textrm{Case a)} \quad \|g(\x_1)\| \leq  & 2 L\|\x_1 - \x_k\| + 2 h\, C_0, \label{g1_bound_0} \\ 
%\end{equation}
%and
%
%CASE B
%
%which is nothing else but the error of the truncated Taylor expansion of $\nabla_{\x} f_1$, which due to Assumptions~\ref{as.str}-\ref{as.smooth}, can be upper bounded as
\textrm{Case b)} \quad  \|g(\x_1)\| \leq  &  \frac{1}{2}\, C_1 \|\x_1 - \x_k\|^2 + \nonumber \\ & \qquad h\, C_2 \|\x_1 - \x_k\| + \frac{1}{2} h^2\, C_3.  \label{g1_bound}
\end{align}
Since $\|\x_1 - \x_k\| \leq \|\x_1 - \x^*(t_k)\| + \|\x^*(t_k) - \x_k\|$, and we can bound the first term of the right-hand side by using~\eqref{eq.lip}, then 
\begin{align}
\textrm{Case a)}\, \|g(\x_1)\| \leq & 2 L\|\x^*(t_k) - \x_k\|\! + \!2 h C_0 (1 \!+\! {L}/m), \\
%\end{equation}
%and
%\begin{multline}
\textrm{Case b)}\, \|g(\x_1)\| \leq & h^2\,C_1 \frac{C_0^2}{2 m^2} + h^2\, C_2 \frac{C_0}{2 m} +  \frac{1}{2} h^2\, C_3 + \nonumber \\ & 
 \hspace*{-2.5cm}\frac{1}{2} C_1 \|\x^*(t_k) \!-\! \x_k\|^2 \!+\! h \Big(\frac{C_1 C_0}{m} \!+\! C_2 \Big) \|\x^*(t_k) \!-\! \x_k\|.
\end{align}
By combining these two last bounds with~\eqref{proofB.dummy6}, the claims~\eqref{prop_inside_0}-\eqref{prop_inside} follow.
\end{IEEEproof}

\vskip2mm


On the other hand, the distance between the approximate prediction $\tilde{\x}_{k+1|k}$ and the optimal prediction $\x_{k+1|k}$ can be bounded by using standard results for the projected gradient method, for the proof see for instance~\cite{Ryu2015,Taylor2017}.

\vskip2mm

\begin{proposition}\label{prop.intheo.2}
{\bf
Under Assumption~\ref{as.str}, we have that
\begin{equation}\label{init1}
\|\tilde{\x}_{k+1|k} - \x_{k+1|k}\| \leq \varrho_{\mathrm{P}}^{P}\,\|{\x}_{k} - \x_{k+1|k}\|, 
\end{equation}
with $\varrho_{\mathrm{P}} = \max\{|1-\alpha m|,|1 - \alpha L|\}$.
}
\end{proposition}

\vskip2mm
By putting together Propositions~\ref{prop.intheo.1} and~\ref{prop.intheo.2} and~\eqref{eq.lip} , we obtain for the total error after prediction as
\begin{subequations}
\begin{align}
\|\tilde{\x}_{k+1|k} \!- \!\x^*(t_{k+1})\| & \!\leq \!\|\tilde{\x}_{k+1|k} \!-\! \x_{k+1|k}\| \!+\! \|\x_{k+1|k}\!- \!\x^*(t_{k+1})\|\\ 
&\hspace*{-3.25cm}\leq \varrho_{\textrm{P}}^{P}\,\|{\x}_{k} \!-\! \x_{k+1|k}\| \!+\! \|\x_{k+1|k}\!-\! \x^*(t_{k+1})\|\\ 
&\hspace*{-3.25cm}\leq \varrho_{\textrm{P}}^{P}\,(\|{\x}_{k}\! - \!\x^*(t_k)\| \! +\!\|\x^*(t_k) \!-\!\x^*(t_{k+1})\| +\nonumber \\ %%
& \hspace*{-2.25cm}\!\|\x^*(t_{k+1})\! - \!\x_{k+1|k}\|)\! +\! \|\x_{k+1|k}\!-\! \x^*(t_{k+1})\| \\
&\hspace*{-3.25cm}\leq \varrho_{\textrm{P}}^{P}\,\|{\x}_{k} - \x^*(t_k)\| + \Big(\varrho_{\textrm{P}}^{P}+1\Big) \|\x_{k+1|k}- \x^*(t_{k+1})\|  +\nonumber \\ %%
& \hspace*{-2.25cm}\varrho_{\textrm{P}}^{P}\| \x^*(t_{k+1}) -  \x^*(t_{k})\|\\ \label{final.result}
&\hspace*{-3.25cm}\leq \eta_0 \|{\x}_{k} - \x^*(t_k)\|^2 +  \eta_1 \|{\x}_{k} - \x^*(t_k)\| + \eta_2,
\end{align}
\end{subequations}
where we have defined
\begin{align} \textrm{Case a)} &\quad \left\{
\begin{array}{rl}
\eta_0 &= 0, \\
%% 
\eta_1 &= \varrho_{\textrm{P}}^{P} + (\varrho_{\textrm{P}}^{P}+1) \frac{2L}{m},\\
%%
\eta_2 &= (2 \varrho_{\textrm{P}}^{P} + 1) \Delta_1, 
\end{array}\right.
\\
\textrm{Case b)}& \quad \left\{
\begin{array}{rl}
\eta_0 &= (\varrho_{\textrm{P}}^{P}+1) \frac{C_1}{2\,m}, \\
%% 
\eta_1 &= \varrho_{\textrm{P}}^{P} + h\,(\varrho_{\textrm{P}}^{P}+1) \Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m}\Big),\\
%%
\eta_2 &= \varrho_{\textrm{P}}^{P} \Big(h\,\frac{C_0}{m} + \Delta_2\Big) + \Delta_2, 
\end{array}\right.
\end{align}
where $\Delta_1$ and $\Delta_2$ are defined as in Proposition~\ref{prop.err}.
\vskip2mm

\noindent \textbf{Correction error.} We look now at the correction step, which by using standard results for the projected gradient method, we have
\begin{equation}\label{corr_eq}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \varrho_{\textrm{C}}^{C}\,\|\tilde{\x}_{k+1|k} - \x^*(t_{k+1})\|, 
\end{equation}
with $\varrho_{\textrm{C}} = \max\{|1-\alpha m|,|1 - \alpha L|\}$. And by putting together the result~\eqref{final.result} with~\eqref{corr_eq}, we obtain the recursive error bound,
\begin{multline}\label{rec}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \varrho_{\textrm{C}}^{C}\Big(\eta_0 \|{\x}_{k} - \x^*(t_k)\|^2 + \\ \eta_1 \|{\x}_{k} - \x^*(t_k)\| + \eta_2\Big).
\end{multline}

\vskip2mm

\noindent \textbf{Global error and convergence.} 

We start with Case a).
%
Call for simplicity $\bar{\eta}_i = \varrho_{\textrm{C}}^{C}\eta_i$, for $i = 0,1,2$. Since $\eta_0 = 0$, then convergence is achieved if 
\begin{equation}
\bar{\eta}_1 < 1 \iff \tau_0 = \varrho_{\textrm{C}}^{C}\left[\varrho_{\textrm{P}}^{P} + (\varrho_{\textrm{P}}^{P}+1) \frac{2L}{m}\right] < 1,
\end{equation}
which guarantees a monotonical decrease of the optimality gap with linear rate and asymptotic bound of
\begin{equation}
\limsup_{k \to \infty}\|{\x}_{k+1} - \x^*(t_{k+1})\|  = \frac{\varrho_{\textrm{C}}^{C}\Delta_1}{1-\tau_0} (2 \varrho_{\textrm{P}}^{P} + 1) = O(\varrho_{\textrm{C}}^{C} h),
\end{equation}
which are the claims in Theorem~\ref{theo.constrained_0}.

\vskip2mm
We finish with Case b).
%
Call again for simplicity $\bar{\eta}_i = \varrho_{\textrm{C}}^{C}\eta_i$, for $i = 0,1,2$. Then convergence is achieved if
\begin{enumerate}
\item[1)] Each iteration does not increase the error, so that
\begin{multline}\label{decrease}
\bar{\eta}_0 \|{\x}_{k} - \x^*(t_k)\|^2 +  \bar{\eta}_1 \|{\x}_{k} - \x^*(t_k)\| + \bar{\eta}_2 \leq \\ \tau \|{\x}_{k} - \x^*(t_k)\| + \bar{\eta}_2 
\end{multline}
for a $\tau < 1$; 
\item[2)] One can find a $\tau <1$ such that~\eqref{decrease} holds. 
\end{enumerate}
By simple algebra, convergence is achieved if $\bar{\eta}_1 < \tau < 1$, that is if 
\begin{equation}
\varrho_{\textrm{P}}^{P}\varrho_{\textrm{C}}^{C} < \tau, \quad h < \frac{\tau - \varrho_{\textrm{C}}^{C}\varrho_{\textrm{P}}^{P}}{\varrho_{\textrm{C}}^{C}(\varrho_{\textrm{P}}^{P} + 1)}\Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m} \Big)^{-1} = \bar{h},
\end{equation}
which sets the bounds on the number of prediction and correction steps as well as the sampling period, and if the initial optimality gap is chosen as
\begin{equation}
\|\x_0 - \x^*(t_0) \| \leq \frac{\tau - \bar{\eta}_1}{\bar{\eta}_0} = \bar{R}.
\end{equation}
The convergence region depends on the sampling period and on the prediction and correction steps. When $h \to 0$, then
\begin{equation}
\lim_{h\to 0} \bar{R} = \frac{2\, m}{C_1}\,\frac{\tau - \varrho_{\textrm{P}}^{P}\varrho_{\textrm{C}}^{C}}{\varrho_{\textrm{C}}^{C}(\varrho_{\textrm{P}}^{P} + 1)}. 
\end{equation}

As for the convergence asymptotical error, by using~\eqref{rec} in combination with~\eqref{decrease}, we can show that
\begin{equation}\label{final}
\|\x_k - \x^*(t_k)\| \leq \tau^{k} \|\x_0 - \x^*(t_0)\| + \bar{\eta}_2 \frac{1-\tau^{k}}{1 - \tau},
\end{equation}
from which, by letting $k \to \infty$, the result~\eqref{main.result1} follows. \qed


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PROOF OF THEOREM 2, UNCONSTRAINED CASE.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Proof of Theorem~\ref{theo.unconstrained} }\label{ap.newton}

We proceed similarly to Appendix~\ref{ap.grad}. One of the main difference is a new Proposition~\ref{prop.intheo.1} suited for the situation at hand. 

\vskip2mm 

\begin{proposition}\label{prop.intheo.1bis}
{\bf
The following facts hold true. 
\begin{enumerate}
\item[{Case a)}] Under the same assumptions and notation of Theorem~\ref{theo.unconstrained_0}, we have that
%%
\begin{equation}\label{pp_0}
\hspace*{-.5cm}\|\x_{k+1|k}\! - \!\x^*(t_{k+1})\| \!\leq\! \Big(1-\gamma + \gamma \frac{2 L}{m}\Big) \|\x_k\!-\! \x^*(t_k)\|\!+\! 2\Delta_1.
\end{equation}
%%
\item[{Case b)}] Under the same assumptions and notation of Theorem~\ref{theo.unconstrained}, we have that
\begin{multline}\label{pp}
\|\x_{k+1|k} - \x^*(t_{k+1})\| \leq \gamma\,\frac{C_1}{2\,m}\|\x_k- \x^*(t_k)\|^2 + \\\Big[1-\gamma + h\,\Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m}  \Big)\Big]\|\x_k- \x^*(t_k)\|+ \Delta_2.
\end{multline}
\end{enumerate}
}
\end{proposition}
\vskip2mm

\begin{IEEEproof}
Start by noticing that Proposition~\ref{prop.err} holds true even when $\gamma < 1$ (in the unconstrained case), since $\nabla_{\x}f(\x^*(t_k); t_k) = \nabla_{\x}f_0 = \textbf{0}$. In fact, Eq.~\eqref{proofA.dummy1} should read
\begin{equation}
\nabla_{\x} f_0 + \Q_0 (\x - \x_0) + h\, \c_0 = (1-\gamma)\nabla_{\x} f_0,
\end{equation} 
but this is in fact equivalent to the original \eqref{proofA.dummy1}, since $\nabla_{\x}f_0 = \textbf{0}$, and therefore the whole proposition is still valid, and in particular $\|\x^*_{k+1|k} - \x^*(t_{k+1})\| \leq \Delta_i$, where $i=1$ for Case a) and $i=2$ for Case b).

Call now $\delta\x_k = \x_{k+1|k} - \x_k$, and $\delta\x^*_k = \x^*_{k+1|k} - \x^*(t_k)$. Then, 
\begin{multline}
\|\x_{k+1|k} - \x^*(t_{k+1})\| = \\ \|\x_{k} + \delta\x_k - (\x^*(t_k) + \delta\x^*_k) + ( \x^*_{k+1|k} - \x^*(t_{k+1})) \|,
\end{multline}
which given Proposition~\ref{prop.err} and by using the Triangle inequality can be upper bounded as
\begin{equation}\label{b_1}
\|\x_{k+1|k} \!-\! \x^*(t_{k+1})\|\! \leq \!(1-\gamma)\|\x_{k}\! -\! \x^*(t_k)\| + \|\delta\check{\x}_k \!-\!  \delta\x^*_k\| \!+\! \Delta_i,
\end{equation}
where we have set $\delta\check{\x}_k = \delta\x_k + \gamma(\x_k - \x^*(t_k))$. Note that this decomposition may seem cumbersome, yet it is the cornerstone of the proof of this proposition.  

For $\delta\check{\x}_k$ and $\delta \x^*_k$, it holds that
\begin{align}
& \gamma\, \nabla_{\x} f_k + \gamma\, \Q_k (\x_0 - \x_k) + \Q_k \delta\check{\x}_k + h\, \c_k = \mathbf{0},\\
& \gamma \nabla_{\x} f_0 + \Q_0\delta{\x}^*_k + h\, \c_0 = \mathbf{0},
\end{align}
where as in~\eqref{simplif2} we have used the simplifications
\begin{subequations}
\begin{align}
\nabla_{\x} f_k = \nabla_{\x} f (\x_k; t_{k}), \quad & \Q_k = \nabla_{\x\x} f (\x_k; t_{k}) \\
\c_k = \nabla_{t\x} f (\x_k; t_{k}),\quad &  \x = \x_{k+1|k}.
\end{align}
\end{subequations}
while $\nabla_{\x} f_0$, $\Q_0$, $\c_0$, and $\x_0$ are defined just as in~\eqref{simplif}-\eqref{simplif22}, for $i = 0$ (i.e., $\x_0 = \x^*(t_k)$, and so on). Define
\begin{align}
g(\delta\x) &= \gamma\, (\nabla_{\x} f_k - \nabla_{\x} f_0 + \Q_k (\x_0 - \x_k)) + \nonumber \\& \hspace*{1cm} (\Q_k - \Q_0)\delta\x + h\, (\c_k-\c_0), \\
G(\delta\x) &= \gamma \nabla_{\x} f_0 + \Q_0\delta{\x} + h\, \c_0,
\end{align}
and notice that $(g + G)(\delta\check{\x}_k) = \mathbf{0}$, while $(g + G)(\delta{\x}^*_k) = g(\delta{\x}^*_k)$. With a similar argument as the one of the proof of Proposition~\ref{prop.intheo.1}, then
\begin{equation}\label{b_0}
\|\delta\check{\x}_k - \delta{\x}^*_k\| \leq \frac{1}{m} \|g(\delta{\x}^*_k)\|.  
\end{equation}
Let us now bound $\|g(\delta{\x}^*_k)\|$. 

Case a) Due to Assumptions~\ref{as.str}:
\begin{equation}\label{b_2_0}
\|g(\delta{\x}^*_k)\| \!\leq \! 2 \gamma L \|\x_k \!-\! \x_0\| + 2L\|\delta{\x}^*_k\| + 2 h\, C_0.
\end{equation}  

Case b) Due to Assumptions~\ref{as.str}-\ref{as.smooth}, 
\begin{equation}\label{b_2}
\|g(\delta{\x}^*_k)\| \!\leq \!\gamma \frac{C_1}{2}\|\x_k \!-\! \x_0\|^2 + C_1  \|\x_k - \x_0\|\|\delta{\x}^*_k\| + h\, C_2 \|\x_k \!-\! \x_0\|.  
\end{equation}

The next step of the proof is to upper bound the term $\|\delta \x^*_k\| = \|\x^*_{k+1|k} - \x^*(t_k)\|$. We know that
\begin{equation}
\gamma \nabla_{\x}f_0 + \Q_0\delta \x^*_k + h \c_0 = \mathbf{0},
\end{equation}
and since $\nabla_{\x}f_0  = \mathbf{0}$, then $\delta \x^*_k = - h\,\Q_0^{-1} \c_0$. Which yields 
\begin{equation}\label{b_3}
\|\delta \x^*_k\| \leq h\,\frac{C_0}{m}.
\end{equation}
By putting together the bounds~\eqref{b_1}, \eqref{b_0}, \eqref{b_2_0}, \eqref{b_2}, and \eqref{b_3}, the claims~\eqref{pp_0} and \eqref{pp} follow. 
\end{IEEEproof}


\vskip2mm
By using Proposition~\ref{prop.intheo.1bis} along with the same arguments as the one in Eq.s~\eqref{init1} till \eqref{rec}, we arrive at the error recursion
\begin{equation}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \bar{\eta}_0' \|{\x}_{k} - \x^*(t_k)\|^2 +  \bar{\eta}_1' \|{\x}_{k} - \x^*(t_k)\| +  \bar{\eta}_2',
\end{equation}
where,
\begin{equation}
\textrm{Case a)}\, \left\{
\begin{array}{rl}
\bar{\eta}_0' &= 0, \\
%% 
\bar{\eta}_1' &= \varrho_{\textrm{C}}^{C} \left[\varrho_{\textrm{P}}^{P} +  (\varrho_{\textrm{P}}^{P}+1)\Big(1-\gamma +\gamma \frac{2L}{m}\Big)\right],\\
%%
\bar{\eta}_2' &=  \varrho_{\textrm{C}}^{C} \left[2 (2 \varrho_{\textrm{P}}^{P} + 1) \Delta_1\right],
%%
\end{array}\right.
\end{equation}
\begin{multline}
\hspace*{-1mm}\textrm{Case b)}\\ \left\{
\begin{array}{rl}
\bar{\eta}_0' &= \gamma \varrho_{\textrm{C}}^{C}(\varrho_{\textrm{P}}^{P}+1) \frac{C_1}{2\,m}, \\
%% 
\bar{\eta}_1' &= \varrho_{\textrm{C}}^{C}\Big[\varrho_{\textrm{P}}^{P} + (\varrho_{\textrm{P}}^{P}+1)\Big( 1-\gamma + h\, \Big(\frac{C_1 C_0}{m^2} + \frac{C_2}{m}\Big)\Big)\Big],\\
%%
\bar{\eta}_2' &= \varrho_{\textrm{C}}^{C}\Big[\varrho_{\textrm{P}}^{P} \Big(h\,\frac{C_0}{m} + \Delta_2\Big) + \Delta_2\Big]. 
\end{array}\right.
\end{multline}
\vskip2mm
By using now the same reasoning as in Eq.s~\eqref{decrease} till Eq.s~\eqref{final}, the claims~\eqref{main.result2_0}-\eqref{main.result2} can be proven.  
\qed


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> arXiv Version 2/Proofs_1.tex <==

% !TEX root = TimeVarying_part1.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\section{Proof of Proposition~\ref{prop.err}}\label{ap.prop}

For the forward Euler method applied to the nonlinear dynamical system
%%%
\begin{equation}\label{proof_100}
\dot{x} = {\mathcal{F}}(x,t),
\end{equation}
%%%
the local discretization error is bounded by~\cite[Chapter~11]{Quarteroni2000} $h^2/2\, \|\mathrm{d}\mathcal{F}(x,t)/\mathrm{d}t\|$. We can extend this result, by considering that the forward Euler method is based on a truncated Taylor series expansion. Let us analyze the forward Euler method applied to the vector-valued nonlinear dynamical system
%%%
\begin{equation}\label{proof_110}
\dot{\x} = {\mathbold{F}}(\x,t).
\end{equation}
%%%
If we apply the forward Euler method to the relation in \eqref{proof_110}, starting at a certain point $\x(t_k)$, we obtain 
%%%
\begin{equation}\label{proof_120}
\x_{k+1} = \x(t_k)+ {\mathbold{F}}(\x(t_k),t_k)\, h. 
\end{equation}
%%%
Subtracting $\x(t_{k+1})$ from the both sides of the equality in \eqref{proof_120} and computing the norm of the resulted relation implies that
%%%
\begin{equation}\label{proof_130} 
\|\x_{k+1} - \x(t_{k+1})\| =  \left\|{\mathbold{F}}(\x(t_k),t_k)\, h  -\int_{t_k}^{t_{k+1}} \!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau \right\|.
\end{equation}
%%%%%
Notice that \eqref{proof_130} is resulted by considering the relation $\x(t_{k+1}) = \x(t_{k}) +\int_{t_k}^{t_{k+1}} {\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau$. Observe that according to the Mean Value theorem there exits a $\hat{\tau} \in [t_k, t_{k+1}]$ that satisfies 
%%%
\begin{equation}\label{proof_140} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau = \int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(t_k),t_k) + \nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,h \, \textrm{d} \tau.
\end{equation}
%%%%%
Notice that the term ${\mathbold{F}}(\x(t_k),t_k)$ does not depend on the integral variable $\tau$. Considering this observation and observing the definition $h:=t_{k+1}-t_k$, we can simplify the first part of the integral in the right hand side of \eqref{proof_140} as 
%
\begin{equation}\label{proof_145} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(t_k),t_k)  \textrm{d} \tau= {\mathbold{F}}(\x(t_k),t_k) h \; .
\end{equation}
%
 Since $\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau})$ is also not a function of variable $\tau$,   by applying the same argument we can simplify the second part of the integral in the right hand side of \eqref{proof_140} as
 %
 \begin{equation}\label{proof_147} 
  \int_{t_k}^{t_{k+1}}\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,h \, \textrm{d} \tau=\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,(h^2)/2 \;.
  \end{equation}
   Therefore, we can rewrite \eqref{proof_140} as 
%%%
\begin{equation}\label{proof_150} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau = {\mathbold{F}}(\x(t_k),t_k)\ \!h + \nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,\frac{h^2}{2}.
\end{equation}
%%%%%
By substituting the integral $\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau$ in \eqref{proof_130} by the simplification in \eqref{proof_150} and considering the definition of the discretization error vector $\mathbold{\Delta}:=\x_{k+1} - \x(t_{k+1})$ we can rewrite \eqref{proof_130} as
%%%
\begin{equation}\label{proof_160} 
\|\mathbold{\Delta} \|=  \frac{h^2}{2} \|\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau})\|.
\end{equation}
%%%%%
Observing the continuous dynamical system in \eqref{eq.dyn} we know that ${\mathbold{F}}(\x,t)$ is given by
%%%
\begin{equation}\label{proof_170} 
{\mathbold{F}}(\x,t) = -[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t).
\end{equation}
%%%%%
We proceed to find an upper bound for the right hand side of \eqref{proof_160}. Note that based on the definition in \eqref{proof_170} we can write 
%%%
\begin{align}\label{proof_180} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|= \left\|\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]\right\|
\end{align}
%%%%%
Notice that by applying the chain rule we can simplify the derivative $\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]$ as
%%%
\begin{align}\label{proof_190} 
&\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]=\\
&\qquad\qquad\qquad[\nabla_{\x\x}f(\x; t)]^{-2} \nabla_{t \x\x}f(\x; t) \nabla_{t\x}f(\x; t)\nonumber\\
&
\qquad\qquad\qquad+ [\nabla_{\x\x}f(\x; t)]^{-1}\nabla_{tt\x}f(\x; t)\nonumber.
\end{align}
%%%%%
Compute the norm of both sides of \eqref{proof_190}. Substitute the norm $\|\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]\|$ by $\|\nabla_{t}{\mathbold{F}}(\x,t) \|$ as shown in \eqref{proof_180}. Further apply the triangle inequality to the right hand side of the resulted expression to obtain 
%%%
\begin{align}\label{proof_200} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|&\leq\left\|[\nabla_{\x\x}f(\x; t)]^{-2} \nabla_{t \x\x}f(\x; t) \nabla_{t\x}f(\x; t)\right\|\nonumber\\
&
\quad+ \left\|[\nabla_{\x\x}f(\x; t)]^{-1}\nabla_{tt\x}f(\x; t)\right\|.
\end{align}
%%%%%
Observe the fact that $\nabla_{t \x\x}f(\x; t) = \nabla_{\x t\x}f(\x; t)$. We use the Cauchy-Schwartz inequality and the bounds in Assumptions \ref{as.str} and  \ref{as.smooth} to update the upper bound in \eqref{proof_200} as
%%%
\begin{align}\label{proof_210} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|  \leq \frac{C_0 C_2}{m^2} + \frac{C_3}{m}
\end{align}
%%%%%
Combining the relation in \eqref{proof_160} and the upper bound in \eqref{proof_210} follows the claim in \eqref{prop_claim_err_bound}.
%%
\qed 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem \ref{th.GTT_convg}}\label{app.GTT_convg}


In order to prove Theorem \ref{th.GTT_convg}, we start by bounding the error in the prediction step by the terms that depend on the functional smoothness and the discretization error using Taylor expansions. Then we bound the tracking error of the gradient step using standard convergence properties of gradient descent on strongly convex functions. By substituting the error improvement achieved in the correction step into the prediction step, we establish the main result.

First, we establish that the criteria in which the bound stated in \eqref{result1} may be satisfied, i.e. that $\rho \sigma$ can be made strictly less than 1, for a sufficiently small $h$. Note that, since $m>0$, there is always a $\gamma$ that makes $\rho < 1$ since $\gamma < m/L^2$. In particular, if we take $\gamma = m/ 2 L^2$, then $\rho$ is minimized and it is equal to 
%
\begin{equation}\label{rho}
\rho^* = \sqrt{ 1 - \frac{m^2}{4 L^2}}. 
\end{equation}
%
The coefficient $\sigma$ is a monotonically increasing function in $h$, and it is equal to $1$ when $h = 0$; by continuity of $\sigma$ in $h$, we can always find a small enough stepsize $h$, such that $\sigma < 1/\rho^*$, which means that we can find a stepsize $\gamma$ that yields $\rho \sigma <1$.

Now we turn to establishing the discrete-time sampling error bound stated in \eqref{result1} is achieved by the updates \eqref{GTT_prediction}-\eqref{GTT_correction}. For simplicity, we modify the notation to omit the arguments $\x_k$ and $t_k$ of the function $f$. In particular, define 
%
\begin{align}\label{eq:thm1_defs}
&\nabla_{\x\x}f = \nabla_{\x\x}f(\x_k; t_k)\; , &&\nabla_{t\x} f = \nabla_{t\x} f(\x_k; t_k)\;,\nonumber \\ 
&\nabla_{\x\x}f^* = \nabla_{\x\x}f({\x}^*(t_{k}); t_k)\;,  && \nabla_{t\x} f^* = \nabla_{t\x} f({\x}^*(t_{k}); t_{k}) \; . \nonumber
\end{align}
%
Begin by considering the update~\eqref{GTT_prediction}, the prediction step, evaluated at a generic point $\x_k$ sampled at the current sample time $t_k$ and with associated optimizer $\x^*(t)$, which due to optimality will have null residual vector $\r(t) = \mathbf{0}$. Thus we may write
%
\begin{equation}\label{eq:null_residual}
\left\{\begin{array}{rcl}
{\x}_{k+1|k} &=& \x_{k} - [\nabla_{\x\x}f]^{-1}\nabla_{t\x} f\,h\\
{\x}^*(t_{k+1}) &=& {\x}^*(t_{k}) - [\nabla_{\x\x}f^*]^{-1} \nabla_{t\x} f^*\,h + \Delta.
\end{array}\right.
\end{equation}
%
By subtracting one from the other and by considering the norm of the result, we obtain 
%
\begin{align}\label{eq.imp}
\|{\x}_{k+1|k}& -  \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\|  \\  & + \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h + \|\mathbold{\Delta}\| .\nonumber 
\end{align}
%
Define $a$ as the second term in the right-hand side of \eqref{eq.imp}, as  $a= \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h$. We may rewrite $a$ by adding and subtracting the Newton step with the Hessian evaluated at the current optimal point,  $[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f$, to obtain
%
\begin{align}\label{eq.hessian_cross_term}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h,
\end{align}
%
We may bound the first and second-order derivative terms in the previous expression \eqref{eq.hessian_cross_term} by using Assumption~\ref{as.smooth} regarding the functional smoothness as well as the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} to write
%
\begin{equation}\label{eq.a}
a  \leq C_0 h \left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We now further bound the first term of the right-hand-side. To do that, we use the non-singularity of the Hessian to write 
%
\begin{multline}\label{eq.dummy10_midstep}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| = \\ \|[\nabla_{\x\x}f^*]^{-1}(\nabla_{\x\x}f - \nabla_{\x\x}f^*)[\nabla_{\x\x}f]^{-1} \|,
\end{multline} 
%
which by employing, once again, the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} we can bound as
\begin{equation}\label{eq.dummy10}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| \leq \frac{1}{m^2}\|\nabla_{\x\x}f - \nabla_{\x\x}f^* \|,
\end{equation} 
%
and therefore~\eqref{eq.a} can be written as
\begin{equation}\label{eq.amid}
a  \leq \frac{C_0}{m^2} h \left\|\nabla_{\x\x}f - \nabla_{\x\x}f^*\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We consider the Taylor expansion of the mixed second-order terms and the second-order terms in \eqref{eq.amid}, and apply the Mean Value Theorem with $\tilde{\x}$ as a point on the line between $\x_k$ and $\x^*(t_k)$ to obtain the following expressions,
%
%\begin{subequations}
\begin{align} \label{eq.dummy11}
\left\| \nabla_{\x\x} f- \nabla_{\x\x} f^*  \right\| &
\leq \left\|\nabla_{\x \x\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \nonumber\\ 
&\leq C_1 \|\x_k - \x^*(t_k)\| \\
%\end{multline}
%\begin{multline}
\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| &
\leq \left\|\nabla_{\x t\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \nonumber \\
& \leq C_2 \|\x_k - \x^*(t_k)\| \label{eq.dummy111}
\end{align}
%\end{subequations}
%
The expressions in \eqref{eq.dummy11} - \eqref{eq.dummy111} may be substituted together into~\eqref{eq.amid} to yield
 %
\begin{align}
a  &\leq \frac{C_0 C_1 h}{m^2}\|\x_k - \x^*(t_k)\| + \frac{C_2 h}{m}\|\x_k - \x^*(t_k)\|.
\end{align}
%
Now we can use this bound for $a$ in~\eqref{eq.imp} to get
%
\begin{align}\label{some_bound}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq&  \Big[1 + h\left(\frac{C_0 C_1 h}{m^2} + \frac{C_2 h}{m}\right) \Big] \times \nonumber \\
& \quad \|{\x}_{k} - \x^*(t_{k})\| + \|\mathbold{\Delta}\|.
\end{align}
%
By considering the definition of $\sigma$ in \eqref{thm:rho_sigma} and substituting the discretization error norm $\|\mathbold{\Delta}\|$ by its upper bound in \eqref{prop_claim_err_bound}, we obtain that
%
\begin{equation}\label{eq.fin1}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \sigma \|{\x}_{k} - \x^*(t_{k})\| + \frac{h^2}{2}\left[\frac{C_0 C_2}{m^2} + \frac{C_3}{m}\right] .
\end{equation}
%
For the correction step [cf. \eqref{GTT_correction}] , we may use the standard property of projected gradient descent for strongly convex functions. In particular, the gradient converges Q-linearly as
%
\begin{equation}\label{eq.fin2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\| \leq \rho \|{\hat{\x}}_{k+1}^{s} - \x^*(t_{k+1})\| .
\end{equation}
%
where $\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}$. To see this, it is sufficient to write the projected gradient step as 
\begin{multline}\label{eq.explanation1}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 = \\  \|P_X[{\hat{\x}}_{k+1}^{s} -\gamma \nabla_{\x} f(\hat{\x}_{k+1}^s; t_{k+1})] - \x^*(t_{k+1})\|^2 .
\end{multline}
Since $\x^*(t_{k+1}) = P_X[\x^*(t_{k+1})-\gamma\nabla_{\x} f(\x^*(t_{k+1}), t_{k+1})]$ for optimality, and since the projection is nonexpansive, we obtain 
\begin{multline}\label{eq.explanation2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 \leq  \|{\hat{\x}}_{k+1}^{s}  - \x^*(t_{k+1}) \\- \gamma (\nabla_{\x} f(\hat{\x}_{k+1}^s; t_{k+1}) - \nabla_{\x} f(\x^*(t_{k+1}), t_{k+1}) )\|^2 .
\end{multline}
By expanding the right-hand side and by the strong convexity and functional smoothness assumptions (Assumptions~\ref{as.str} and \ref{as.smooth}), we can write
\begin{equation}\label{eq.explanation2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 \! \leq \! (1+\gamma^2L^2-\gamma m)\|{\hat{\x}}_{k+1}^{s} - \x^*(t_{k+1})\|^2 .
\end{equation}
which is~\eqref{eq.fin2}. 
%see \cite{Nesterov2004} for further details. 
%
%
%
Observe that the sequence ${\hat{\x}}_{k+1}^{s}$ is initialized by the predicted variable $\x_{k+1|k}$ and the corrected variable $\x_{k+1}$ is equal to $ {\hat{\x}}_{k+1}^{\tau}$. Considering these observation and the relation in \eqref{eq.fin2} between two consecutive iterates of the sequence ${\hat{\x}}_{k+1}^{s}$ we can write 
%
\begin{equation}\label{eq.fin222}
\|{{\x}}_{k+1}- \x^*(t_{k+1})\| \leq \rho^\tau \|\x_{k+1|k} - \x^*(t_{k+1})\| .
\end{equation}
%
We are ready to consider the combined error bound achieved by the prediction-correction scheme. By plugging the correction error in \eqref{eq.fin222} into the prediction error in \eqref{eq.fin1} we obtain
%
\begin{equation}\label{eq.fin_t_k}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^\tau \sigma \|{\x}_{k} - \x^*(t_{k})\| +  \rho^\tau \Gamma,
\end{equation}
%
where $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$ is defined to simplify the notation. Notice that the relation between $\|{\x}_{k+1} - \x^*(t_{k+1})\|$ and $\|{\x}_{k} - \x^*(t_{k})\| $ in \eqref{eq.fin_t_k} is also holds true for $\|{\x}_{k} - \x^*(t_{k})\| $ and $\|{\x}_{k-1} - \x^*(t_{k-1})\| $. I.e., 
%
\begin{equation}\label{eq.fin_t_k_1}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^\tau \sigma \|{\x}_{k-1} - \x^*(t_{k-1})\| +  \rho^\tau \Gamma.
\end{equation}
%
Substituting the upper bound in \eqref{eq.fin_t_k_1} for $\|{\x}_{k} - \x^*(t_{k})\|$ into \eqref{eq.fin_t_k} implies an upper bound for $\|{\x}_{k+1} - \x^*(t_{k+1})\| $ in terms of the norm difference for time $k-1$ as
%
\begin{align}\label{eq.fin_t_k_new}
\|{\x}_{k+1} - \x^*(t_{k+1})\| &\leq (\rho^\tau \sigma)^2 \|{\x}_{k-1} - \x^*(t_{k-1})\|
\nonumber \\
& \qquad +\rho^\tau \Gamma(\rho^\tau \sigma+1) .
\end{align}
%
Now recursively apply the relationship \eqref{eq.fin_t_k} backwards in time to the initial time sample and use the same argument form \eqref{eq.fin_t_k} to \eqref{eq.fin_t_k_new} to write 
%
\begin{equation}\label{eq.fin_t_00}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq (\rho^\tau \sigma)^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \rho^\tau \Gamma \sum_{i=0}^k (\rho^\tau\sigma)^i.
\end{equation}
%
Substituting $k+1$ by $k$ and simplifying the sum in \eqref{eq.fin_t_00} leads to
%
\begin{equation}\label{eq.fin_t_0000}
\|{\x}_{k} - \x^*(t_{k})\| \leq (\rho^\tau \sigma)^{k} \|{\x}_{0} - \x^*(t_{0})\| + \rho^\tau \Gamma \left[ \frac{1-(\rho^\tau\sigma)^k}{1-\rho^\tau\sigma}\right].
\end{equation}
%
Considering the result in \eqref{eq.fin_t_0000} and the definition for the constant $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$, the result in \eqref{result1} follows.

To establish the result stated in \eqref{result2}, observe that in the worst case, we may upper bound the term $a$ in \eqref{eq.amid} by using the bounds in Assumption \ref{as.smooth} to obtain the right hand side of the following expression 
%
\begin{align}\label{eq.worst_case}
a  
 & \leq \frac{2 C_0 L h}{m^2} + \frac{2 C_0 h}{m}.
\end{align}
%
Remembering the definition of the nonnegative scalar term $a:=\left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h $ and substituting the bound~\eqref{eq.worst_case} into \eqref{eq.imp}, we can write
%
\begin{multline}\label{eq.a_subst}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\| \\ + h\left(\frac{2 C_0 L }{m^2} + \frac{2 C_0 }{m}\right) +  \|\mathbold{\Delta}\|.
\end{multline}
%
To simplify the notation we define a new constant $\Gamma_2:= h\left(({2 C_0 L }/{m^2} )+ ({2 C_0 }/{m})\right)$. Considering this definition and observing the  the relation in \eqref{eq.fin222} we can write 
%
\begin{equation}\label{eq.sampling_error2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^\tau \|{\x}_{k} - \x^*(t_{k})\| + \rho^\tau (\Gamma_2 + \Gamma).
\end{equation}
%
%
Now recursively apply the relationship \eqref{eq.sampling_error2} backwards in time to the initial time sample and use the same argument form \eqref{eq.fin_t_k} to \eqref{eq.fin_t_0000} to write 
%
\begin{multline}\label{eq.rho_error_dependence}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^{\tau(k+1)} \|{\x}_{0} - \x^*(t_{0})\| \\ +  \rho^\tau (\Gamma_2 + \Gamma) \left[ \frac{1-\rho^{\tau (k+1)}}{1-\rho^\tau}\right].
\end{multline}
%
Note that relation \eqref{eq.rho_error_dependence} shows an upper bound for $\|{\x}_{k+1} - \x^*(t_{k+1})\|$ in terms of the initial error $\|{\x}_{0} - \x^*(t_{0})\|$ and an extra error term for the bound of convergence. If we substitute $k+1$ by $k$ in \eqref{eq.rho_error_dependence} and recall the definition $\Gamma_2:= h\left(({2 C_0 L }/{m^2} )+ ({2 C_0 }/{m})\right)$ and $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$, then the result in \eqref{result2} follows.
%%
\qed

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem~\ref{th.NTT_convg} }\label{ap.newton}

We consider once again the proof of Theorem~\ref{th.GTT_convg}, in particular Equation~\eqref{some_bound} for $k = 0$, due to the prediction step. For the correction step, if we applied one time the Newton step, we would have that
\begin{equation}\label{eq.dummy300}
\|\x_{1} - \x^*(t_{1})\| \leq  (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \frac{\gamma C_1}{2 m} \|\x_{1|0} - \x^*(t_{1})\|^2.
\end{equation}
The reason for~\eqref{eq.dummy300} is explained as follows: Define
\begin{align}%\label{eq:thm1_defs2}
&\nabla_{\x\x}f_1 = \nabla_{\x\x}f(\x_{1|0}; t_1)\; , &&\nabla_{\x} f_1 = \nabla_{\x} f(\x_{1|0}; t_1)\;,\nonumber \\ 
&\nabla_{\x\x}f^*_1 = \nabla_{\x\x}f({\x}^*(t_{1}); t_1)\;,  && \nabla_{\x} f^*_1 = \nabla_{\x} f({\x}^*(t_{1}); t_{1}) \; . \nonumber
\end{align}
We can write, by applying one Newton step
\begin{align}
\|\x_{1} - \x^*(t_{1})\| &=  \|P_X[\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1]- \x^*(t_{1})\| \nonumber \\
& = \|P_X[\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1]- P_X[\x^*(t_{1})]\| \nonumber \\
& \leq \|\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1- \x^*(t_{1})\|, \label{eq.aryan1}
\end{align}
where we have used the fact that $\x^*(t_{1}) \in X$ and the nonexpansive property of the projection. We can now expand the right-hand side of~\eqref{eq.aryan1} as
\begin{equation}\label{eq.aryan2}
(1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma\|\x_{1|0} - \x^*(t_{1}) - \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1\|,
\end{equation}
which can be further upper bounded as 
\begin{align}
\eqref{eq.aryan2} & \leq (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma\|\nabla_{\x\x}f_1^{-1}\|\times \nonumber \\ &\qquad\qquad\qquad\|\nabla_{\x\x}f_1(\x_{1|0} - \x^*(t_{1})) - \nabla_{\x}f_1\| \nonumber \\ 
&\leq (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma \frac{C_1}{2 m}\| \x_{1|0} - \x^*(t_{1})\|^2,\label{eq.aryan3}
\end{align}

\textbf{Maybe expand this one!}

where the last inequality comes from the Assumption~\ref{as.smooth}, and in particular the Lipschitz continuity of the Hessian~[cfr.~\cite[Chapter~1]{Nesterov2004}]. By plugging the bound~\eqref{eq.aryan3} into~\eqref{eq.aryan1} the claim~\eqref{eq.dummy300} follows. 

Consider now $\gamma = 1$ and multiple Newton steps: we have,
\begin{equation}\label{eq.dummy30}
\|\x_{1} - \x^*(t_{1})\| \leq  \left(\frac{C_1}{2 m}\right)^{2\tau - 1}\hskip-2mm \left(\|\x_{1|0} - \x^*(t_{1})\|\right)^{2 \tau}.
\end{equation}
In order to ease the notation, we define $p_k$ as $\|\x_{k} - \x^*(t_{k})\|$ and $q = 2\tau -1$. By substituting~\eqref{eq.dummy30} into the bound on the predictions step~\eqref{some_bound}, we obtain, 
\begin{equation}\label{eq.dummy31}
p_1 \leq \left(\frac{C_1}{2 m}\right)^q  \left(\sigma p_0 + \|\mathbold{\Delta}\| \right)^{2\tau}.
\end{equation}
Due to strong convexity and Lipschitz continuity of the gradient (Assumptions~\ref{as.str} and \ref{as.smooth}), and the fact that at optimality the gradient vanishes, we can write
\begin{align}
\|\nabla_x f(\x_0, t_0)\| &= \|\nabla_x f(\x_0, t_0) - \nabla_x f^*_0\| \nonumber \\&\hspace*{-1.5cm}\geq (\nabla_x f(\x_0, t_0) - \nabla_x f^*_0)^\transp(\x_{0} - \x^*(t_0))/\|\x_{0} - \x^*(t_0)\| \nonumber \\  &\geq  m \|\x_{0} - \x^*(t_0)\|, 
\end{align}
\begin{equation}
\|\nabla_x f(\x_1, t_1)\| = \|\nabla_x f(\x_1, t_1) - \nabla_x f^*_1\| \leq L \|\x_{1} - \x^*(t_1)\|.
\end{equation}
Calling.. , due to , the inequality~\eqref{eq.dummy31} implies, 
\begin{equation}\label{eq.dummy31aryan}
g_1 \leq \frac{1}{L}\,\left(\frac{C_1}{2 m}\right)^q  \left(\sigma/m \,g_0 + \|\mathbold{\Delta}\| \right)^{2\tau}.
\end{equation}
and by recalling that by the local convergence hypothesis we have $g_0 \leq \beta\|\mathbold{\Delta}\|$, then
\begin{equation}\label{eq.dummy32}
g_1 \leq  \frac{1}{L} \left(\frac{C_1}{2 m}\right)^{q} \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau}.
\end{equation}

To enforce convergence of the sequence $\{g_k\}$, we need first to make sure that $g_1 \leq g_0$:
\begin{equation}\label{eq.dummy33}
\frac{1}{L}\left(\frac{C_1}{2 m}\right)^{q} \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau} \leq g_0 \leq \beta \|\mathbold{\Delta}\|,
\end{equation}
which yields
\begin{equation}\label{eq.dummy34}
\frac{C_1}{2 m}\|\mathbold{\Delta}\| \leq  \frac{(\beta\, L) ^{1/q}}{\left(\sigma/m\, \beta + 1 \right)^{2\tau/q}}.
\end{equation}
If condition~\eqref{eq.dummy34} is satisfied, then $g_1 \leq g_0$. By induction on $g_k$, one can show that under~\eqref{eq.dummy34}, it is also true that 
\begin{equation}\label{eq.dummy35}
g_k \leq \beta\,\|\mathbold{\Delta}\|, \quad \text{ for all } k\geq 1,
\end{equation}
or, by using again the strong convexity assumption
\begin{equation}\label{eq.dummy35}
p_k \leq g_k/m \leq \beta/m\,\|\mathbold{\Delta}\|, \quad \text{ for all } k\geq 1,
\end{equation}
which is the claim~\eqref{..}.

If we want to make sure to have a smaller asymptotical error (and quadratic convergence of the Newton method), then we need to change~\eqref{eq.dummy33} and enforce
\begin{equation}\label{eq.dummy36}
\frac{1}{L}\left(\frac{C_1}{2 m}\right)^{2\tau - 1}\hskip-2mm \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau} \leq \beta \|\mathbold{\Delta}\|^{2\tau}.
\end{equation}
Since $\|\mathbold{\Delta}\| \leq 1$ this condition is stronger than~\eqref{eq.dummy33} and implies $g_1 \leq g_0$. By solving~\eqref{eq.dummy36}, we obtain the condition:
\begin{equation}\label{eq.dummy37}
\left(\frac{C_1}{2 m}\right)^{q}  \leq \frac{\beta L}{\left(\sigma \beta + 1 \right)^{2\tau}},
\end{equation}
In particular, if this condition is satisfied then, 
\begin{equation}\label{eq.dummy38}
p_k \leq g_k/m \leq \beta/m \,\|\mathbold{\Delta}\|^{2\tau}, \quad \text{ for all } k\geq 1.
\end{equation}
%%%
which is . 
\qed


\section{Proof of Theorem~\ref{th.AGT_convg} }\label{ap.agt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     P  R   O  O   F    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We prove Theorem~\ref{th.AGT_convg} by evaluating the extra error term coming from the approximate time derivative in~\eqref{fobd}. In particular, by Taylor expansion, one can see that
\begin{equation}\label{appder_oh}
\|\tilde{\nabla}_{t\x}{f}_k  - {\nabla}_{t\x}{f}(\x_k; t_k)\| = O(h),  
\end{equation} 
In fact, one Taylor expands
\begin{align}
{\nabla}_{\x}{f}(\x_{k-1}; t_{k-1})  =& {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h \nonumber \\
& \quad + {\nabla}_{tt\x}{f}(\x(\tau); \tau) {h^2}/{2},
\end{align} 
for a particular choice of $\tau\in[t_{k-1}, t_k]$. By solving for ${\nabla}_{t\x}{f}(\x_k; t_k)$, 
\begin{align}
{\nabla}_{t\x}{f}(\x_k; t_k) = \frac{1}{h} ( {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h \nonumber \\
 + {\nabla}_{tt\x}{f}(\x(\tau); \tau) {h^2}/{2}).
\end{align}
By substituting this result and the definition~\eqref{fobd} into~\eqref{appder_oh}, the $O(h)$ error bound is proven. 

Consider now the approximate prediction step, 
\begin{equation}
\x_{k+1|k} = \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h,
\end{equation}
which by adding and subtracting the exact prediction direction becomes, 
\begin{align}
\x_{k+1|k} &= \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h + \nonumber \\ 
&\quad 
+[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h  \nonumber \\ 
&\quad - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h.
\end{align}
By following the same steps as in Theorem~\ref{th.GTT_convg}, the term $a$ in Equation~\eqref{eq.hessian_cross_term} can be written with an extra error term as, 
\begin{align}\label{eq.hessian_cross_term_2}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\
 &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h \nonumber \\ &\quad + \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h.
\end{align}
%
The extra error term w.r.t. Equation~\eqref{eq.hessian_cross_term} can be further bounded by using~\eqref{appder_oh} and the smoothness Assumption~\ref{as.smooth} (with the strong convexity constrant $m$)
\begin{align}\label{dummy_101}
& \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h  \nonumber\\
&\quad \leq \|[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1}\| \| {\nabla}_{t\x}{f}(\x_k; t_k)  - \tilde{\nabla}_{t\x}{f}_k \| \, h  \nonumber\\
&\quad \leq \frac{1}{m} \|{\nabla}_{tt\x}{f}(\x(\tau); \tau) {h}/{2}\| \, h = \frac{C_3}{m}\,\frac{h^2}{2}.
\end{align}
By adding this extra error term in the bounds~\eqref{some_bound} and \eqref{eq.a_subst} and proceeding in similar fashion as in the proof of Theorem~\ref{th.GTT_convg}, claims~\eqref{result2a} and \eqref{result1a} can be easily proven. 
%
\qed

\section{Proof of Theorem~\ref{th.ANT_convg} }\label{ap.ant}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     P  R   O  O   F    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The proof of Theorem~\ref{th.ANT_convg} is based on the proof of Theorems~\ref{th.NTT_convg} and \ref{th.AGT_convg}. In particular, the use of an approximate time derivative yields an additional error term equivalent to $({C_3}/{m})\,({h^2}/{2})$ as shown in~\eqref{dummy_101}. This means that~\eqref{eq.dummy31} will now read
\begin{align}
p_1 &\leq \left(\frac{C_1}{2 m}\right)^{q} \left(\sigma p_0 + \|\mathbold{\Delta}\| + \frac{C_3}{m}\,\frac{h^2}{2} \right)^{2\tau} \nonumber \\
 &= \left(\frac{C_1}{2 m}\right)^q (\sigma p_0 + D)^{2\tau} \; ,
\end{align}
where we have used the definition of the cumulative error $D$. The rest follows as in the proof of Theorem~\ref{th.NTT_convg}.
%
\qed


==> arXiv Version 2/Simulations.tex <==
% !TEX root = Double.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%S I M U L A T I O N S %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical Experiments}\label{sec:num}

In this section, we report three numerical examples to showcase the performance of the proposed algorithms. First, we analyze the unconstrained case (Algorithm~\ref{algo_fou}), then we switch our attention to the constrained one (Algorithm~\ref{algo_fo}). Finally, we present a realistic simulation stemming from real-time control of energy resources. 

\subsection{Unconstrained example}

%\textcolor{red}{[Comment: not sure we should leave the unconstrained example; after all, this paper is focused on constrained problems]}

We use the same scalar example of~\cite[Section~IV.A]{Paper1}, and in particular we consider a time-varying cost function of the form
%%
\begin{equation}\label{eq:scalar}
\min_{x \in \reals} f(x; t): = \frac{1}{2}\left(x - \cos(\omega t)\right)^2 + \kappa \log[1 + \exp(\mu x)]. 
\end{equation} 
The function in \eqref{eq:scalar} represents, for instance, the goal of staying close to a periodically varying trajectory plus a logistic term that penalizes large values of $x$. The terms $\omega$, $\kappa$, and $\mu$ are arbitrary nonnegative scalar parameters. In our experiments these parameters are set to $\omega = \pi/2$, $\kappa = 2$, and $\mu = 1.75$. The function $f(x; t)$  satisfies all the conditions in Assumptions \ref{as.str} and \ref{as.smooth}. In particular, $m = 1$ and $L = 2.53$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
%\psfragfig*[width=0.75\textwidth, trim=0 -0.1cm 0 0, clip=on]{Figure/Fig1Rev}
{
\psfrag{x}[c]{\footnotesize Sampling time $t_k$}
\psfrag{y}[c]{\footnotesize Tracking error $\|x_k - x^*(t_k)\|$}
\psfrag{runninggradientgradientgradientgradient}{\footnotesize \footnotesize U-FOPC, $P=0$, $C=3$, $\gamma = 0$}
\psfrag{gradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 0$}
\psfrag{approxgradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 1$}
\psfrag{newton3}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 0$}
\psfrag{newton4}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 1$}
\psfrag{newton}{\footnotesize\footnotesize U-FOPC, $P=3$, $C=3$, $\gamma = 0$}
\psfrag{newton2}{\footnotesize \footnotesize U-FOPC, $P=3$, $C=3$, $\gamma = 1$}
}
\includegraphics[width=0.5\textwidth]{Figure/Fig1Rev}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/first_error_t.pdf}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/error_t_with_bounds.pdf}
\caption{Error with respect to the sampling time $t_k$ for different algorithms applied to the scalar problem~\eqref{eq:scalar}, with $h = 0.1$.}
\label{fig.centr1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
%\psfragfig*[width=0.75\textwidth, trim=0 -0.1cm 0 0, clip=on]{Figure/Fig2Rev}
{
\psfrag{x}[c]{\footnotesize Sampling period $h$}
\psfrag{y}[c]{\footnotesize Asymptotical worst-case error}
\psfrag{runninggradientgradientgradientgradient}{\footnotesize \footnotesize U-FOPC, $P=0$, $C=3$, $\gamma = 0$}
\psfrag{gradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 0$}
\psfrag{approxgradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 1$}
\psfrag{newton3}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 0$}
\psfrag{newton4}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 1$}
\psfrag{newton}{\footnotesize U-FOPC, $P=3$, $C=3$, $\gamma = 0$}
\psfrag{newton2}{\footnotesize  U-FOPC, $P=3$, $C=3$, $\gamma = 1$}
\psfrag{oh}{\footnotesize $O(h)$}
\psfrag{oh2}{\footnotesize  $O(h^2)$}
}
\includegraphics[width=0.5\textwidth]{Figure/Fig2rev}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/first_error_h.pdf}
\caption{Asymptotical worst case error floor with respect to the sampling time interval $h$ for different algorithms applied to the scalar problem~\eqref{eq:scalar}.}
\label{fig.centr2}
\end{figure}

We choose the constant stepsizes as $\alpha = \beta = 0.56< 2/L$ in the gradient methods stated in Algorithm~\ref{algo_fou} and initialize $x_0=0$ for all the algorithms. According to Theorem~\ref{theo.unconstrained_0}, for $\gamma = 1$, we need $C>2$ to ensure $\tau_0<1$ and therefore $O(h)$ convergence. In the case of Theorem~\ref{theo.unconstrained}, for $\gamma = 0$, $P = 1$ and $C=3$: we can set $\tau > 0.16$, the sampling period needs to be chosen as $h \leq \bar{h} =   4.2$, and the convergence region is the whole $\reals$, while for $\gamma =1$, $P = 1$ and $C=3$: we can set $\tau > 0.038$, $\bar{h} = 4.84$, and $\bar{R} = 12.7$ (notice that for greater $P$ or $C$ the requirements are less stringent).
 
In Figure~\ref{fig.centr1}, we plot the error $\|x_k - x^*(t_k)\|$ versus the discrete time $t_k$ for a sampling period of $h = 0.1$, for different schemes (we fix the correction steps at $C=3$ for all the algorithms and we study the behavior for different prediction steps $P$ and $\gamma$ values). Observe that the running gradient method~\cite{Popkov2005}, that is U-FOPC with no prediction and one correction step performs the worst, while U-FOPC with exact prediction (that is $P = \infty$) performs the best\footnote{The running gradient is a standard gradient descent with constant stepsize, where at each iteration one performs $C$ correction steps and the cost changes at each sampling time. }. Furthermore, we can notice that increasing $P$, one obtains better and better asymptotical error, with the drawback of an increased computational burden. Lastly, we notice how $\gamma =1$, that is having a Newton-like prediction step helps in achieving a faster convergence, and yet it appears that the asymptotical error is slightly greater than using $\gamma = 0$ (i.e., tangential prediction).  

The differences in performance can be also appreciated by varying $h$ and observing the worst case error floor size which is defined as 
$ 
%\begin{equation}\label{efl}
\max_{k>\bar{k}} \{\|x_k - x^*(t_k)\|\},
%\end{equation}
$
where $\bar{k} = 10^4$ in the simulations. Figure~\ref{fig.centr2} illustrates the error as a function of $h$. The performance differences between the proposed methods that may be observed here corroborate the differences seen in Figure \ref{fig.centr1}. In particular, the U-FOPC method with $P=0, C=1$ achieves the largest worst case error bound, while exact prediction with $\gamma = 0$ attains the best case error bound. Notice also the dashed lines displaying the theoretical performance of $O(h)$, $O(h^2)$, and the fact that for any finite $P$ there is a trade-off between computational complexity and asymptotical error\footnote{The simulation code is made available online to further analyze how different parameters can affect the algorithm trade-offs.}. 

\subsection{Constrained example}\label{sec:numconstr}

We consider here a mid-size optimization problem consisting of $n = 1000$ scalar variables. The cost function we study has the form
\begin{equation}
f(\x; t) = \frac{1}{2}\|\x + {\bf 1}_n\|^2_{\Q} + \sum_{i=1}^n \kappa_i \sin^2(\omega t + \varphi_i)\,\exp(\mu (x_{(i)}-2)^2),
\end{equation}
where we have defined ${\bf 1}_n$ as the column vector of all ones of dimension $n$, while $x_{(i)}$ is the $i$-th component of $\x\in \reals^n$. In addition, the matrix $\Q$ is chosen as $\Q = {\bf I}_n + \vv\vv^\transp/n$ with $\vv$ being a vector randomly generated by a normal distribution of mean $0$ and variance $1$, $\kappa_i \sim \mathcal{U}_{[0,1]} $, $\omega = 0.1\pi $, $\varphi \sim \mathcal{N}(0,\pi)$, and $\mu = 0.25$. 

We study the time-varying problem
\begin{equation}\label{prob.vector}
\minimize_{\x \in [0,0.4]^n} \, f(\x; t).
\end{equation}
We notice that the cost function $f$ verifies the Assumptions~\ref{as.str}-\ref{as.smooth} on on $[0,0.4]^n$, which is our optimization set (even though it would not satisfy them on the whole $\reals^n$). In particular, $m = 1$ and $L = 6.07$. 

One could run a similar analysis as the unconstrained example, however here we focus on realistic run-time constraints. Every time a new function is available, a number of correction steps are performed. The number depends on how fast we need the corrected variable to be available and the computational time necessary to compute the gradient and perform the correction step. We fix at $r_1 h$, with $r_1<1$ the time allocated for the correction steps, while $t_{\textrm{C}}$ is the time to perform one correction step. For the above considerations, we can afford to run
\begin{equation}\label{opt.c}
C = \lfloor r_1 h/ t_{\textrm{C}}\rfloor,
\end{equation}  
correction steps. After the corrected variable is available, one can use it for the decision making process (which may require extra time to be performed). For the time-varying algorithm perspective, one can use the variable to either run $P$ gradient prediction, or $C'$ extra correction steps (to improve the corrected variable for having a better starting point when a new function becomes available). Fix at $r_2 h$, with $r_2<1$ the time allocated for the prediction (or extra correction) steps. The affordable number of prediction steps can be determined considering that $P$ prediction steps require a time equal to $\bar{t} + P t_{\textrm{P}}$, where $\bar{t}$ is the time required to evaluate the Hessian, gradient, and time derivative of the gradient, while $t_{\textrm{P}}$ is the time to perform one prediction calculation. Thus, 
\begin{equation}\label{opt.p}
P = \lfloor (\,r_2 h - \bar{t}\,)/ t_{\textrm{P}}\rfloor.
\end{equation}  
The affordable extra correction steps $C'$ can be computed as in~\eqref{opt.c}, substituting $r_1$ with $r_2$. 

In the simulation example, we choose $r_1 = r_2 = 0.5$, while by running the experiments on a $1.8$~GHz Intel Core i5, we empirically fix $t_{\textrm{C}} = .76$~ms, $\bar{t} = 10$~ms, $t_{\textrm{P}} = .62$~ms. Note that the time that would be needed to solve the prediction step exactly (by solving a quadratic program) is $190$~ms, which is not affordable in the considered sampling period range.%\footnote{Potential time savings for this box-constrained quadratic program could be achieved by parallel algorithms as suggested in~\cite{}, but they are not considered here.}. 

In addition, we consider the situation in which one can use the whole sampling period to do correction, that is $r_1 = 1$, while $r_2 = 0$, and we call this case \emph{total correction}. This situation is particularly interesting when one has to make a choice whether to stop the correction steps to perform prediction, or to continue to do correction steps till a new function evaluation becomes available. Note that the correction+extra correction strategy is different from the total correction one, since the error is computed with the corrected variable (which is used for the decision making process), that is after $r_1 h$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
%\psfragfig*[width=0.75\textwidth, trim=0 -0.1cm 0 0, clip=on]{Figure/fig3}
{
\psfrag{x}[c]{\footnotesize Sampling period $h$ in [ms]}
\psfrag{y}[c]{\footnotesize Asymptotical worst-case error}
\psfrag{Ecorr}{\footnotesize Correction + Extra correction, $r_1$ = $0.5$, $r_2$ = $0.5$}
\psfrag{CorrTotCorrTotCorrTotCorrTot}{\footnotesize Total correction, $r_1$ = $1$, $r_2$ = $0$}
\psfrag{Pred}{\footnotesize C-FOPC Algorithm, $r_1$ = $0.5$, $r_2$ = $0.5$}
}
\includegraphics[width=0.5\textwidth]{Figure/fig3}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/first_error_h.pdf}
\caption{Asymptotical worst case error floor with respect to the sampling time interval $h$ for different algorithms applied to~\eqref{prob.vector}}
\label{fig.centr3}
\end{figure}

In Figure~\ref{fig.centr3}, we report the asymptotical worst-case error w.r.t the sampling period for the three considered cases (correction+extra correction, total correction, and prediction-correction, i.e. the C-FOPC algorithm)\footnote{Note that both the correction+extra correction and the total correction strategies are in fact (running) projected gradient descent algorithms.}, while the number of prediction steps and correction steps are optimized via the available resources as in Eq.s~\eqref{opt.c}-\eqref{opt.p}. With the simulation parameters, for $h = 6$~ms, we can perform $C = C' = 3$ steps of correction and extra correction, or $C = 7$ steps of (total) correction. For $h = 40$~ms, these values are $C = C' = 26$ and $C = 52$, respectively. For the prediction-correction strategy, for $h = 22$~ms, then $C = 14$ and $P = 1$, while for $h = 40$~ms, $C = 26$ and $P = 16$. 

For sampling times below $22$~ms, prediction cannot be performed due to time constraints. For sampling periods greater or equal than $22$~ms, prediction can be performed and for $h = [22, 40]$~ms, then $\bar{h} = [90, 370]$~ms, and $\bar{R} = [.13, .68]$. We see clearly that, in this simulation example, if prediction is affordable, the prediction-correction strategy, that is our C-FOPC algorithm is to be preferred to traditional correction-only schemes, since it achieves a lower asymptotical worst-case error. We notice that this error is lower by an half order of magnitude, while the error of the correction-extra correction and the total correction strategy are practically the same. For completeness, we report that $\x_0$ is chosen to be zero.%, while the initial optimality gap is $.30$, which indicates that, for the first sampling periods, the algorithm starts outside the attraction region, in the global $O(h)$ convergence zone, and then eventually reaches the local $O(h^2)$ convergence region. 

%As we notice, for sampling times below $22$~ms, prediction cannot be performed due to time constraints. For sampling periods greater or equal than $22$~ms, prediction can be performed and the conditions of Theorem~\ref{theo.constrained} are also satisfied, and in particular for $h = [22, 40]$~ms, then $\bar{h} = [90, 370]$~ms, and $\bar{R} = [.13, .68]$. We see clearly that, in this simulation example, if prediction is affordable, the prediction-correction strategy, that is our C-FOPC algorithm is to be preferred to traditional correction-only schemes, since it achieves a lower asymptotical worst-case error. We notice that this error is lower by an half order of magnitude, while the error of the correction-extra correction and the total correction strategy are practically the same. 

The result is quite remarkable, telling that performing Newton-like prediction steps on a fixed (Hessian, gradient, time derivative) triple can be computationally much more interesting that performing correction steps on a varying (i.e., re-updated) gradient.  

In Figure~\ref{fig.centr4}, we report the time trajectories of a number of variables for the three strategies to appreciate how the constraints are in fact active. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
%\psfragfig*[width=0.75\textwidth, trim=0 -0.1cm 0 0, clip=on]{Figure/fig4}
{
\psfrag{x}[c]{\footnotesize Time [s]}
\psfrag{y}[c]{\footnotesize Trajectories $\{\x_k\}$ and $\x^*(t)$}
\psfrag{xopt}{\footnotesize Optimal trajectory $\x^*(t)$}
\psfrag{Ecorr}{\footnotesize Correction + Extra correction, $r_1$ = $0.5$, $r_2$ = $0.5$}
\psfrag{CorrTotCorrTotCorrTotCorrTot}{\footnotesize Total correction, $r_1$ = $1$, $r_2$ = $0$}
\psfrag{Pred}{\footnotesize C-FOPC Algorithm, $r_1$ = $0.5$, $r_2$ = $0.5$}
}
\includegraphics[width=0.5\textwidth]{Figure/fig4}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/first_error_h.pdf}
\caption{Trajectories of $\{\x_k\}$ and optimal trajectory $\x^*(t)$ for different algorithms applied to~\eqref{prob.vector}, with $h = 22$~ms.}
\label{fig.centr4}
\end{figure}

\subsection{An example of realistic application}

As an example of realistic application, we consider the problem of optimizing  the operation of aggregations  of  energy resources connected to a power distribution system -- a research task that has gained significant interest from academic and industrial sectors because of the increased  deployment of distributed energy resources (DERs).  The proposed algorithm can be implemented to enable a \emph{real-time} optimization of the DER operation, where the term ``real-time'' refers to a setting where the power setpoints of the DERs are updated on a second or subsecond time scale based on streaming measurements, to maximize operational objectives while coping with variability of ambient conditions and non-controllable energy assets~\cite{DallAnese2016, LowOnlineOPF, AndreayOnlineOpt}. 


Consider then a distribution network consisting of one slack bus and $N$ nodes with controllable DERs. Let $s_n = p_n + j q_n \in \mathbb{C}$ denote the net injected complex power at node $j$,  and let $p_0  \in  \mathbb{R}$ denote  the active power flow at a point of connection of the distribution system with the rest of the grid.  For future developments, let $\x_{n} := [\Re\{s_n\}, \Im\{s_n\}]^\transp$ collect the active and reactive setpoints of the DER at node $n$. To further simplify the notation, define the vector $\x := [\x_{1}^{\transp}, \ldots, \x_N^{\transp}]^{\transp}$. To facilitate the development of computationally-affordable algorithms, we postulate the following approximate linear relationship between $\x$ and the active powers $p_0$:  
\begin{align} 
\tilde{p}_0(\x, t) & =  \m^{\transp}(t) [\x - \x_\ell(t)] + n(t) \nonumber \\
& := \sum_{n = 1}^N \m^{\transp}_n(t)[\x_{n} - \x_{n, \ell}(t) ] + \eta(t) \label{eqn:lin_s0}
\end{align}
where $\x_{n,\ell}(t)$ denotes the non-controllable loads and the model parameters $\{\bm_n(t) \in \mathbb{R}^2\}$ and $\eta(t)  \in \mathbb{R}$ can be obtained as shown in, e.g.,~\cite{DallAnese2016,bolognani2015linear}. These model parameters can be either fixed or time-varying.

Consider a discrete-time operational setting where the setpoints of the DERs are updated at time instants $t_k = h k$, with $k \in \mathbb{N}$ and $h > 0$ based on the specific implementation requirements (e.g., second, sub-second,  or a few seconds), and formulate the following optimization problem per time $k$:
\begin{subequations} 
\label{eq:powerproblem}
\begin{align} 
\min_{\substack{\x}\in\mathbb{R}^{2n}} & \, \sum_{n=1}^N  C_{n}(\x_{n}; t_k) + \frac{\gamma}{2} \left (p_0^{\mathrm{set}}(t_k) - \tilde{p}_0(\x, t_k)\right )^2 \\
\textrm{s.~t.:~} & \quad \x_{n} \in Y_{n}, \, \forall \,\,\, n = 1, \dots, N \label{eqn:constr_Y_exact} 
 \end{align}
\end{subequations}
where  $p_0^\mathrm{set}(t_k) $ is a setpoint for  the aggregate power at the point of connection~\cite{AndreayOnlineOpt},  $\gamma > 0$ is a design parameter that influences the ability to track the reference signal $p_0^\mathrm{set}(t_k) $, $C_n(\x_{n}; t_k):\mathbb{R}^2\times\mathbb{R}_{+} \to \mathbb{R}$ is a local cost function, and $Y_{n}$ specifies the operating region for DER $n$. For example, $Y_{n}$ can be given by
\begin{align} 
Y_{n} = \{p_n, q_n: \underline{p}_n \leq p_n \leq \overline{p}_n, \underline{q}_n \leq q_n \leq \overline{q}_n\}
 \end{align}
with $ \underline{p}_n$, $\overline{p}_n$, $ \underline{q}_n$, and $\overline{q}_n$ given limits. This is the case, for example, for variable-speed drives, natural-gas generators, electric vehicle chargers, and renewable sources of energy operating with (fixed) headroom from the maximum available power.  Problem~\eqref{eq:powerproblem} is pertinent for settings where a number of customers aim at maximizing given performance objectives related to the DERs (e.g., minimization of net electricity payment), while partaking in grid services;  specifically, customers may be incentivized by utility or aggregators to adjust the DERs' output powers so that the aggregate power $\tilde{p}_0(\x; t_k)$ can be driven to the setpoint $p_0^\mathrm{set}(t_k)$.

For the numerical experiments, we utilize real data belonging to residential loads from a neighborhood located in the Sacramento metro area~\cite{Bank13}. The data have a granularity of 1 second and they are utilized to populate the IEEE 37-node test feeder (see e.g.,~\cite{DallAnese2016}). For simplicity, we consider a single-phase equivalent of the feeder. The model parameters $\{\m_n(t) \in \mathbb{R}^2\}$ and $\eta(t)  \in \mathbb{R}$ are computed  as shown in~\cite{DallAnese2016}.  With this setting, the non-controllable portion of $\tilde{p}_0(\x; t_k)$ in~\eqref{eq:powerproblem}, which defined as 
\begin{align} 
a(t_k) := - \sum_{n = 1}^N \m^{\transp}_n(t_k)\x_{n, \ell}(t_k) + \eta(t_k) 
\end{align}
varies over time as illustrated in Figure~\ref{fig:mov_a}. The trajectory for the setpoint $p_0^\mathrm{set}(t_k)$ is also provided in Fig.~\ref{fig:mov_a}; in the considered setting, the specified setpoints promote a smoother variability of the aggregate load $\tilde{p}_0(\x; t)$ over time. 

With reference to the feeder in~\cite{DallAnese2016}, we assume that controllable DERs are located at nodes 4, 7, 10, 13, 17, 20, 22, 26, 30, and 35,  and it is assumed that the real power $p_n$ can be controlled within the interval $ \underline{p}_n = -50$ kW and $\overline{p}_n = 50$ kW. The cost functions $C_n(\x_n;t_k) = p_n^2$ and $\gamma = 2$. This setting is representative of the case where DERs can deviate their active powers from a nominal operating point to provide services to the grid, but their adjustment is limited within $[\underline{p}_n, \overline{p}_n]$. In addition, $\m_n(t_k)$ is considered constant in time (as often varies at slower time-scales than $a(t_k)$, typically minutes).

To track the solution trajectory $\x^*(t_k)$ of~\eqref{eq:powerproblem} while $k$ increases, we run both a running projected gradient algorithm, i.e., Algorithm~\ref{algo_fo} with $P=0$, and our prediction-correction Algorithm~\ref{algo_fo}.  The prediction step is computed by approximating the time-derivative of the gradient as explained in~\cite{Paper1}, which does not affect convergence or the rates. 

For the simulation runs, the functional parameters are $m = 1$ and $L = 21$, while since the cost function is a time-varying quadratic function with constant Hessian, $C_1 = 0$, $C_2=0$, the convergence attraction region is the whole space and there is no upper bound on the sampling period (see Theorem~\ref{theo.constrained}). 
%
We choose the stepsizes $\alpha$ and $\beta$ as $\alpha = \beta = 0.0048$, such that $\varrho_{\textrm{P}} = \varrho_{\textrm{C}}<1 $, while $h = 1$~s, and $\x_0 = \bf{0}$.

We keep the computational time fixed in our comparison of running projected gradient and prediction-correction algorithm, so that we could identify better the contribution of the prediction step. With the same notation and nomenclature of Section~\ref{sec:numconstr}, we look at a total-correction strategy for the running projected gradient with $C = 3$. Each correction step takes $76$~$\mu$s on a $1.8$~GHz Intel Core i5 (and $3$ steps, $228$~$\mu$s). For the prediction-correction algorithm, we fix $C = 1$, while we choose $P = 2$, such that the total computational time is $206$~$\mu$s, which is similar to the running strategy. 

We report the error $\|\x_{k} - \x^*(t_k)\|$ of the two strategies in time in Figure~\ref{fig:fig6} (for readability purposes only for the time frame $12$:$38$-$12$:$48$, but in fact it is qualitatively the same for all the other time frames), and in particular the averaged asymptotical error (averaged in the time frame $12$:$10$-$13$:$00$) of the running method ($P=0$) is $3.73$~kW, while the one of the prediction-correction algorithm is $3.14$~kW. As captured in Figure~\ref{fig:fig6}, the prediction-correction algorithm seems to be more reactive to changes, responding more quickly, which is expected. This further corroborates the usefulness of the prediction step, hence of the prediction-correction methodology, even when real noisy time-varying data is used, and the time derivative of the gradient can only be approximated. %Further analysis of this numerical set up is left as future research.   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
%\psfragfig*[width=0.55\textwidth, trim=0 0cm 0 0, clip=on]{Figure/F_power}
{
\psfrag{x}[c]{\footnotesize Time}
\psfrag{y}[c]{\footnotesize Aggregate active power [kW]}
\psfrag{Non-controllable aggregate load}{\footnotesize Non-controllable aggr. load}
\psfrag{Setpoint}{\footnotesize Setpoint}
%\psfrag{x}[c]{\footnotesize Sampling time $t_k$}
%\psfrag{y}[c]{\footnotesize Tracking error $\|x_k - x^*(t_k)\|$}
%\psfrag{runninggradientgradientgradientgradient}{\footnotesize \footnotesize U-FOPC, $P=0$, $C=3$, $\gamma = 0$}
%\psfrag{gradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 0$}
%\psfrag{approxgradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 1$}
%\psfrag{newton3}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 0$}
%\psfrag{newton4}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 1$}
%\psfrag{newton}{\footnotesize\footnotesize U-FOPC, $P=3$, $C=3$, $\gamma = 0$}
%\psfrag{newton2}{\footnotesize \footnotesize U-FOPC, $P=3$, $C=3$, $\gamma = 1$}
}
\includegraphics[width=0.5\textwidth]{Figure/F_power}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/first_error_t.pdf}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/error_t_with_bounds.pdf}
\caption{Aggregate effect of the non-controllable residential load on the power at the point of common coupling $\tilde{p}_0(\x; t_k)$ [kW] in the considered simulation setting. The red trajectory represents the prescribed setpoint $p_0^\mathrm{set}(t_k)$. }
\label{fig:mov_a}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
%\psfragfig*[width=0.55\textwidth, trim=0 0cm 0 0, clip=on]{Figure/Fig6}
{
\psfrag{x}[c]{\footnotesize Time}
\psfrag{y}[c]{\footnotesize Tracking error $\|x_k - x^*(t_k)\|$}
\psfrag{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa}{\footnotesize \footnotesize C-FOPC, $P=0$, $C=3$}
\psfrag{b}{\footnotesize \footnotesize C-FOPC, $P=2$, $C=1$}
%\psfrag{gradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 0$}
%\psfrag{approxgradient}{\footnotesize U-FOPC, $P=1$, $C=3$, $\gamma = 1$}
%\psfrag{newton3}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 0$}
%\psfrag{newton4}{\footnotesize \footnotesize U-FOPC, $P=\infty$, $C=3$, $\gamma = 1$}
%\psfrag{newton}{\footnotesize\footnotesize U-FOPC, $P=3$, $C=3$, $\gamma = 0$}
%\psfrag{newton2}{\footnotesize \footnotesize U-FOPC, $P=3$, $C=3$, $\gamma = 1$}
}
\includegraphics[width=0.5\textwidth]{Figure/Fig6}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/first_error_t.pdf}
%\includegraphics[width=0.5\textwidth,height=0.3\textwidth]{Figure/error_t_with_bounds.pdf}
\caption{Tracking error in [kW] for the two considered strategies in the time frame $12$:$38$-$12$:$48$. }
\label{fig:fig6}
\end{figure}

\section{Conclusions}\label{sec:concl}

We have proposed first-order algorithms to find and track the solution trajectory of strongly convex, strongly smooth constrained time-varying optimization problems. These algorithms rely on a discrete-time prediction-correction strategy, by which at each sampling time, the decision variables are corrected through one or multiple projected gradient steps, and then used to predict the next decision variables via successive projected gradient steps on a suitably defined quadratic program. The proposed algorithms exhibit better asymptotical accuracy than state-of-the-art correction-only schemes, even when computational complexity issues are taken into account. %This makes them a very appealing strategy, especially for smooth small-to-mid-scale problems.




%\newpage
